Updated theoretical Period-Age and Period-Age-Color relations for Galactic Classical Cepheids: an application to the Gaia DR2 sample

Updated evolutionary and pulsational model predictions are combined in order to interpret the properties of Galactic Classical Cepheids in the Gaia Data Release 2. In particular, the location of the instability strip boundaries and the analytical relations connecting pulsation periods to the intrinsic stellar parameters are combined with evolutionary tracks to derive reliable and accurate period-age, and the first theoretical period-age-color relations in the Gaia bands for a solar chemical abundance pattern ($Z$=$0.02$, $Y$=$0.28$). The adopted theoretical framework takes into account possible variations in the mass-luminosity relation for the core helium-burning stage as due to changes in the core convective overshooting and/or mass loss efficiency, as well as the impact on the instability strip boundaries due to different assumptions for superadiabatic convection efficiency. The inferred period-age and period-age-color relations are applied to a selected sample of both fundamental and first overtone Gaia Cepheids, and individual ages for the various adopted theoretical scenarios are derived. The retrieved age distributions confirm that a variation in the efficiency of superadiabatic convection in the pulsational model computations has a negligible effect, whereas a brighter Mass-Luminosity relation, as produced by mild overshooting, rotation or mass loss, implies significantly older age predictions. Moreover, older Cepheids are found at larger Galactocentric distances, while first overtone Cepheids are found to be systematically older than the fundamental ones. The comparison with independent age distribution analysis in literature supports the predictive capability of current theoretical framework.

==> tab_age_1.5_A_FO_PA_PAC.tex <==
\begin{table}
\begin{tabular}{cccccccccccccc}
Gaia DR2 source Id & RA[deg] & DEC[deg] & P[d] & G[mag] & G_BP[mag] & G_RP[mag] & E(gbp-grb)[mag] & sigma_E(gbp-grb)[mag] & Note & t_pa[Myr] & sigma(t)_pa[Myr] & t_pac[Myr] & sigma(t)_pac[Myr] \\
5958267083020200448 & 263.74736 & -44.83491 & 0.48582 & 15.31 & 15.67 & 14.78 & 0.48 & 0.11 & G & 175.45 & 21.01 & 168.26 & 17.82 \\
4652801401061740800 & 72.89387 & -73.52919 & 0.54856 & 17.88 & 18.20 & 17.42 & 0.32 & 0.11 & G & 167.21 & 20.02 & 161.55 & 17.11 \\
4649684869708905600 & 78.33946 & -73.18860 & 0.62515 & 17.60 & 17.85 & 17.14 & 0.28 & 0.11 & G & 158.78 & 19.01 & 149.33 & 15.82 \\
4757521942202075904 & 84.00743 & -62.92647 & 0.66840 & 17.23 & 17.49 & 16.81 & 0.21 & 0.11 & G & 154.63 & 18.51 & 147.46 & 15.62 \\
4648894973678313600 & 78.74744 & -76.16060 & 0.68428 & 17.58 & 17.85 & 17.13 & 0.26 & 0.11 & G & 153.20 & 18.34 & 145.22 & 15.38 \\
426097765508018560 & 13.85755 & 59.72753 & 0.69910 & 13.67 & 14.18 & 12.99 & 0.72 & 0.12 & G & 151.90 & 18.19 & 145.17 & 15.38 \\
5255955821811454592 & 150.19748 & -61.57770 & 0.70107 & 14.74 & 15.09 & 14.05 & 0.65 & 0.12 & G & 151.73 & 18.17 & 137.97 & 14.61 \\
6380124062227694208 & 357.83150 & -72.69153 & 0.72213 & 17.86 & 18.07 & 17.44 & 0.19 & 0.11 & G & 149.96 & 17.96 & 139.41 & 14.77 \\
4648520761770393088 & 85.76598 & -75.18605 & 0.81359 & 17.25 & 17.54 & 16.80 & 0.25 & 0.11 & G & 143.05 & 17.13 & 135.51 & 14.35 \\
4652889258915055488 & 72.48404 & -73.00018 & 0.95488 & 17.24 & 17.54 & 16.77 & 0.27 & 0.11 & G & 134.26 & 16.08 & 126.16 & 13.36 \\
5542032357742851712 & 125.44982 & -37.46816 & 1.01087 & 16.30 & 17.08 & 15.38 & 1.19 & 0.12 & O & 131.26 & 15.72 & 122.76 & 13.00 \\
4652312599416423040 & 68.88711 & -74.56297 & 1.01787 & 17.03 & 17.30 & 16.59 & 0.18 & 0.11 & G & 130.90 & 15.67 & 123.28 & 13.06 \\
4649732762885142272 & 77.24295 & -73.85941 & 1.02268 & 17.06 & 17.35 & 16.58 & 0.26 & 0.11 & G & 130.66 & 15.64 & 122.03 & 12.92 \\
5860021737714232576 & 190.95445 & -65.86875 & 1.03985 & 15.64 & 16.14 & 14.78 & 0.82 & 0.1 & O & 129.80 & 15.54 & 123.61 & 13.09 \\
4690203483799384832 & 12.47494 & -70.52511 & 1.05413 & 16.86 & 17.06 & 16.51 & 0.03 & 0.11 & G & 129.10 & 15.46 & 120.55 & 12.77 \\
5879216457587855872 & 220.33866 & -58.95261 & 1.05620 & 17.35 & 19.40 & 15.97 & 3.13 & 0.28 & G & 129.00 & 15.45 & 106.51 & 11.28 \\
4650448854192694144 & 84.54695 & -73.04031 & 1.05937 & 17.06 & 17.37 & 16.55 & 0.29 & 0.11 & G & 128.85 & 15.43 & 120.72 & 12.79 \\
5264781017499895936 & 90.70098 & -74.81688 & 1.06456 & 17.00 & 17.31 & 16.47 & 0.33 & 0.11 & G & 128.60 & 15.40 & 119.49 & 12.66 \\
5262612604471337344 & 112.55193 & -74.18419 & 1.06846 & 16.96 & 17.27 & 16.47 & 0.28 & 0.11 & G & 128.41 & 15.38 & 120.29 & 12.74 \\
4636454029673286400 & 17.74748 & -75.46487 & 1.07579 & 16.93 & 17.12 & 16.56 & 0.06 & 0.11 & G & 128.07 & 15.33 & 118.85 & 12.59 \\
457599392117044224 & 37.51571 & 56.69572 & 1.08362 & 14.26 & 14.77 & 13.58 & 0.64 & 0.12 & G & 127.70 & 15.29 & 121.01 & 12.82 \\
4649292305396315904 & 75.79134 & -74.77767 & 1.08725 & 16.91 & 17.17 & 16.47 & 0.17 & 0.11 & G & 127.53 & 15.27 & 119.38 & 12.64 \\
4757456147604475392 & 81.34978 & -62.60265 & 1.09098 & 16.36 & 16.57 & 16.01 & 0.03 & 0.11 & G & 127.36 & 15.25 & 119.56 & 12.66 \\
5984686633766186752 & 239.21288 & -47.24860 & 1.10006 & 17.53 & 18.72 & 16.43 & 1.79 & 0.18 & G & 126.94 & 15.20 & 116.56 & 12.35 \\
5978153915467156992 & 257.17120 & -34.22662 & 1.10037 & 16.06 & 16.91 & 15.10 & 1.29 & 0.15 & G & 126.93 & 15.20 & 117.28 & 12.42 \\
5280952256562534784 & 106.38399 & -67.14481 & 1.11229 & 16.67 & 17.24 & 15.96 & 0.72 & 0.12 & G & 126.39 & 15.13 & 120.18 & 12.73 \\
5351436724362450304 & 157.99176 & -58.24496 & 1.11936 & 11.09 & 11.62 & 10.41 & 0.65 & 0.12 & G & 126.07 & 15.09 & 120.10 & 12.72 \\
4296034376370310144 & 292.98705 & 8.05287 & 1.12815 & 15.60 & 16.01 & 15.02 & 0.44 & 0.11 & G & 125.68 & 15.05 & 118.71 & 12.57 \\
4649121747955000448 & 77.26192 & -74.66745 & 1.12938 & 16.84 & 17.13 & 16.41 & 0.17 & 0.11 & G & 125.62 & 15.04 & 118.78 & 12.58 \\
6388401494999249280 & 359.61640 & -68.76654 & 1.14138 & 17.31 & 17.49 & 17.02 & 0.0 & 0.11 & G & 125.10 & 14.98 & 112.44 & 11.91 \\
4691907009561849088 & 13.52583 & -70.09840 & 1.14422 & 17.39 & 17.61 & 17.00 & 0.07 & 0.11 & G & 124.98 & 14.96 & 116.83 & 12.37 \\
5610147893350949504 & 107.91737 & -26.97786 & 1.14435 & 13.22 & 13.56 & 12.71 & 0.31 & 0.11 & G & 124.97 & 14.96 & 117.13 & 12.41 \\
4757580426778468480 & 83.23229 & -62.74256 & 1.14539 & 16.58 & 16.85 & 16.19 & 0.1 & 0.11 & G & 124.93 & 14.96 & 118.22 & 12.52 \\
4757352209396545664 & 82.53930 & -63.27145 & 1.15017 & 16.74 & 17.03 & 16.28 & 0.21 & 0.11 & G & 124.72 & 14.93 & 116.62 & 12.35 \\
4117130567344719232 & 266.37656 & -21.56332 & 1.15336 & 15.57 & 16.66 & 14.46 & 1.74 & 0.16 & O & 124.58 & 14.92 & 111.12 & 11.77 \\
5604731630351388928 & 109.71092 & -32.64398 & 1.16324 & 12.74 & 13.02 & 12.29 & 0.19 & 0.11 & G & 124.16 & 14.87 & 116.31 & 12.32 \\
4693976423589147648 & 27.99098 & -69.98706 & 1.16412 & 17.18 & 17.36 & 16.80 & 0.04 & 0.11 & G & 124.13 & 14.86 & 114.76 & 12.16 \\
5237294738660182912 & 173.70859 & -65.08935 & 1.16453 & 16.56 & 17.60 & 15.48 & 1.57 & 0.15 & O & 124.11 & 14.86 & 116.51 & 12.34 \\
5265006108149270016 & 91.76627 & -74.14746 & 1.16991 & 16.91 & 17.27 & 16.39 & 0.33 & 0.11 & G & 123.88 & 14.83 & 116.76 & 12.37 \\
4703373747608086272 & 5.59416 & -68.47642 & 1.17306 & 17.24 & 17.38 & 16.89 & 0.0 & 0.11 & G & 123.75 & 14.82 & 112.73 & 11.94 \\
4652373209998248832 & 72.57003 & -74.23271 & 1.18622 & 16.94 & 17.25 & 16.45 & 0.25 & 0.11 & G & 123.21 & 14.75 & 115.34 & 12.22 \\
4650275547972932608 & 84.58900 & -74.11395 & 1.20074 & 16.63 & 16.91 & 16.17 & 0.19 & 0.11 & G & 122.61 & 14.68 & 114.90 & 12.17 \\
4685118349894560128 & 7.25192 & -75.20856 & 1.20327 & 17.11 & 17.30 & 16.78 & -0.0 & 0.11 & G & 122.51 & 14.67 & 112.92 & 11.96 \\
4649352954637972224 & 73.46156 & -74.63390 & 1.21391 & 16.75 & 17.07 & 16.29 & 0.22 & 0.11 & G & 122.08 & 14.62 & 115.76 & 12.26 \\
4705063044144940416 & 21.21681 & -65.43852 & 1.21627 & 17.07 & 17.22 & 16.77 & 0.0 & 0.11 & G & 121.99 & 14.61 & 108.10 & 11.45 \\
5612678213207148032 & 111.30775 & -27.79913 & 1.21642 & 13.14 & 13.59 & 12.52 & 0.5 & 0.11 & G & 121.99 & 14.61 & 115.17 & 12.20 \\
5311837740049326848 & 137.44370 & -52.56716 & 1.25693 & 17.96 & 19.08 & 16.88 & 1.68 & 0.17 & G & 120.41 & 14.42 & 110.47 & 11.70 \\
5311347637061714304 & 137.25223 & -53.59880 & 1.29623 & 12.22 & 12.74 & 11.55 & 0.61 & 0.12 & G & 118.95 & 14.24 & 112.54 & 11.92 \\
5613275454180075264 & 112.04712 & -26.49072 & 1.30756 & 15.45 & 16.20 & 14.57 & 1.07 & 0.14 & G & 118.54 & 14.19 & 110.63 & 11.72 \\
5857396447520828288 & 196.47891 & -67.30630 & 1.31275 & 15.12 & 15.57 & 14.43 & 0.61 & 0.12 & G & 118.36 & 14.17 & 108.65 & 11.51 \\
4134649262221615104 & 258.39633 & -18.09767 & 1.32706 & 14.44 & 14.76 & 13.89 & 0.33 & 0.11 & G & 117.85 & 14.11 & 108.60 & 11.50 \\
5851370058646053120 & 205.56594 & -66.97277 & 1.39185 & 15.25 & 15.76 & 14.57 & 0.61 & 0.12 & G & 115.65 & 13.85 & 108.61 & 11.50 \\
4637883330365589376 & 19.13912 & -75.74839 & 1.39916 & 16.91 & 17.17 & 16.48 & 0.12 & 0.11 & G & 115.41 & 13.82 & 107.60 & 11.40 \\
4650280594551796864 & 83.97161 & -74.03424 & 1.44214 & 16.55 & 16.86 & 16.09 & 0.19 & 0.11 & G & 114.03 & 13.65 & 106.89 & 11.32 \\
4688096922599486336 & 22.41111 & -70.44117 & 1.44633 & 16.55 & 16.77 & 16.14 & 0.08 & 0.11 & G & 113.90 & 13.64 & 105.02 & 11.12 \\
4649981772207548672 & 89.03492 & -74.93384 & 1.45533 & 16.50 & 16.86 & 16.02 & 0.23 & 0.11 & G & 113.62 & 13.60 & 108.00 & 11.44 \\
5533237604747205120 & 122.05543 & -43.25773 & 1.50255 & 13.94 & 14.37 & 13.32 & 0.46 & 0.11 & G & 112.20 & 13.43 & 104.99 & 11.12 \\
6715705353307835776 & 286.24834 & -41.24300 & 1.56682 & 11.93 & 12.75 & 11.03 & 1.13 & 0.14 & G & 110.35 & 13.21 & 103.01 & 10.91 \\
5279103771359717760 & 98.49359 & -69.58687 & 1.56734 & 15.91 & 16.13 & 15.52 & 0.04 & 0.11 & G & 110.34 & 13.21 & 102.17 & 10.82 \\
5236253535532145792 & 178.47741 & -66.15551 & 1.61221 & 15.41 & 16.07 & 14.58 & 0.92 & 0.11 & O & 109.11 & 13.06 & 100.22 & 10.61 \\
4652839746530357120 & 72.51981 & -73.13928 & 1.61261 & 16.33 & 16.63 & 15.91 & 0.11 & 0.11 & G & 109.10 & 13.06 & 102.93 & 10.90 \\
4690389954099065984 & 11.18371 & -70.34446 & 1.62180 & 17.50 & 17.73 & 17.09 & 0.07 & 0.11 & G & 108.85 & 13.03 & 99.98 & 10.59 \\
4633993842341089152 & 31.03923 & -77.07734 & 1.64148 & 17.45 & 17.73 & 17.00 & 0.14 & 0.11 & G & 108.33 & 12.97 & 100.19 & 10.61 \\
4684545126380271488 & 15.02763 & -75.21117 & 1.64178 & 16.00 & 16.23 & 15.64 & 0.0 & 0.11 & G & 108.33 & 12.97 & 100.18 & 10.61 \\
4650241016434474624 & 86.69286 & -73.38162 & 1.64223 & 16.14 & 16.45 & 15.72 & 0.11 & 0.11 & G & 108.31 & 12.97 & 102.08 & 10.81 \\
5238583980437740416 & 165.04708 & -66.57781 & 1.64338 & 14.57 & 15.07 & 13.89 & 0.59 & 0.12 & G & 108.28 & 12.97 & 100.68 & 10.66 \\
5317494559886504704 & 133.34151 & -54.05494 & 1.66917 & 13.41 & 13.79 & 12.85 & 0.33 & 0.11 & G & 107.62 & 12.89 & 100.38 & 10.63 \\
5253058471238877312 & 155.13635 & -62.12037 & 1.67042 & 13.72 & 14.18 & 13.10 & 0.48 & 0.11 & G & 107.59 & 12.88 & 100.83 & 10.68 \\
4649714659602296448 & 76.35029 & -74.03501 & 1.68909 & 16.17 & 16.44 & 15.76 & 0.08 & 0.11 & G & 107.11 & 12.83 & 99.84 & 10.57 \\
4650425115918541312 & 85.71464 & -73.43898 & 1.69512 & 16.15 & 16.44 & 15.69 & 0.15 & 0.11 & G & 106.96 & 12.81 & 99.32 & 10.52 \\
5324781367038315648 & 132.52689 & -50.88632 & 1.70128 & 14.58 & 15.45 & 13.63 & 1.22 & 0.14 & G & 106.81 & 12.79 & 98.87 & 10.47 \\
5587628692622346624 & 116.43209 & -35.40995 & 1.71526 & 14.35 & 15.03 & 13.54 & 0.89 & 0.13 & G & 106.46 & 12.75 & 99.18 & 10.50 \\
5850702517654588928 & 207.15791 & -66.88149 & 1.72076 & 14.78 & 15.24 & 14.13 & 0.51 & 0.11 & G & 106.33 & 12.73 & 99.15 & 10.50 \\
5306502089316773248 & 141.31930 & -57.56125 & 1.73125 & 14.64 & 15.27 & 13.86 & 0.81 & 0.12 & G & 106.07 & 12.70 & 98.44 & 10.43 \\
5306051873674535680 & 146.31100 & -57.27895 & 1.73470 & 15.00 & 15.87 & 14.05 & 1.24 & 0.13 & O & 105.99 & 12.69 & 96.51 & 10.22 \\
4649467368264365312 & 79.98448 & -74.44347 & 1.74813 & 16.25 & 16.55 & 15.75 & 0.22 & 0.11 & G & 105.67 & 12.65 & 97.09 & 10.28 \\
5599120204043561600 & 113.85342 & -31.07499 & 1.74843 & 13.57 & 14.07 & 12.92 & 0.53 & 0.11 & G & 105.66 & 12.65 & 98.95 & 10.48 \\
2164475809937299584 & 317.78601 & 47.16828 & 1.76585 & 10.18 & 10.74 & 9.49 & 0.62 & 0.12 & G & 105.25 & 12.60 & 99.33 & 10.52 \\
5607793392275328640 & 106.26306 & -29.86583 & 1.79788 & 15.08 & 15.37 & 14.61 & 0.16 & 0.11 & G & 104.50 & 12.51 & 96.59 & 10.23 \\
4650394089074151168 & 85.29071 & -73.67826 & 1.82035 & 16.16 & 16.48 & 15.68 & 0.18 & 0.11 & G & 103.99 & 12.45 & 96.78 & 10.25 \\
4649470739818783104 & 79.60945 & -74.44693 & 1.82744 & 16.16 & 16.47 & 15.67 & 0.19 & 0.11 & G & 103.83 & 12.43 & 96.16 & 10.18 \\
5609883112903185152 & 108.15032 & -27.83878 & 1.83506 & 12.62 & 12.95 & 12.13 & 0.2 & 0.11 & G & 103.66 & 12.41 & 96.39 & 10.21 \\
4688179115387628544 & 24.10374 & -70.41784 & 1.84246 & 16.42 & 16.70 & 15.97 & 0.12 & 0.11 & G & 103.49 & 12.39 & 95.70 & 10.14 \\
5516544028942005120 & 126.74790 & -46.55246 & 1.90177 & 14.41 & 14.99 & 13.65 & 0.73 & 0.12 & G & 102.20 & 12.24 & 94.69 & 10.03 \\
5857773580024503552 & 201.67066 & -65.86683 & 1.93030 & 15.32 & 16.06 & 14.43 & 1.0 & 0.11 & O & 101.60 & 12.16 & 94.47 & 10.01 \\
5533667238912747648 & 122.49124 & -41.54244 & 1.94450 & 15.04 & 15.96 & 14.08 & 1.26 & 0.15 & G & 101.31 & 12.13 & 93.48 & 9.90 \\
508824711142351488 & 30.47766 & 62.70521 & 1.94936 & 13.87 & 14.63 & 12.99 & 1.02 & 0.13 & G & 101.21 & 12.12 & 93.86 & 9.94 \\
5329861901039268736 & 131.14422 & -46.08450 & 1.96760 & 14.26 & 15.19 & 13.29 & 1.26 & 0.13 & O & 100.83 & 12.07 & 94.66 & 10.03 \\
4650327358155154176 & 83.68263 & -74.01122 & 1.98597 & 15.82 & 16.08 & 15.39 & 0.07 & 0.11 & G & 100.46 & 12.03 & 92.62 & 9.81 \\
5241983434223208192 & 161.77131 & -62.17635 & 1.99082 & 14.89 & 15.70 & 13.97 & 1.07 & 0.12 & O & 100.37 & 12.02 & 94.73 & 10.03 \\
6723719246886877440 & 277.60780 & -39.85986 & 1.99883 & 12.26 & 13.26 & 11.26 & 1.38 & 0.15 & G & 100.21 & 12.00 & 92.44 & 9.79 \\
5606634988063582848 & 109.96244 & -28.79174 & 1.99937 & 12.52 & 12.89 & 11.97 & 0.29 & 0.11 & G & 100.20 & 12.00 & 93.13 & 9.86 \\
5864085979393757824 & 203.27370 & -64.58181 & 2.00621 & 15.53 & 16.47 & 14.52 & 1.37 & 0.14 & O & 100.06 & 11.98 & 90.21 & 9.55 \\
5406720409514852352 & 152.68706 & -50.15948 & 2.00631 & 11.89 & 12.35 & 11.28 & 0.42 & 0.11 & G & 100.06 & 11.98 & 93.63 & 9.92 \\
5858749121746467456 & 197.53034 & -65.31814 & 2.02235 & 14.71 & 15.40 & 13.88 & 0.9 & 0.11 & O & 99.74 & 11.94 & 92.35 & 9.78 \\
5251623535508264064 & 156.10874 & -64.71312 & 2.02842 & 12.49 & 12.95 & 11.87 & 0.44 & 0.11 & G & 99.62 & 11.93 & 92.97 & 9.85 \\
5322072960659445760 & 129.57544 & -50.47626 & 2.03043 & 15.39 & 16.23 & 14.43 & 1.2 & 0.14 & G & 99.59 & 11.92 & 90.63 & 9.60 \\
4640289096166011392 & 40.62046 & -74.72156 & 2.03078 & 16.16 & 16.41 & 15.73 & 0.06 & 0.11 & G & 99.58 & 11.92 & 91.56 & 9.70 \\
5543722994310379136 & 125.64924 & -34.40031 & 2.03970 & 14.33 & 14.88 & 13.60 & 0.69 & 0.1 & O & 99.41 & 11.90 & 90.45 & 9.58 \\
4190528813947695232 & 298.45948 & -9.93928 & 2.04003 & 14.23 & 14.62 & 13.67 & 0.32 & 0.11 & G & 99.40 & 11.90 & 92.15 & 9.76 \\
5245796334347122944 & 150.01533 & -66.27623 & 2.06344 & 8.09 & 8.53 & 7.54 & 0.3 & 0.06 & L & 98.95 & 11.85 & 94.48 & 10.01 \\
3054600330268450560 & 111.10215 & -7.85545 & 2.07131 & 10.15 & 10.57 & 9.59 & 0.33 & 0.11 & G & 98.80 & 11.83 & 92.71 & 9.82 \\
2195158098523149312 & 310.87509 & 61.75625 & 2.09946 & 14.31 & 14.85 & 13.59 & 0.63 & 0.12 & G & 98.28 & 11.77 & 90.60 & 9.60 \\
3398383973788673024 & 86.41888 & 18.65688 & 2.10240 & 7.88 & 8.29 & 7.35 & 0.23 & 0.02 & L & 98.22 & 11.76 & 94.72 & 10.03 \\
2203988169026743936 & 329.46631 & 61.01885 & 2.11413 & 7.51 & 8.05 & 6.84 & 0.55 & 0.07 & L & 98.00 & 11.73 & 91.98 & 9.74 \\
524799786155513984 & 18.62522 & 64.65289 & 2.11885 & 12.54 & 13.45 & 11.59 & 1.22 & 0.14 & G & 97.92 & 11.72 & 90.79 & 9.62 \\
3425495186047291136 & 92.58065 & 24.02085 & 2.13754 & 10.49 & 11.00 & 9.85 & 0.49 & 0.11 & G & 97.58 & 11.68 & 91.32 & 9.67 \\
4767484964954044544 & 87.95841 & -55.74149 & 2.16924 & 15.36 & 15.65 & 14.92 & 0.08 & 0.11 & G & 97.01 & 11.62 & 90.14 & 9.55 \\
4690719846243518208 & 18.54532 & -70.98892 & 2.17640 & 15.99 & 16.23 & 15.61 & -0.0 & 0.11 & G & 96.88 & 11.60 & 88.62 & 9.39 \\
2930223059544294912 & 111.42332 & -19.89666 & 2.17773 & 11.21 & 11.76 & 10.53 & 0.61 & 0.09 & O & 96.86 & 11.60 & 88.63 & 9.39 \\
5611675694812770176 & 113.56309 & -28.62465 & 2.18938 & 12.97 & 13.51 & 12.28 & 0.58 & 0.12 & G & 96.66 & 11.57 & 90.02 & 9.54 \\
5251882921501101312 & 158.02003 & -63.67476 & 2.23584 & 15.84 & 16.21 & 15.26 & 0.32 & 0.11 & G & 95.86 & 11.48 & 87.96 & 9.32 \\
6057943520139661184 & 186.29705 & -61.34817 & 2.30569 & 9.77 & 10.32 & 9.10 & 0.55 & 0.11 & G & 94.70 & 11.34 & 88.80 & 9.41 \\
2949440564287527552 & 104.71105 & -13.73667 & 2.32596 & 11.92 & 12.50 & 11.21 & 0.63 & 0.12 & G & 94.37 & 11.30 & 87.94 & 9.31 \\
5877460679352962048 & 221.67487 & -61.46196 & 2.39812 & 7.29 & 7.73 & 6.70 & 0.35 & 0.06 & L & 93.23 & 11.16 & 87.93 & 9.31 \\
3157950918582624256 & 104.70966 & 9.62273 & 2.39815 & 9.23 & 9.55 & 8.78 & 0.14 & 0.03 & L & 93.23 & 11.16 & 85.22 & 9.03 \\
4650132886338231296 & 88.06762 & -74.12767 & 2.42105 & 15.93 & 16.28 & 15.49 & 0.09 & 0.11 & G & 92.88 & 11.12 & 87.62 & 9.28 \\
5824226655600824704 & 232.70754 & -65.59936 & 2.42829 & 7.58 & 8.02 & 7.02 & 0.26 & 0.1 & L & 92.77 & 11.11 & 89.97 & 9.53 \\
5257722221591844480 & 147.63941 & -58.85915 & 2.44212 & 14.62 & 15.51 & 13.66 & 1.21 & 0.14 & G & 92.56 & 11.08 & 84.57 & 8.96 \\
5241536688894529408 & 162.42510 & -62.63364 & 2.47137 & 14.52 & 15.25 & 13.62 & 1.0 & 0.11 & O & 92.13 & 11.03 & 83.95 & 8.89 \\
5311598634949142400 & 139.31963 & -53.08485 & 2.48165 & 10.41 & 10.92 & 9.76 & 0.38 & 0.05 & L & 91.98 & 11.01 & 91.39 & 9.68 \\
5546003793739552896 & 119.74495 & -34.07069 & 2.48812 & 14.64 & 15.52 & 13.68 & 1.18 & 0.12 & O & 91.88 & 11.00 & 84.50 & 8.95 \\
3028237786647550464 & 112.35338 & -15.97682 & 2.50363 & 12.77 & 13.68 & 11.82 & 1.11 & 0.12 & O & 91.66 & 10.97 & 88.66 & 9.39 \\
5930952980798060032 & 250.81165 & -52.27422 & 2.53380 & 15.74 & 16.44 & 14.89 & 0.9 & 0.13 & G & 91.22 & 10.92 & 83.49 & 8.84 \\
3027132189042054400 & 114.83954 & -17.34696 & 2.59875 & 10.76 & 11.24 & 10.12 & 0.45 & 0.11 & G & 90.31 & 10.81 & 83.88 & 8.88 \\
5614274807174596864 & 115.45717 & -25.04177 & 2.62584 & 10.35 & 10.87 & 9.70 & 0.42 & 0.05 & L & 89.94 & 10.77 & 87.27 & 9.24 \\
5718755624717348096 & 116.00252 & -17.12887 & 2.62974 & 11.30 & 11.69 & 10.76 & 0.25 & 0.11 & G & 89.89 & 10.76 & 83.45 & 8.84 \\
5525825109665030528 & 132.70396 & -39.44449 & 2.63045 & 12.64 & 13.53 & 11.71 & 1.16 & 0.14 & G & 89.88 & 10.76 & 82.77 & 8.77 \\
3350719221309022720 & 101.47216 & 10.06146 & 2.64460 & 10.41 & 10.92 & 9.75 & 0.5 & 0.11 & G & 89.69 & 10.74 & 83.13 & 8.80 \\
5594180167020044544 & 120.11432 & -33.31980 & 2.65696 & 12.94 & 13.58 & 12.16 & 0.84 & 0.1 & O & 89.52 & 10.72 & 78.08 & 8.27 \\
4684364458577939328 & 12.41486 & -76.07638 & 2.65759 & 15.75 & 15.99 & 15.31 & 0.03 & 0.11 & G & 89.52 & 10.72 & 81.23 & 8.60 \\
3112550812164329856 & 105.47340 & -1.13095 & 2.67492 & 8.43 & 8.79 & 7.94 & 0.12 & 0.02 & L & 89.29 & 10.69 & 85.11 & 9.01 \\
5598174486604978176 & 116.20151 & -31.36252 & 2.69267 & 13.83 & 14.71 & 12.89 & 1.14 & 0.14 & G & 89.05 & 10.66 & 81.75 & 8.66 \\
5547538196579026816 & 122.56082 & -32.89204 & 2.71935 & 12.80 & 13.69 & 11.86 & 1.14 & 0.12 & O & 88.71 & 10.62 & 82.23 & 8.71 \\
4513544886184515584 & 286.95604 & 16.95625 & 2.72920 & 14.44 & 15.17 & 13.60 & 0.9 & 0.13 & G & 88.58 & 10.61 & 81.69 & 8.65 \\
3105345570728492416 & 101.18311 & -3.95240 & 2.77475 & 11.39 & 12.04 & 10.62 & 0.72 & 0.09 & L & 88.00 & 10.54 & 82.06 & 8.69 \\
3107234707804768384 & 100.46536 & -1.33498 & 2.79810 & 11.82 & 12.42 & 11.08 & 0.65 & 0.12 & G & 87.71 & 10.50 & 81.31 & 8.61 \\
2007654601080023040 & 338.42226 & 57.31830 & 2.80533 & 9.12 & 9.68 & 8.43 & 0.59 & 0.08 & L & 87.62 & 10.49 & 79.96 & 8.47 \\
3398143803515552768 & 88.22807 & 18.01082 & 2.81521 & 12.22 & 12.85 & 11.47 & 0.69 & 0.12 & G & 87.50 & 10.48 & 81.31 & 8.61 \\
425324052915862912 & 10.09664 & 58.61852 & 2.82322 & 13.03 & 13.55 & 12.34 & 0.44 & 0.06 & L & 87.40 & 10.46 & 84.36 & 8.94 \\
429182376660681984 & 3.16670 & 60.22643 & 2.84185 & 9.90 & 10.50 & 9.18 & 0.62 & 0.12 & G & 87.17 & 10.44 & 81.18 & 8.60 \\
5598479085688742656 & 115.17910 & -30.71466 & 2.89019 & 12.54 & 13.01 & 11.89 & 0.43 & 0.11 & G & 86.59 & 10.37 & 79.89 & 8.46 \\
4319599865468760832 & 290.79264 & 13.85664 & 2.97303 & 10.15 & 11.24 & 9.14 & 1.41 & 0.16 & G & 85.63 & 10.25 & 78.91 & 8.36 \\
468646563398354176 & 61.61184 & 56.38261 & 2.99120 & 10.78 & 11.50 & 9.96 & 0.83 & 0.13 & G & 85.42 & 10.23 & 79.27 & 8.40 \\
6703004658279987200 & 272.40289 & -50.27762 & 3.01343 & 11.87 & 12.90 & 10.88 & 1.32 & 0.15 & G & 85.17 & 10.20 & 78.61 & 8.33 \\
2008577744163053696 & 341.59050 & 59.95872 & 3.02796 & 11.06 & 11.96 & 10.12 & 1.16 & 0.14 & G & 85.01 & 10.18 & 77.94 & 8.26 \\
5258420858142702208 & 152.56700 & -58.18688 & 3.03785 & 9.12 & 9.61 & 8.50 & 0.39 & 0.11 & G & 84.90 & 10.17 & 79.19 & 8.39 \\
3121755094578376832 & 95.20696 & 0.04161 & 3.03825 & 11.65 & 12.29 & 10.88 & 0.71 & 0.12 & G & 84.89 & 10.16 & 78.51 & 8.32 \\
2200929331984972672 & 337.77214 & 60.26569 & 3.05313 & 10.87 & 11.74 & 9.96 & 1.07 & 0.14 & G & 84.73 & 10.15 & 78.46 & 8.31 \\
5848500161483878400 & 222.62620 & -67.49763 & 3.06525 & 7.10 & 7.64 & 6.44 & 0.5 & 0.04 & L & 84.60 & 10.13 & 77.87 & 8.25 \\
4156512638614879104 & 279.16501 & -8.18483 & 3.09090 & 9.62 & 10.40 & 8.79 & 0.84 & 0.07 & L & 84.32 & 10.10 & 81.03 & 8.58 \\
3050824676059815168 & 104.89544 & -8.37710 & 3.10304 & 13.30 & 14.21 & 12.34 & 1.18 & 0.14 & G & 84.19 & 10.08 & 76.80 & 8.13 \\
5613541295473114496 & 111.61767 & -25.92677 & 3.12653 & 8.99 & 9.63 & 8.26 & 0.6 & 0.05 & L & 83.94 & 10.05 & 80.32 & 8.51 \\
3356119713188276096 & 98.47754 & 14.47138 & 3.13632 & 10.38 & 10.98 & 9.67 & 0.59 & 0.05 & L & 83.83 & 10.04 & 78.02 & 8.26 \\
3409635486731094400 & 69.31155 & 18.54301 & 3.14835 & 6.23 & 6.75 & 5.59 & 0.41 & 0.04 & L & 83.71 & 10.02 & 78.87 & 8.35 \\
2953155500537706752 & 102.77785 & -11.33744 & 3.15452 & 13.27 & 14.17 & 12.31 & 1.17 & 0.14 & G & 83.64 & 10.01 & 76.21 & 8.07 \\
1833295112309561344 & 300.69070 & 23.27608 & 3.16429 & 13.11 & 13.99 & 12.19 & 1.1 & 0.14 & G & 83.54 & 10.00 & 76.66 & 8.12 \\
5334449269746243328 & 171.30404 & -61.36915 & 3.21183 & 8.42 & 8.81 & 7.89 & 0.22 & 0.02 & L & 83.05 & 9.94 & 76.08 & 8.06 \\
4628830428362208512 & 61.12043 & -75.07970 & 3.21459 & 15.15 & 15.43 & 14.70 & 0.04 & 0.11 & G & 83.02 & 9.94 & 75.60 & 8.01 \\
511226491206912128 & 26.79965 & 61.42249 & 3.22284 & 9.83 & 10.65 & 8.96 & 1.03 & 0.09 & L & 82.93 & 9.93 & 74.89 & 7.93 \\
6387986571094721280 & 353.32270 & -67.76696 & 3.23536 & 15.51 & 15.74 & 15.11 & 0.0 & 0.11 & G & 82.81 & 9.91 & 72.75 & 7.71 \\
4650239813843637248 & 86.77105 & -73.41004 & 3.24359 & 15.50 & 15.85 & 14.98 & 0.17 & 0.11 & G & 82.72 & 9.90 & 75.99 & 8.05 \\
3049261303661303552 & 103.66285 & -10.91295 & 3.25924 & 12.36 & 13.14 & 11.49 & 0.95 & 0.13 & G & 82.57 & 9.89 & 75.67 & 8.01 \\
2952531635068093952 & 100.53995 & -12.66113 & 3.26141 & 11.41 & 11.92 & 10.75 & 0.46 & 0.11 & G & 82.55 & 9.88 & 76.42 & 8.09 \\
5614701001056464384 & 116.11513 & -24.28858 & 3.27320 & 12.50 & 13.21 & 11.69 & 0.86 & 0.11 & O & 82.43 & 9.87 & 73.65 & 7.80 \\
1971722045688053248 & 320.13710 & 45.46749 & 3.28391 & 8.67 & 9.33 & 7.92 & 0.7 & 0.06 & L & 82.32 & 9.86 & 76.18 & 8.07 \\
514736269771300224 & 33.88110 & 63.51778 & 3.29886 & 10.32 & 11.00 & 9.53 & 0.75 & 0.12 & G & 82.17 & 9.84 & 76.18 & 8.07 \\
5593427031607304704 & 112.12402 & -30.65555 & 3.30515 & 12.05 & 12.45 & 11.51 & 0.22 & 0.11 & G & 82.11 & 9.83 & 75.79 & 8.03 \\
5336579363014965376 & 171.69650 & -58.81950 & 3.32711 & 12.88 & 13.51 & 12.10 & 0.72 & 0.1 & O & 81.90 & 9.81 & 74.29 & 7.87 \\
5960623272099513856 & 264.40651 & -40.81355 & 3.38020 & 7.05 & 7.51 & 6.12 & 0.34 & 0.04 & L & 81.38 & 9.74 & 91.65 & 9.71 \\
5255209665741407744 & 156.49253 & -59.94550 & 3.39566 & 10.75 & 11.38 & 9.99 & 0.66 & 0.12 & G & 81.24 & 9.73 & 75.17 & 7.96 \\
3027746854704868608 & 111.98560 & -16.83151 & 3.39628 & 10.85 & 11.65 & 9.98 & 0.95 & 0.13 & G & 81.23 & 9.73 & 75.14 & 7.96 \\
5347071319596612864 & 167.83483 & -54.55701 & 3.52731 & 7.78 & 8.12 & 7.32 & 0.07 & 0.11 & G & 80.02 & 9.58 & 74.16 & 7.85 \\
2935055065243490048 & 107.71609 & -16.73962 & 3.64877 & 11.94 & 12.55 & 11.19 & 0.63 & 0.12 & G & 78.96 & 9.45 & 72.78 & 7.71 \\
429635993926502912 & 2.46412 & 61.51404 & 3.65163 & 10.44 & 11.33 & 9.53 & 1.36 & 0.18 & L & 78.93 & 9.45 & 61.44 & 6.51 \\
4237423603350413568 & 300.63619 & 0.71388 & 3.76719 & 10.95 & 11.38 & 10.38 & 0.25 & 0.11 & G & 77.96 & 9.34 & 72.10 & 7.64 \\
5932565900081831040 & 242.83526 & -54.35413 & 3.78678 & 8.58 & 9.10 & 7.93 & 0.39 & 0.04 & L & 77.80 & 9.32 & 73.25 & 7.76 \\
5836231845180574592 & 240.40305 & -56.18477 & 3.79369 & 15.02 & 15.94 & 14.05 & 1.19 & 0.12 & O & 77.75 & 9.31 & 70.01 & 7.41 \\
2246124001521354368 & 310.79959 & 67.24650 & 3.92667 & 12.35 & 12.87 & 11.70 & 0.42 & 0.11 & G & 76.69 & 9.18 & 70.87 & 7.51 \\
2006085421882734336 & 333.44753 & 55.41078 & 3.98692 & 12.18 & 12.95 & 11.32 & 0.89 & 0.13 & G & 76.23 & 9.13 & 69.73 & 7.39 \\
5334591003669216000 & 178.38968 & -62.85220 & 3.99765 & 9.72 & 10.32 & 9.02 & 0.51 & 0.07 & L & 76.15 & 9.12 & 71.80 & 7.61 \\
4664274255137737984 & 77.76935 & -63.43402 & 4.03938 & 15.80 & 16.14 & 15.30 & 0.1 & 0.11 & G & 75.84 & 9.08 & 69.39 & 7.35 \\
4649907692617316480 & 76.13718 & -73.15621 & 4.09895 & 15.02 & 15.35 & 14.54 & 0.06 & 0.11 & G & 75.40 & 9.03 & 68.84 & 7.29 \\
5310680130430560768 & 139.02433 & -54.30973 & 4.11692 & 11.01 & 11.52 & 10.36 & 0.4 & 0.11 & G & 75.27 & 9.01 & 69.45 & 7.36 \\
6060761362259462528 & 189.78014 & -58.28456 & 4.25428 & 12.83 & 13.44 & 12.07 & 0.62 & 0.12 & G & 74.30 & 8.90 & 67.77 & 7.18 \\
428839329030983040 & 6.64980 & 60.79817 & 4.30649 & 8.68 & 9.37 & 7.90 & 0.81 & 0.1 & L & 73.94 & 8.85 & 64.18 & 6.80 \\
5254916611530412672 & 154.36075 & -60.33320 & 4.31079 & 13.77 & 14.52 & 12.85 & 0.99 & 0.11 & O & 73.91 & 8.85 & 64.84 & 6.87 \\
5881995546318024704 & 232.96911 & -59.24980 & 4.37292 & 8.65 & 9.30 & 7.92 & 0.61 & 0.12 & G & 73.49 & 8.80 & 68.07 & 7.21 \\
5339554336583678464 & 168.50011 & -57.91090 & 4.43091 & 8.09 & 8.52 & 7.54 & 0.24 & 0.02 & L & 73.11 & 8.75 & 66.21 & 7.01 \\
5715901567412202496 & 117.25952 & -19.11357 & 4.64442 & 9.52 & 10.00 & 8.90 & 0.32 & 0.11 & G & 71.76 & 8.59 & 66.11 & 7.00 \\
5718760258978008320 & 116.04965 & -17.08099 & 4.70117 & 10.04 & 10.50 & 9.45 & 0.28 & 0.11 & G & 71.42 & 8.55 & 65.71 & 6.96 \\
1965135696153566336 & 319.08500 & 38.92738 & 4.74035 & 9.51 & 9.95 & 8.93 & 0.25 & 0.11 & G & 71.18 & 8.52 & 65.53 & 6.94 \\
3345254098763568768 & 92.59262 & 14.64450 & 4.83734 & 9.53 & 10.18 & 8.79 & 0.59 & 0.12 & G & 70.61 & 8.46 & 65.45 & 6.93 \\
5711201189563596416 & 119.24042 & -22.82542 & 4.86103 & 8.46 & 8.92 & 7.86 & 0.24 & 0.04 & L & 70.48 & 8.44 & 66.30 & 7.02 \\
2004036486267748352 & 342.26323 & 56.42820 & 5.44565 & 8.09 & 8.63 & 7.41 & 0.42 & 0.05 & L & 67.38 & 8.07 & 62.01 & 6.57 \\
2045359534871088384 & 294.54825 & 32.48955 & 5.57148 & 10.45 & 10.95 & 9.82 & 0.33 & 0.04 & L & 66.77 & 7.99 & 61.17 & 6.48 \\
5868451040512196224 & 202.88916 & -61.58237 & 5.62283 & 6.39 & 6.83 & 5.83 & 0.2 & 0.05 & L & 66.53 & 7.97 & 60.75 & 6.43 \\
5337634589276921856 & 167.68575 & -60.75027 & 5.72548 & 8.82 & 9.39 & 8.13 & 0.45 & 0.07 & L & 66.06 & 7.91 & 60.54 & 6.41 \\
\end{tabular}
\end{table}


==> tab_age_1.5_A_PA_PAC.tex <==
\begin{table}
\begin{tabular}{cccccccccccccc}
Gaia DR2 source Id & RA[deg] & DEC[deg] & P[d] & G[mag] & G_BP[mag] & G_RP[mag] & E(gbp-grb)[mag] & sigma_E(gbp-grb)[mag] & Note & t_pa[Myr] & sigma(t)_pa[Myr] & t_pac[Myr] & sigma(t)_pac[Myr] \\
3442172745919329664 & 82.35887 & 27.00089 & 3.34920 & 11.57 & 12.21 & 10.78 & 0.72 & 0.12 & G & 105.55 & 20.41 & 98.88 & 18.9 \\
4704080802304630784 & 12.82014 & -68.98430 & 0.99469 & 18.24 & 18.45 & 17.79 & 0.18 & 0.11 & G & 248.10 & 47.99 & 230.53 & 44.06 \\
5521400228203695232 & 123.35129 & -42.27568 & 1.00189 & 16.05 & 16.93 & 15.15 & 1.23 & 0.15 & G & 246.84 & 47.74 & 234.34 & 44.79 \\
6379351625245757568 & 359.99997 & -75.19496 & 1.03777 & 17.68 & 17.98 & 17.36 & 0.02 & 0.11 & G & 240.80 & 46.58 & 231.16 & 44.18 \\
4711142067840447360 & 21.61608 & -64.87535 & 1.06447 & 17.86 & 18.05 & 17.41 & 0.16 & 0.11 & G & 236.54 & 45.75 & 219.39 & 41.93 \\
4639539705975935360 & 50.85364 & -74.96868 & 1.11640 & 17.83 & 18.12 & 17.50 & 0.02 & 0.11 & G & 228.74 & 44.24 & 218.50 & 41.76 \\
4690768156035338624 & 18.95551 & -70.54573 & 1.14292 & 17.53 & 17.82 & 17.09 & 0.18 & 0.11 & G & 224.99 & 43.52 & 212.14 & 40.54 \\
4703965697180635136 & 9.31520 & -67.04117 & 1.15729 & 17.89 & 18.12 & 17.43 & 0.17 & 0.11 & G & 223.02 & 43.14 & 207.66 & 39.69 \\
4666616485480394368 & 60.40851 & -69.47789 & 1.15905 & 16.29 & 16.45 & 15.90 & 0.12 & 0.08 & O & 222.78 & 43.09 & 203.12 & 38.82 \\
4691081375113472256 & 20.83822 & -70.57775 & 1.17564 & 17.33 & 17.45 & 17.02 & 0.0 & 0.11 & G & 220.56 & 42.66 & 200.73 & 38.36 \\
4637614151878607232 & 20.74650 & -76.24745 & 1.20857 & 17.80 & 17.95 & 17.36 & 0.1 & 0.11 & G & 216.31 & 41.84 & 199.28 & 38.09 \\
5834840099568788864 & 241.98124 & -58.78225 & 1.23577 & 13.71 & 14.05 & 13.19 & 0.31 & 0.11 & G & 212.95 & 41.19 & 200.06 & 38.23 \\
4636112425153243904 & 16.19343 & -76.86050 & 1.25457 & 17.34 & 17.55 & 16.84 & 0.21 & 0.11 & G & 210.70 & 40.75 & 194.40 & 37.15 \\
4690721839108141568 & 19.01385 & -70.91305 & 1.30481 & 17.25 & 17.73 & 17.00 & -0.0 & 0.11 & G & 204.95 & 39.64 & 201.29 & 38.47 \\
4698739817197286912 & 23.24870 & -66.49795 & 1.30920 & 17.05 & 17.30 & 16.67 & 0.05 & 0.11 & G & 204.47 & 39.55 & 192.58 & 36.8 \\
5298606801235832064 & 140.10591 & -62.22648 & 1.36601 & 18.36 & 18.60 & 17.89 & 0.18 & 0.11 & G & 198.45 & 38.38 & 184.56 & 35.27 \\
5850083595712857472 & 220.66054 & -64.27433 & 1.37135 & 17.67 & 18.47 & 16.71 & 1.23 & 0.15 & G & 197.90 & 38.28 & 183.88 & 35.14 \\
4690414800484275840 & 12.25946 & -70.13797 & 1.37867 & 17.09 & 17.39 & 16.78 & -0.0 & 0.11 & G & 197.16 & 38.13 & 186.94 & 35.73 \\
5935901715187592704 & 255.13630 & -53.09007 & 1.39879 & 15.45 & 15.92 & 14.78 & 0.58 & 0.12 & G & 195.16 & 37.75 & 183.01 & 34.98 \\
5615958881027868544 & 115.24714 & -22.49207 & 1.39928 & 15.46 & 16.23 & 14.69 & 0.89 & 0.11 & O & 195.11 & 37.74 & 187.45 & 35.82 \\
4627114812265929856 & 55.76893 & -76.93405 & 1.42992 & 17.95 & 18.31 & 17.50 & 0.18 & 0.11 & G & 192.16 & 37.17 & 182.94 & 34.96 \\
4690838421706602624 & 15.93439 & -70.90033 & 1.43044 & 17.33 & 17.58 & 16.94 & 0.06 & 0.11 & G & 192.11 & 37.16 & 180.59 & 34.51 \\
4637822960304562560 & 24.11091 & -75.12545 & 1.43113 & 17.25 & 17.49 & 16.82 & 0.11 & 0.11 & G & 192.04 & 37.14 & 179.71 & 34.35 \\
6027070573648725632 & 251.47116 & -33.16585 & 1.45594 & 13.89 & 14.47 & 13.13 & 0.75 & 0.12 & G & 189.73 & 36.70 & 178.32 & 34.08 \\
5321579073778197888 & 130.00710 & -52.33019 & 1.53045 & 15.25 & 15.90 & 14.48 & 0.81 & 0.12 & G & 183.18 & 35.43 & 172.97 & 33.06 \\
6008381624727734784 & 237.76802 & -39.75981 & 1.57244 & 17.10 & 17.91 & 16.20 & 1.12 & 0.14 & G & 179.73 & 34.76 & 168.77 & 32.26 \\
4649187405119614848 & 75.03872 & -75.15255 & 1.57491 & 16.97 & 17.25 & 16.49 & 0.18 & 0.11 & G & 179.53 & 34.72 & 167.82 & 32.07 \\
4108167833903339520 & 259.75244 & -27.43467 & 1.58118 & 16.78 & 17.65 & 15.71 & 1.45 & 0.16 & G & 179.03 & 34.63 & 163.50 & 31.25 \\
4691023998645738368 & 17.49608 & -69.93794 & 1.60821 & 16.70 & 16.83 & 16.30 & 0.0 & 0.11 & G & 176.90 & 34.22 & 162.54 & 31.06 \\
4650261219962135424 & 85.33831 & -74.16668 & 1.62049 & 16.91 & 17.29 & 16.43 & 0.22 & 0.11 & G & 175.96 & 34.03 & 167.16 & 31.95 \\
426580107514101376 & 15.41660 & 60.59426 & 1.62477 & 14.87 & 15.52 & 14.07 & 0.85 & 0.13 & G & 175.63 & 33.97 & 164.77 & 31.49 \\
4684195339947360512 & 6.98869 & -76.24706 & 1.64272 & 17.58 & 17.86 & 17.10 & 0.17 & 0.11 & G & 174.28 & 33.71 & 162.87 & 31.13 \\
2031982665929461504 & 296.05399 & 29.68730 & 1.64410 & 16.22 & 17.13 & 15.31 & 1.2 & 0.14 & G & 174.18 & 33.69 & 164.77 & 31.49 \\
181620805307496192 & 76.98162 & 33.05659 & 1.66805 & 14.61 & 15.30 & 13.80 & 0.88 & 0.13 & G & 172.41 & 33.35 & 162.36 & 31.03 \\
4702506576531479424 & 12.34403 & -69.50825 & 1.68632 & 17.24 & 17.63 & 16.86 & 0.08 & 0.11 & G & 171.09 & 33.09 & 164.81 & 31.5 \\
2021540814501736320 & 293.71912 & 25.61797 & 1.69319 & 17.40 & 18.66 & 16.25 & 1.87 & 0.19 & G & 170.60 & 33.00 & 157.51 & 30.1 \\
4684369749977673472 & 13.14590 & -75.95877 & 1.75282 & 17.35 & 17.52 & 16.89 & 0.09 & 0.11 & G & 166.50 & 32.20 & 153.11 & 29.26 \\
4392367984521092608 & 254.76077 & 4.79169 & 1.77576 & 14.89 & 15.22 & 14.38 & 0.23 & 0.11 & G & 164.98 & 31.91 & 154.50 & 29.53 \\
4652327614621999872 & 70.43479 & -74.41493 & 1.79655 & 16.84 & 16.86 & 16.26 & 0.21 & 0.11 & G & 163.63 & 31.65 & 144.51 & 27.62 \\
5516409029527928064 & 125.97858 & -47.25490 & 1.83399 & 15.20 & 15.90 & 14.37 & 0.91 & 0.13 & G & 161.28 & 31.19 & 151.29 & 28.91 \\
5814577169727787392 & 254.58683 & -67.66312 & 1.85575 & 13.93 & 14.19 & 13.51 & 0.06 & 0.11 & G & 159.94 & 30.94 & 149.78 & 28.63 \\
4189050211325803008 & 299.56897 & -12.07101 & 1.99398 & 17.75 & 18.07 & 17.21 & 0.24 & 0.11 & G & 152.05 & 29.41 & 141.93 & 27.12 \\
252595410453952384 & 67.62787 & 43.65313 & 1.99947 & 13.06 & 14.01 & 12.09 & 1.29 & 0.15 & G & 151.76 & 29.35 & 142.30 & 27.2 \\
5928285810456681344 & 247.54255 & -57.33140 & 2.00665 & 13.64 & 14.08 & 13.01 & 0.44 & 0.11 & G & 151.38 & 29.28 & 142.10 & 27.16 \\
5851830444814064512 & 206.04645 & -65.60886 & 2.02729 & 15.84 & 16.51 & 14.95 & 0.97 & 0.13 & G & 150.29 & 29.07 & 139.10 & 26.58 \\
2928096226097916160 & 109.16266 & -22.18043 & 2.04402 & 14.73 & 15.46 & 13.87 & 0.96 & 0.13 & G & 149.42 & 28.90 & 140.17 & 26.79 \\
5322875157471168768 & 129.59122 & -49.81203 & 2.04472 & 15.13 & 15.93 & 14.31 & 0.92 & 0.13 & G & 149.39 & 28.89 & 142.17 & 27.17 \\
5859972946880769408 & 189.52856 & -66.38308 & 2.06540 & 15.01 & 15.58 & 14.31 & 0.63 & 0.09 & O & 148.33 & 28.69 & 139.25 & 26.61 \\
4636099402811865344 & 19.45728 & -76.56544 & 2.06770 & 16.80 & 17.11 & 16.32 & 0.16 & 0.11 & G & 148.22 & 28.67 & 138.81 & 26.53 \\
6379917835078618752 & 359.03700 & -73.64989 & 2.08819 & 17.15 & 17.32 & 16.70 & 0.05 & 0.11 & G & 147.19 & 28.47 & 135.36 & 25.87 \\
5211831178906807040 & 93.60903 & -79.18168 & 2.09182 & 16.74 & 16.98 & 16.24 & 0.15 & 0.11 & G & 147.01 & 28.43 & 136.03 & 26.0 \\
2162679246615275264 & 315.66755 & 45.09280 & 2.11305 & 16.28 & 17.23 & 15.27 & 1.34 & 0.15 & G & 145.97 & 28.23 & 135.76 & 25.95 \\
200016111582079744 & 73.82548 & 39.97972 & 2.12061 & 13.35 & 13.95 & 12.58 & 0.73 & 0.08 & L & 145.60 & 28.16 & 136.31 & 26.05 \\
5613411827982576768 & 112.81549 & -25.90739 & 2.14810 & 11.58 & 12.04 & 10.97 & 0.29 & 0.08 & O & 144.29 & 27.91 & 140.62 & 26.88 \\
5256605839340504576 & 149.84616 & -60.33354 & 2.30293 & 14.62 & 15.23 & 13.86 & 0.71 & 0.12 & G & 137.39 & 26.57 & 129.19 & 24.69 \\
228673477705878400 & 63.37936 & 41.31878 & 2.31244 & 14.04 & 14.74 & 13.23 & 0.85 & 0.13 & G & 136.99 & 26.50 & 128.88 & 24.63 \\
6377896696484508544 & 355.61170 & -75.25641 & 2.33045 & 17.06 & 17.34 & 16.70 & -0.0 & 0.11 & G & 136.25 & 26.35 & 127.20 & 24.31 \\
5521137101325930624 & 122.45845 & -43.97272 & 2.34215 & 14.33 & 14.88 & 13.65 & 0.56 & 0.11 & G & 135.77 & 26.26 & 128.02 & 24.47 \\
5521712145909463680 & 128.16223 & -46.79047 & 2.36600 & 15.36 & 16.18 & 14.36 & 1.23 & 0.15 & G & 134.80 & 26.07 & 124.09 & 23.72 \\
5534744416711687424 & 119.86019 & -40.02830 & 2.36819 & 14.81 & 15.55 & 13.92 & 0.99 & 0.13 & G & 134.71 & 26.06 & 125.47 & 23.98 \\
4688062360997085440 & 21.38773 & -70.75956 & 2.37759 & 16.60 & 17.05 & 16.33 & 0.0 & 0.11 & G & 134.34 & 25.98 & 128.20 & 24.5 \\
5310255272261039488 & 138.08441 & -55.23391 & 2.39764 & 14.44 & 15.10 & 13.65 & 0.79 & 0.12 & G & 133.55 & 25.83 & 125.42 & 23.97 \\
3134002107923090944 & 101.39057 & 7.81629 & 2.42684 & 12.82 & 13.74 & 12.10 & 0.88 & 0.11 & O & 132.41 & 25.61 & 127.43 & 24.35 \\
4445130042844217216 & 249.98383 & 7.67920 & 2.44837 & 15.83 & 16.15 & 15.32 & 0.18 & 0.11 & G & 131.59 & 25.45 & 122.86 & 23.48 \\
1865228537734352896 & 317.06710 & 32.74552 & 2.45861 & 14.11 & 14.56 & 13.50 & 0.39 & 0.11 & G & 131.21 & 25.38 & 123.36 & 23.58 \\
4650211741937480192 & 86.25630 & -73.56541 & 2.47100 & 16.37 & 16.64 & 15.80 & 0.23 & 0.11 & G & 130.74 & 25.29 & 120.43 & 23.02 \\
207722317998325632 & 80.88983 & 44.76008 & 2.47685 & 12.75 & 13.46 & 11.93 & 0.85 & 0.13 & G & 130.53 & 25.25 & 122.64 & 23.44 \\
523700107035878272 & 14.38545 & 63.15643 & 2.48837 & 13.96 & 14.89 & 13.01 & 1.22 & 0.14 & G & 130.10 & 25.16 & 122.04 & 23.32 \\
5596920115637629184 & 119.15388 & -30.95279 & 2.49448 & 13.91 & 14.77 & 12.99 & 1.15 & 0.12 & O & 129.88 & 25.12 & 120.27 & 22.99 \\
4757183606166564864 & 83.55789 & -63.16699 & 2.50146 & 16.10 & 16.40 & 15.61 & 0.14 & 0.11 & G & 129.62 & 25.07 & 121.19 & 23.16 \\
5329778887909167232 & 131.65005 & -46.52931 & 2.52412 & 15.66 & 16.74 & 14.60 & 1.51 & 0.16 & G & 128.80 & 24.91 & 119.65 & 22.87 \\
5520935444020919296 & 122.93820 & -44.17210 & 2.54078 & 14.99 & 15.78 & 14.08 & 1.05 & 0.14 & G & 128.20 & 24.80 & 119.35 & 22.81 \\
5613111347760892672 & 110.69908 & -26.71455 & 2.54548 & 12.91 & 13.38 & 12.29 & 0.4 & 0.11 & G & 128.04 & 24.76 & 120.37 & 23.0 \\
2934255449716149760 & 107.39410 & -18.56329 & 2.54653 & 13.25 & 14.02 & 12.37 & 0.99 & 0.13 & G & 128.00 & 24.76 & 119.57 & 22.85 \\
5520440663787736192 & 122.44604 & -45.35460 & 2.55121 & 15.84 & 16.42 & 15.08 & 0.69 & 0.12 & G & 127.84 & 24.73 & 119.47 & 22.83 \\
2932101334643047680 & 105.10347 & -20.43170 & 2.55778 & 12.65 & 13.15 & 11.98 & 0.36 & 0.05 & L & 127.60 & 24.68 & 124.36 & 23.77 \\
470144751068871808 & 61.63394 & 58.11309 & 2.57812 & 16.51 & 16.97 & 15.88 & 0.42 & 0.11 & G & 126.89 & 24.54 & 119.01 & 22.74 \\
5597352047599988352 & 119.45786 & -29.38405 & 2.58612 & 11.59 & 12.21 & 10.84 & 0.73 & 0.1 & O & 126.62 & 24.49 & 117.57 & 22.47 \\
5404862853352596736 & 149.21983 & -51.60892 & 2.60474 & 13.30 & 14.09 & 12.41 & 1.0 & 0.11 & O & 125.98 & 24.37 & 118.31 & 22.61 \\
5599566983722741248 & 114.47706 & -29.43804 & 2.62004 & 14.18 & 14.88 & 13.38 & 0.81 & 0.12 & G & 125.46 & 24.27 & 118.10 & 22.57 \\
5617745003304609536 & 109.88037 & -23.80181 & 2.63003 & 14.53 & 15.53 & 13.52 & 1.35 & 0.15 & G & 125.13 & 24.20 & 116.71 & 22.3 \\
2004103831357741696 & 332.32734 & 51.40539 & 2.63200 & 14.84 & 15.40 & 14.13 & 0.59 & 0.12 & G & 125.06 & 24.19 & 117.42 & 22.44 \\
3425576270732293632 & 93.99953 & 23.74749 & 2.63501 & 11.57 & 12.24 & 10.79 & 0.75 & 0.1 & L & 124.96 & 24.17 & 118.22 & 22.59 \\
4690127037676227840 & 13.29901 & -70.85695 & 2.63769 & 16.20 & 16.67 & 15.89 & 0.0 & 0.11 & G & 124.87 & 24.15 & 120.72 & 23.07 \\
5254994264542210560 & 153.53708 & -59.85044 & 2.64145 & 15.11 & 15.96 & 14.18 & 1.08 & 0.12 & O & 124.74 & 24.13 & 117.65 & 22.48 \\
5932284528150696704 & 245.22589 & -53.55461 & 2.64407 & 11.70 & 11.99 & 11.25 & 0.03 & 0.08 & O & 124.66 & 24.11 & 118.10 & 22.57 \\
5857845872913577856 & 199.32909 & -66.11714 & 2.65755 & 15.60 & 16.34 & 14.72 & 0.96 & 0.13 & G & 124.21 & 24.02 & 115.98 & 22.17 \\
198681686717279616 & 72.85353 & 38.18855 & 2.65963 & 13.15 & 13.88 & 12.23 & 0.78 & 0.07 & L & 124.14 & 24.01 & 122.82 & 23.47 \\
5322962499927658880 & 129.02740 & -49.26527 & 2.66635 & 14.82 & 15.62 & 13.88 & 1.1 & 0.14 & G & 123.92 & 23.97 & 114.90 & 21.96 \\
3330259852538068608 & 91.85611 & 11.15198 & 3.88939 & 11.07 & 11.64 & 10.37 & 0.5 & 0.06 & L & 95.00 & 18.37 & 89.84 & 17.17 \\
5611563995612988928 & 112.16780 & -29.34422 & 2.70160 & 12.72 & 13.13 & 12.17 & 0.27 & 0.11 & G & 122.78 & 23.75 & 115.58 & 22.09 \\
3133819112256378368 & 100.02326 & 7.60583 & 2.70467 & 10.13 & 10.86 & 9.35 & 0.74 & 0.08 & L & 122.69 & 23.73 & 117.87 & 22.53 \\
5515778734493663232 & 127.31510 & -46.74924 & 2.71653 & 14.80 & 15.48 & 13.93 & 0.9 & 0.13 & G & 122.31 & 23.66 & 113.59 & 21.71 \\
4688033735040263168 & 23.36268 & -70.67097 & 2.74408 & 16.45 & 16.67 & 16.04 & -0.0 & 0.11 & G & 121.44 & 23.49 & 112.23 & 21.45 \\
5280590173638560128 & 104.74084 & -68.31085 & 2.75554 & 15.96 & 16.28 & 15.44 & 0.17 & 0.11 & G & 121.09 & 23.42 & 112.95 & 21.59 \\
355488086540394112 & 35.70997 & 50.07193 & 2.75989 & 14.54 & 14.96 & 13.95 & 0.32 & 0.11 & G & 120.95 & 23.39 & 113.44 & 21.68 \\
5520506531407532928 & 121.80022 & -45.06591 & 2.77254 & 14.02 & 14.57 & 13.29 & 0.6 & 0.12 & G & 120.56 & 23.32 & 112.83 & 21.56 \\
5545066700588440832 & 119.73893 & -36.89733 & 2.77514 & 15.07 & 16.06 & 14.05 & 1.35 & 0.15 & G & 120.48 & 23.30 & 112.11 & 21.43 \\
4637956099996538752 & 18.33566 & -75.37716 & 2.77979 & 16.46 & 16.76 & 15.98 & 0.11 & 0.11 & G & 120.34 & 23.28 & 112.29 & 21.46 \\
2948568273607650560 & 105.01213 & -14.16082 & 2.78195 & 13.90 & 14.80 & 13.11 & 0.91 & 0.13 & G & 120.28 & 23.26 & 115.97 & 22.16 \\
4066429066901946368 & 273.26040 & -23.11729 & 5.05787 & 6.82 & 7.37 & 6.23 & 0.25 & 0.03 & L & 78.96 & 15.27 & 76.16 & 14.56 \\
460909093912435072 & 42.02334 & 57.93448 & 2.79873 & 14.03 & 15.07 & 13.01 & 1.39 & 0.15 & G & 119.77 & 23.17 & 111.65 & 21.34 \\
430052537038350976 & 0.60589 & 62.84717 & 2.81345 & 14.41 & 15.25 & 13.49 & 1.08 & 0.14 & G & 119.33 & 23.08 & 111.62 & 21.33 \\
1873298884367855872 & 314.17890 & 40.25849 & 2.82245 & 16.21 & 17.13 & 15.23 & 1.25 & 0.15 & G & 119.06 & 23.03 & 110.80 & 21.18 \\
5616130129962210048 & 110.43814 & -26.53341 & 2.82545 & 12.91 & 13.38 & 12.30 & 0.37 & 0.11 & G & 118.97 & 23.01 & 112.02 & 21.41 \\
3117307814859500416 & 97.77268 & -2.14679 & 3.13523 & 13.29 & 14.09 & 12.47 & 0.9 & 0.12 & L & 110.57 & 21.39 & 104.02 & 19.88 \\
5293246995583678336 & 109.08524 & -60.30341 & 2.84929 & 15.52 & 16.19 & 14.69 & 0.83 & 0.13 & G & 118.27 & 22.87 & 110.27 & 21.07 \\
5544259212380322560 & 120.85675 & -37.19998 & 2.85529 & 14.09 & 14.84 & 13.23 & 0.93 & 0.11 & O & 118.09 & 22.84 & 110.08 & 21.04 \\
2928335747830554240 & 108.43497 & -21.72421 & 2.86166 & 14.22 & 14.98 & 13.36 & 0.94 & 0.13 & G & 117.91 & 22.81 & 110.57 & 21.13 \\
4757607983288353024 & 83.76190 & -62.33990 & 2.86849 & 16.03 & 16.25 & 15.52 & 0.12 & 0.11 & G & 117.71 & 22.77 & 108.11 & 20.66 \\
513074186146353536 & 24.74994 & 64.98924 & 2.87151 & 11.01 & 11.84 & 10.14 & 1.03 & 0.11 & L & 117.62 & 22.75 & 109.72 & 20.97 \\
4688114725237948672 & 24.52435 & -70.61840 & 2.88021 & 16.38 & 16.64 & 15.99 & -0.0 & 0.11 & G & 117.37 & 22.70 & 108.80 & 20.79 \\
261927068718088832 & 81.89283 & 50.86737 & 2.88526 & 13.17 & 13.81 & 12.41 & 0.7 & 0.12 & G & 117.23 & 22.67 & 110.22 & 21.06 \\
4682206533865906944 & 65.11048 & -57.85114 & 2.89258 & 15.71 & 16.00 & 15.30 & -0.0 & 0.11 & G & 117.02 & 22.63 & 110.03 & 21.03 \\
5253289093802878592 & 152.85139 & -61.48616 & 2.91146 & 14.11 & 14.59 & 13.44 & 0.46 & 0.11 & G & 116.48 & 22.53 & 109.01 & 20.83 \\
2947842664653933824 & 104.19146 & -15.63763 & 3.69400 & 13.25 & 13.97 & 12.43 & 0.81 & 0.12 & G & 98.51 & 19.05 & 92.36 & 17.65 \\
5310969267622303872 & 136.56210 & -54.93719 & 2.92762 & 14.52 & 15.11 & 13.78 & 0.63 & 0.12 & G & 116.03 & 22.44 & 108.96 & 20.82 \\
4642866828161408512 & 52.89342 & -70.99389 & 2.92900 & 16.29 & 16.60 & 15.82 & 0.08 & 0.11 & G & 115.99 & 22.43 & 108.83 & 20.8 \\
5533064637824258816 & 119.78798 & -43.17517 & 2.92921 & 13.49 & 13.98 & 12.84 & 0.45 & 0.11 & G & 115.99 & 22.43 & 108.97 & 20.82 \\
5598642947280233984 & 116.71718 & -30.66590 & 2.96840 & 14.15 & 14.95 & 13.28 & 0.97 & 0.11 & O & 114.91 & 22.22 & 107.76 & 20.59 \\
5856662557855409280 & 187.47093 & -68.27871 & 2.98190 & 14.44 & 14.92 & 13.79 & 0.44 & 0.11 & G & 114.54 & 22.15 & 107.43 & 20.53 \\
5318708901756763520 & 131.02834 & -51.91945 & 2.98495 & 15.08 & 15.82 & 14.23 & 0.89 & 0.13 & G & 114.46 & 22.14 & 107.38 & 20.52 \\
4265371574109405824 & 284.35111 & -0.73024 & 2.98806 & 10.56 & 11.32 & 9.69 & 0.99 & 0.14 & L & 114.37 & 22.12 & 105.79 & 20.22 \\
5519861423017907840 & 124.43265 & -45.18550 & 3.00610 & 14.46 & 15.24 & 13.61 & 0.93 & 0.13 & G & 113.89 & 22.03 & 107.23 & 20.49 \\
5241937353463150848 & 162.59092 & -62.19142 & 3.02574 & 15.21 & 16.09 & 14.26 & 1.16 & 0.12 & O & 113.37 & 21.93 & 105.26 & 20.12 \\
466906311366699520 & 48.44587 & 63.34948 & 3.03268 & 13.18 & 14.11 & 12.24 & 1.17 & 0.14 & G & 113.19 & 21.89 & 106.22 & 20.3 \\
5252269709082759936 & 156.40361 & -62.55651 & 3.04556 & 15.10 & 15.67 & 14.35 & 0.64 & 0.12 & G & 112.85 & 21.83 & 105.32 & 20.13 \\
5310863370918375552 & 140.55281 & -53.06412 & 3.05163 & 13.60 & 14.46 & 12.66 & 1.11 & 0.12 & O & 112.69 & 21.80 & 105.41 & 20.14 \\
5863815636949490048 & 202.86552 & -65.32720 & 3.06221 & 15.68 & 16.55 & 14.75 & 1.08 & 0.12 & O & 112.42 & 21.74 & 106.26 & 20.31 \\
2930525287803260288 & 109.84202 & -19.54033 & 3.07149 & 12.79 & 13.35 & 12.07 & 0.57 & 0.09 & O & 112.18 & 21.70 & 105.38 & 20.14 \\
5858259014403682304 & 195.97407 & -66.33292 & 3.08394 & 15.37 & 16.09 & 14.47 & 0.95 & 0.11 & O & 111.86 & 21.64 & 103.91 & 19.86 \\
5235910694044165760 & 176.13694 & -67.30525 & 3.08613 & 8.70 & 9.22 & 8.06 & 0.43 & 0.06 & L & 111.80 & 21.62 & 105.46 & 20.16 \\
5237406545247540608 & 171.64645 & -65.58218 & 3.11677 & 14.99 & 15.84 & 14.04 & 1.12 & 0.14 & G & 111.03 & 21.47 & 103.25 & 19.73 \\
5335753015664095104 & 173.80588 & -60.91465 & 3.12750 & 14.19 & 14.98 & 13.30 & 1.0 & 0.11 & O & 110.76 & 21.42 & 103.37 & 19.76 \\
5594991812757424768 & 115.97856 & -32.50378 & 3.14920 & 14.81 & 15.79 & 13.80 & 1.33 & 0.15 & G & 110.22 & 21.32 & 102.23 & 19.54 \\
2932737092877188352 & 105.22172 & -19.45929 & 3.15504 & 12.36 & 12.85 & 11.73 & 0.4 & 0.11 & G & 110.08 & 21.29 & 103.74 & 19.83 \\
2059517087110475392 & 299.88745 & 36.02152 & 3.16632 & 15.16 & 16.04 & 14.20 & 1.16 & 0.14 & G & 109.80 & 21.24 & 102.08 & 19.51 \\
5329323277776517120 & 130.36480 & -47.64966 & 3.17573 & 14.05 & 14.90 & 13.10 & 1.13 & 0.14 & G & 109.57 & 21.19 & 101.81 & 19.46 \\
5239658688657671680 & 160.70962 & -65.55805 & 3.18304 & 16.74 & 17.37 & 16.02 & 0.6 & 0.12 & G & 109.40 & 21.16 & 103.55 & 19.79 \\
5322878146768508800 & 129.73194 & -49.77016 & 3.18474 & 14.62 & 15.39 & 13.75 & 0.94 & 0.13 & G & 109.35 & 21.15 & 102.37 & 19.56 \\
5612661716228387200 & 111.62263 & -27.92502 & 3.18518 & 12.78 & 13.26 & 12.14 & 0.41 & 0.11 & G & 109.34 & 21.15 & 102.75 & 19.64 \\
377753613615880832 & 14.89365 & 45.40672 & 3.20017 & 11.48 & 11.87 & 10.98 & 0.16 & 0.11 & G & 108.98 & 21.08 & 102.94 & 19.67 \\
5875602191067578752 & 230.82679 & -61.21710 & 3.23038 & 15.66 & 16.48 & 14.71 & 1.1 & 0.14 & G & 108.26 & 20.94 & 100.28 & 19.17 \\
512491028363231616 & 24.35667 & 63.69136 & 3.23980 & 13.13 & 14.16 & 12.13 & 1.33 & 0.15 & G & 108.04 & 20.90 & 100.93 & 19.29 \\
4513100717859042176 & 286.49619 & 16.09800 & 3.26984 & 13.47 & 14.24 & 12.60 & 0.93 & 0.13 & G & 107.34 & 20.76 & 100.65 & 19.23 \\
5617316606087829888 & 109.16777 & -24.50300 & 3.27499 & 12.80 & 13.31 & 12.13 & 0.47 & 0.11 & G & 107.22 & 20.74 & 100.60 & 19.23 \\
5520505328816739584 & 121.80935 & -45.12830 & 3.28292 & 13.45 & 14.07 & 12.67 & 0.69 & 0.12 & G & 107.04 & 20.70 & 100.13 & 19.14 \\
5241803217391469568 & 165.52136 & -62.28989 & 3.28899 & 14.54 & 15.40 & 13.59 & 1.1 & 0.12 & O & 106.90 & 20.68 & 100.11 & 19.13 \\
279382060625871360 & 76.63188 & 55.35352 & 3.29487 & 7.19 & 7.81 & 6.48 & 0.55 & 0.07 & L & 106.77 & 20.65 & 102.22 & 19.54 \\
5405496240766414464 & 148.01595 & -51.99247 & 3.29644 & 13.56 & 14.38 & 12.67 & 1.01 & 0.11 & O & 106.73 & 20.64 & 99.63 & 19.04 \\
505178760644698880 & 31.25913 & 57.14294 & 3.29700 & 12.34 & 12.82 & 11.68 & 0.35 & 0.05 & L & 106.72 & 20.64 & 102.14 & 19.52 \\
5306043592977093504 & 145.89770 & -57.23830 & 3.00860 & 15.29 & 16.16 & 14.31 & 1.23 & 0.13 & O & 113.82 & 22.02 & 104.31 & 19.93 \\
505368121464666112 & 29.62897 & 57.81985 & 3.32910 & 13.78 & 14.44 & 12.98 & 0.74 & 0.12 & G & 105.99 & 20.50 & 99.42 & 19.0 \\
5600862070985787136 & 119.26547 & -28.16158 & 3.33098 & 11.61 & 12.25 & 10.88 & 0.58 & 0.09 & O & 105.95 & 20.49 & 101.70 & 19.44 \\
5605736961940589568 & 110.81312 & -29.72244 & 3.33617 & 12.87 & 13.38 & 12.30 & 0.3 & 0.11 & G & 105.84 & 20.47 & 100.86 & 19.28 \\
5313250548085699712 & 139.88405 & -51.62042 & 3.35503 & 12.70 & 13.62 & 11.69 & 1.34 & 0.13 & O & 105.42 & 20.39 & 95.64 & 18.28 \\
5516452460238707968 & 125.52706 & -47.30395 & 3.36831 & 14.28 & 14.93 & 13.46 & 0.77 & 0.12 & G & 105.12 & 20.33 & 98.08 & 18.75 \\
2073935223599391872 & 300.89457 & 39.15963 & 3.37031 & 13.22 & 13.96 & 12.38 & 1.02 & 0.13 & L & 105.08 & 20.32 & 94.39 & 18.04 \\
5592331544376193792 & 113.82822 & -31.66418 & 3.38307 & 13.77 & 14.53 & 12.93 & 0.87 & 0.13 & G & 104.80 & 20.27 & 98.67 & 18.86 \\
5824464493705913472 & 229.94041 & -66.49608 & 3.38932 & 6.44 & 6.86 & 5.91 & 0.23 & 0.04 & L & 104.66 & 20.24 & 98.41 & 18.81 \\
5598852026287511424 & 116.00045 & -30.14146 & 3.39082 & 13.12 & 13.66 & 12.45 & 0.58 & 0.09 & O & 104.63 & 20.24 & 95.93 & 18.33 \\
2025217890612425344 & 293.14591 & 26.80479 & 3.39154 & 15.51 & 16.38 & 14.54 & 1.15 & 0.14 & G & 104.62 & 20.23 & 96.98 & 18.53 \\
5857294605251013760 & 193.30159 & -67.96426 & 3.40117 & 14.41 & 14.91 & 13.73 & 0.48 & 0.11 & G & 104.41 & 20.19 & 97.69 & 18.67 \\
206211859601169792 & 74.06344 & 44.78185 & 3.40680 & 12.54 & 13.43 & 11.62 & 1.1 & 0.14 & G & 104.29 & 20.17 & 97.74 & 18.68 \\
189739251272296192 & 85.62191 & 37.64633 & 3.41272 & 12.05 & 12.93 & 11.18 & 0.84 & 0.11 & L & 104.16 & 20.15 & 103.05 & 19.69 \\
4690436069162376576 & 10.68389 & -70.27426 & 3.42463 & 16.23 & 16.48 & 15.74 & 0.07 & 0.11 & G & 103.90 & 20.10 & 96.22 & 18.39 \\
5932997939411720960 & 243.72813 & -53.33844 & 3.45291 & 9.79 & 10.63 & 8.92 & 0.92 & 0.08 & L & 103.30 & 19.98 & 98.50 & 18.82 \\
3051144427784813824 & 103.54766 & -7.66438 & 3.45403 & 13.28 & 13.98 & 12.44 & 0.85 & 0.11 & L & 103.28 & 19.98 & 96.08 & 18.36 \\
5547358117187868288 & 122.79503 & -33.51586 & 3.48218 & 10.44 & 11.05 & 9.72 & 0.58 & 0.06 & L & 102.69 & 19.86 & 97.06 & 18.55 \\
5310265099146146816 & 138.32401 & -54.93121 & 3.50424 & 14.23 & 15.01 & 13.34 & 0.96 & 0.13 & G & 102.24 & 19.77 & 95.53 & 18.26 \\
515527570241664512 & 34.14985 & 65.17655 & 3.52190 & 12.69 & 13.52 & 11.78 & 1.02 & 0.13 & G & 101.88 & 19.70 & 95.22 & 18.2 \\
2936165984303583360 & 105.87696 & -15.54334 & 3.52281 & 13.45 & 14.09 & 12.65 & 0.73 & 0.12 & G & 101.86 & 19.70 & 95.12 & 18.18 \\
5268616973048513664 & 107.46385 & -68.48372 & 3.52627 & 15.80 & 16.25 & 15.26 & 0.23 & 0.11 & G & 101.79 & 19.69 & 96.40 & 18.42 \\
5618354751226656640 & 112.51063 & -23.67398 & 3.54416 & 13.26 & 14.12 & 12.36 & 1.08 & 0.14 & L & 101.42 & 19.62 & 93.94 & 17.95 \\
5612495762995320576 & 113.72248 & -26.85579 & 3.55250 & 13.56 & 14.36 & 12.63 & 1.03 & 0.13 & G & 101.26 & 19.58 & 94.15 & 17.99 \\
5547421437881152256 & 122.36346 & -33.26212 & 3.56310 & 11.82 & 12.44 & 11.06 & 0.8 & 0.1 & O & 101.04 & 19.54 & 90.90 & 17.37 \\
2162640763705905920 & 316.08941 & 45.23937 & 3.56914 & 13.70 & 14.61 & 12.76 & 1.13 & 0.14 & G & 100.92 & 19.52 & 94.55 & 18.07 \\
5311139245252191616 & 137.38339 & -53.98770 & 3.59050 & 11.68 & 12.22 & 11.02 & 0.44 & 0.11 & G & 100.50 & 19.44 & 94.79 & 18.12 \\
5599370549100412544 & 114.32029 & -29.60773 & 3.59160 & 14.17 & 15.06 & 13.23 & 1.12 & 0.14 & G & 100.48 & 19.43 & 93.92 & 17.95 \\
2952257272558933248 & 101.92934 & -13.66668 & 4.85729 & 11.71 & 12.23 & 10.93 & 0.57 & 0.12 & G & 81.24 & 15.71 & 74.92 & 14.32 \\
3441484760885586176 & 86.43715 & 27.06790 & 3.62280 & 11.67 & 12.56 & 10.71 & 1.13 & 0.15 & L & 99.87 & 19.32 & 93.43 & 17.86 \\
429562773322439296 & 3.51343 & 60.98626 & 3.63045 & 11.91 & 12.73 & 11.01 & 0.99 & 0.13 & L & 99.72 & 19.29 & 93.81 & 17.93 \\
457807268533229056 & 38.46902 & 57.02750 & 3.64942 & 11.13 & 11.84 & 10.31 & 0.84 & 0.08 & L & 99.36 & 19.22 & 92.23 & 17.63 \\
5329405672431387648 & 130.00864 & -47.19842 & 3.67080 & 13.98 & 14.88 & 13.03 & 1.14 & 0.14 & G & 98.95 & 19.14 & 92.32 & 17.64 \\
5351721738384434048 & 157.29679 & -57.61339 & 3.68221 & 8.08 & 8.45 & 7.59 & 0.14 & 0.03 & L & 98.73 & 19.10 & 92.16 & 17.61 \\
5542528959037609984 & 127.24360 & -36.23207 & 3.70536 & 11.33 & 12.03 & 10.52 & 0.77 & 0.12 & G & 98.30 & 19.01 & 92.19 & 17.62 \\
5539023922122441728 & 118.71081 & -37.62246 & 3.70789 & 12.47 & 13.45 & 11.50 & 1.23 & 0.15 & G & 98.25 & 19.00 & 91.87 & 17.56 \\
4707044742055169152 & 9.21974 & -66.59323 & 3.72828 & 16.74 & 17.10 & 16.23 & 0.14 & 0.11 & G & 97.87 & 18.93 & 91.92 & 17.57 \\
2202500843341252736 & 328.64443 & 59.12168 & 3.75817 & 13.83 & 14.85 & 12.81 & 1.34 & 0.15 & G & 97.32 & 18.82 & 90.48 & 17.29 \\
2200018111723748224 & 335.91092 & 57.68078 & 3.76750 & 11.66 & 12.55 & 10.75 & 1.06 & 0.14 & L & 97.15 & 18.79 & 91.18 & 17.43 \\
3445039825569144192 & 86.71173 & 31.59791 & 3.04664 & 11.88 & 12.55 & 11.09 & 0.76 & 0.1 & L & 112.82 & 21.82 & 105.89 & 20.24 \\
3378049163365268608 & 100.78130 & 20.93911 & 3.78798 & 9.70 & 10.10 & 9.22 & 0.28 & 0.07 & L & 96.78 & 18.72 & 87.53 & 16.73 \\
5856994365517642112 & 194.75148 & -68.57855 & 3.79741 & 13.12 & 13.58 & 12.60 & 0.19 & 0.11 & G & 96.61 & 18.69 & 91.94 & 17.57 \\
5311409896910828800 & 137.14651 & -53.19702 & 3.80582 & 13.72 & 14.48 & 12.86 & 0.89 & 0.13 & G & 96.46 & 18.66 & 90.39 & 17.28 \\
430647231080076416 & 5.01280 & 63.17979 & 3.81071 & 11.68 & 12.53 & 10.74 & 1.01 & 0.13 & L & 96.38 & 18.64 & 91.53 & 17.49 \\
465719182408723072 & 41.18048 & 61.46470 & 3.83288 & 10.43 & 11.14 & 9.64 & 0.76 & 0.09 & L & 95.98 & 18.56 & 89.88 & 17.18 \\
6059635702888301952 & 190.35842 & -59.79419 & 3.83834 & 7.99 & 8.43 & 7.42 & 0.33 & 0.04 & L & 95.89 & 18.55 & 88.63 & 16.94 \\
509629965971797376 & 25.81989 & 59.99762 & 3.84314 & 12.33 & 13.18 & 11.42 & 1.02 & 0.13 & G & 95.80 & 18.53 & 89.65 & 17.13 \\
2031776202613700480 & 296.20306 & 29.26468 & 3.84599 & 6.69 & 7.01 & 6.22 & 0.17 & 0.04 & L & 95.75 & 18.52 & 86.84 & 16.6 \\
2012494342018730496 & 353.33454 & 61.11907 & 3.87118 & 12.21 & 13.18 & 11.23 & 1.22 & 0.14 & G & 95.31 & 18.44 & 88.94 & 17.0 \\
5619369359933924992 & 111.25618 & -23.15791 & 3.89113 & 13.75 & 14.75 & 12.76 & 1.26 & 0.15 & G & 94.97 & 18.37 & 88.60 & 16.93 \\
2072235820984829312 & 299.71473 & 37.64725 & 3.89187 & 14.29 & 14.88 & 13.51 & 0.67 & 0.12 & G & 94.96 & 18.37 & 88.26 & 16.87 \\
2072329902270080128 & 299.38702 & 38.09177 & 3.89671 & 13.59 & 14.22 & 12.81 & 0.68 & 0.12 & G & 94.87 & 18.35 & 88.62 & 16.94 \\
5335934297643679360 & 172.92831 & -60.73455 & 3.89770 & 13.14 & 13.88 & 12.32 & 0.78 & 0.1 & O & 94.86 & 18.35 & 89.85 & 17.17 \\
4253603501158148736 & 280.61175 & -5.34085 & 3.91771 & 10.51 & 11.41 & 9.60 & 1.05 & 0.1 & L & 94.52 & 18.28 & 89.21 & 17.05 \\
5615233993628681216 & 112.66125 & -24.68752 & 3.91882 & 13.09 & 13.87 & 12.21 & 0.91 & 0.11 & O & 94.50 & 18.28 & 88.92 & 16.99 \\
2010134274671099264 & 345.33801 & 57.86702 & 3.91921 & 11.49 & 12.30 & 10.62 & 0.92 & 0.12 & L & 94.49 & 18.28 & 89.18 & 17.04 \\
3052092481686246016 & 107.65830 & -7.12290 & 3.28782 & 12.52 & 13.23 & 11.64 & 0.68 & 0.09 & L & 106.93 & 20.68 & 105.65 & 20.19 \\
5540422122959807232 & 125.36087 & -38.42170 & 3.96098 & 12.55 & 13.54 & 11.57 & 1.22 & 0.13 & O & 93.79 & 18.14 & 87.96 & 16.81 \\
5606739884038472704 & 109.26954 & -28.82351 & 3.96993 & 12.72 & 13.24 & 12.05 & 0.45 & 0.11 & G & 93.64 & 18.11 & 87.83 & 16.79 \\
486834100624652800 & 54.08395 & 62.28723 & 3.99690 & 12.74 & 13.79 & 11.72 & 1.31 & 0.17 & L & 93.19 & 18.03 & 87.73 & 16.77 \\
2015458213056909184 & 351.49362 & 61.26683 & 4.00024 & 12.51 & 13.36 & 11.59 & 0.92 & 0.12 & L & 93.14 & 18.01 & 89.90 & 17.18 \\
506923449381427968 & 32.69322 & 59.25369 & 4.00720 & 12.24 & 13.07 & 11.35 & 0.94 & 0.12 & L & 93.03 & 17.99 & 88.11 & 16.84 \\
5238994102591371776 & 162.35781 & -66.62534 & 4.01417 & 14.04 & 14.61 & 13.31 & 0.56 & 0.11 & G & 92.91 & 17.97 & 87.01 & 16.63 \\
514674933331699584 & 32.62154 & 63.29753 & 4.03790 & 10.27 & 10.96 & 9.49 & 0.76 & 0.1 & L & 92.53 & 17.90 & 85.70 & 16.38 \\
2166861170366710272 & 313.73970 & 47.53379 & 4.04921 & 10.29 & 11.11 & 9.41 & 1.02 & 0.13 & L & 92.34 & 17.86 & 84.95 & 16.23 \\
5242076514741190272 & 162.97536 & -61.46728 & 4.05483 & 12.23 & 12.91 & 11.45 & 0.68 & 0.1 & O & 92.25 & 17.84 & 87.54 & 16.73 \\
5530071831587999232 & 129.78343 & -37.37551 & 4.06392 & 12.24 & 12.87 & 11.48 & 0.66 & 0.09 & O & 92.11 & 17.82 & 85.87 & 16.41 \\
422923956470923008 & 3.79087 & 58.42428 & 4.07117 & 9.54 & 10.14 & 8.83 & 0.61 & 0.06 & L & 91.99 & 17.79 & 85.09 & 16.26 \\
5545837900614099584 & 121.29597 & -34.36027 & 4.08860 & 11.73 & 12.56 & 10.84 & 0.9 & 0.11 & O & 91.72 & 17.74 & 87.57 & 16.74 \\
5254281334339678208 & 160.11285 & -60.07640 & 4.08916 & 13.97 & 14.91 & 12.96 & 1.25 & 0.15 & G & 91.71 & 17.74 & 84.80 & 16.21 \\
5241961409628951296 & 162.73299 & -62.09798 & 4.09530 & 14.32 & 15.12 & 13.43 & 0.99 & 0.11 & O & 91.61 & 17.72 & 84.80 & 16.21 \\
5861648327739540736 & 193.74820 & -65.20062 & 4.10167 & 14.64 & 15.63 & 13.62 & 1.28 & 0.13 & O & 91.51 & 17.70 & 85.32 & 16.31 \\
511706805997227648 & 25.25207 & 63.05553 & 4.13309 & 12.66 & 13.61 & 11.69 & 1.19 & 0.14 & G & 91.02 & 17.61 & 84.93 & 16.23 \\
3127458403130026112 & 101.78917 & 3.96710 & 4.13423 & 10.21 & 10.72 & 9.53 & 0.42 & 0.04 & L & 91.00 & 17.60 & 85.67 & 16.37 \\
462252662762965120 & 50.94951 & 59.35567 & 4.15636 & 11.84 & 12.87 & 10.84 & 1.22 & 0.16 & L & 90.66 & 17.54 & 86.38 & 16.51 \\
5321257604065975040 & 128.76428 & -52.47757 & 4.15812 & 14.51 & 15.28 & 13.68 & 0.83 & 0.13 & G & 90.64 & 17.53 & 85.35 & 16.31 \\
2031590552598614784 & 295.87018 & 29.23810 & 4.15973 & 14.49 & 15.30 & 13.56 & 1.02 & 0.13 & G & 90.61 & 17.53 & 84.17 & 16.09 \\
5852389305960163328 & 208.75541 & -64.03195 & 4.16962 & 11.28 & 12.18 & 10.36 & 1.06 & 0.14 & G & 90.46 & 17.50 & 84.93 & 16.23 \\
5614191175568405376 & 115.20408 & -25.45771 & 4.17117 & 12.42 & 13.36 & 11.45 & 1.15 & 0.12 & O & 90.44 & 17.49 & 84.94 & 16.23 \\
5619786177922254336 & 110.28102 & -21.51060 & 4.17560 & 12.51 & 13.26 & 11.67 & 0.82 & 0.1 & O & 90.37 & 17.48 & 85.12 & 16.27 \\
2934506447605426944 & 105.97944 & -17.87991 & 4.20487 & 11.59 & 12.31 & 10.79 & 0.75 & 0.12 & G & 89.92 & 17.39 & 84.59 & 16.17 \\
4690834328595493760 & 16.04228 & -70.95614 & 4.20529 & 15.60 & 15.92 & 15.22 & 0.0 & 0.11 & G & 89.92 & 17.39 & 83.12 & 15.89 \\
5253875717619475200 & 158.46303 & -61.80622 & 4.23097 & 14.74 & 15.57 & 13.80 & 1.07 & 0.12 & O & 89.53 & 17.32 & 82.66 & 15.8 \\
1981367545804985088 & 329.05685 & 52.98601 & 4.23698 & 11.95 & 12.85 & 11.02 & 1.07 & 0.14 & G & 89.44 & 17.30 & 83.66 & 15.99 \\
515832929535462016 & 41.08082 & 64.76592 & 4.23841 & 10.96 & 11.83 & 10.06 & 1.01 & 0.13 & G & 89.42 & 17.30 & 84.02 & 16.06 \\
5254653759541047424 & 155.20707 & -61.25195 & 4.23925 & 13.98 & 14.57 & 13.25 & 0.57 & 0.12 & G & 89.41 & 17.29 & 83.80 & 16.02 \\
5587972801102905984 & 113.75856 & -35.91299 & 4.24340 & 12.16 & 12.74 & 11.47 & 0.5 & 0.11 & G & 89.35 & 17.28 & 84.07 & 16.07 \\
5521352536886237952 & 123.41069 & -42.69920 & 4.24935 & 13.62 & 14.40 & 12.76 & 0.89 & 0.13 & G & 89.26 & 17.26 & 83.56 & 15.97 \\
3027940437469882880 & 110.38690 & -16.68722 & 4.25689 & 9.32 & 9.95 & 8.59 & 0.64 & 0.06 & L & 89.15 & 17.24 & 82.66 & 15.8 \\
522468168674975616 & 18.17150 & 61.21335 & 4.25925 & 10.96 & 11.64 & 10.19 & 0.63 & 0.07 & L & 89.11 & 17.24 & 84.98 & 16.24 \\
5338024572321721216 & 164.46108 & -60.74208 & 4.26618 & 9.44 & 9.99 & 8.79 & 0.55 & 0.07 & L & 89.01 & 17.22 & 80.98 & 15.48 \\
510584788742165760 & 19.00502 & 61.62071 & 4.27770 & 11.35 & 12.36 & 10.37 & 1.16 & 0.15 & L & 88.84 & 17.18 & 85.04 & 16.25 \\
2014609252631258496 & 342.09618 & 60.40476 & 4.27863 & 11.57 & 12.60 & 10.58 & 1.27 & 0.15 & G & 88.83 & 17.18 & 83.18 & 15.9 \\
5620400182140135168 & 112.95453 & -20.14966 & 4.28543 & 10.96 & 11.65 & 10.18 & 0.67 & 0.06 & L & 88.73 & 17.16 & 84.16 & 16.08 \\
2033008274099620480 & 296.26534 & 31.33077 & 4.28897 & 12.25 & 13.01 & 11.39 & 0.87 & 0.11 & L & 88.68 & 17.15 & 82.87 & 15.84 \\
228741784865956224 & 64.27528 & 41.73183 & 4.29045 & 10.67 & 11.41 & 9.90 & 0.72 & 0.09 & L & 88.66 & 17.15 & 83.80 & 16.01 \\
429890595286480384 & 0.67404 & 61.86107 & 4.30528 & 12.11 & 13.08 & 11.13 & 0.99 & 0.13 & L & 88.44 & 17.11 & 87.78 & 16.78 \\
1977074811892425600 & 332.26210 & 51.04585 & 4.32355 & 8.96 & 9.40 & 8.39 & 0.29 & 0.04 & L & 88.18 & 17.06 & 81.86 & 15.64 \\
2074102933481447808 & 301.83830 & 40.17809 & 4.32699 & 13.77 & 14.52 & 12.91 & 0.82 & 0.08 & L & 88.13 & 17.05 & 83.22 & 15.9 \\
5311298983669288832 & 136.84989 & -54.09276 & 4.35093 & 13.37 & 13.93 & 12.65 & 0.52 & 0.11 & G & 87.79 & 16.98 & 82.20 & 15.71 \\
2060021625508894592 & 302.28232 & 37.15195 & 4.36470 & 9.49 & 10.10 & 8.77 & 0.61 & 0.1 & L & 87.59 & 16.94 & 80.98 & 15.48 \\
429385923752386944 & 0.24680 & 60.95900 & 4.36516 & 10.86 & 11.53 & 9.96 & 0.9 & 0.07 & L & 87.59 & 16.94 & 79.87 & 15.27 \\
2006033847910275584 & 335.02002 & 56.06090 & 4.36625 & 12.13 & 12.97 & 11.21 & 1.01 & 0.13 & G & 87.57 & 16.94 & 81.70 & 15.61 \\
204588190167650048 & 71.39513 & 43.57284 & 4.37214 & 13.22 & 14.18 & 12.25 & 1.19 & 0.14 & G & 87.49 & 16.92 & 81.57 & 15.59 \\
4693901042617667584 & 27.66874 & -70.50366 & 4.37264 & 15.68 & 15.92 & 15.29 & 0.0 & 0.11 & G & 87.48 & 16.92 & 79.18 & 15.13 \\
5594091823824942464 & 119.66611 & -33.50405 & 4.40279 & 11.64 & 12.44 & 10.78 & 0.84 & 0.1 & O & 87.06 & 16.84 & 83.08 & 15.88 \\
197337185858157440 & 84.11148 & 44.59136 & 4.40345 & 11.82 & 12.43 & 11.25 & 0.48 & 0.06 & L & 87.05 & 16.84 & 80.17 & 15.32 \\
6055722403534963840 & 195.79449 & -60.87747 & 4.42452 & 9.46 & 10.21 & 8.65 & 0.78 & 0.08 & L & 86.76 & 16.78 & 81.66 & 15.61 \\
3397212822106196992 & 81.77704 & 16.93643 & 4.43840 & 12.75 & 13.32 & 12.06 & 0.48 & 0.11 & G & 86.57 & 16.74 & 81.58 & 15.59 \\
2936110669428633216 & 106.65835 & -15.80206 & 4.46484 & 12.42 & 13.21 & 11.56 & 0.82 & 0.1 & O & 86.21 & 16.67 & 82.22 & 15.71 \\
5881952871520184960 & 234.52125 & -58.69441 & 4.47575 & 15.24 & 16.25 & 14.22 & 1.32 & 0.13 & O & 86.06 & 16.65 & 79.55 & 15.2 \\
2011892320749270912 & 359.53791 & 61.21363 & 4.47861 & 10.57 & 11.12 & 9.66 & 0.74 & 0.07 & L & 86.02 & 16.64 & 79.71 & 15.23 \\
2005011237689458688 & 335.31995 & 54.53204 & 4.47944 & 11.44 & 12.16 & 10.63 & 0.76 & 0.07 & L & 86.01 & 16.64 & 80.52 & 15.39 \\
5254078504458244352 & 160.72436 & -61.02361 & 4.48366 & 12.84 & 13.68 & 11.94 & 0.97 & 0.11 & O & 85.95 & 16.62 & 80.57 & 15.4 \\
426881614218441600 & 12.47192 & 60.12738 & 4.50162 & 9.55 & 10.21 & 8.79 & 0.7 & 0.08 & L & 85.71 & 16.58 & 79.42 & 15.18 \\
5254000340399606016 & 157.26590 & -60.78069 & 4.50519 & 14.48 & 15.29 & 13.56 & 1.03 & 0.11 & O & 85.66 & 16.57 & 78.97 & 15.09 \\
5594382644652353664 & 119.05201 & -32.60264 & 4.51675 & 11.53 & 12.38 & 10.70 & 0.87 & 0.13 & G & 85.51 & 16.54 & 81.13 & 15.51 \\
5850308411442294400 & 206.85370 & -68.24990 & 4.52474 & 13.65 & 14.14 & 13.00 & 0.37 & 0.11 & G & 85.40 & 16.52 & 80.01 & 15.29 \\
4054440301294394624 & 262.70159 & -33.60992 & 4.52781 & 7.55 & 8.14 & 6.92 & 0.48 & 0.05 & L & 85.36 & 16.51 & 79.41 & 15.18 \\
5534012004528220160 & 119.94883 & -42.02838 & 4.54706 & 13.90 & 14.74 & 12.98 & 1.01 & 0.13 & G & 85.11 & 16.46 & 79.32 & 15.16 \\
506699870563323264 & 33.28119 & 58.07995 & 4.56524 & 11.27 & 11.94 & 10.55 & 0.62 & 0.06 & L & 84.87 & 16.41 & 79.45 & 15.18 \\
2012787293154800896 & 358.60238 & 62.14947 & 4.56615 & 11.45 & 12.28 & 10.57 & 0.96 & 0.12 & L & 84.85 & 16.41 & 79.13 & 15.12 \\
5338148473537341312 & 165.30989 & -60.11656 & 4.58610 & 11.08 & 11.81 & 10.25 & 0.76 & 0.07 & L & 84.59 & 16.36 & 79.99 & 15.29 \\
4690829659971892480 & 16.84515 & -70.88734 & 4.59426 & 15.88 & 16.22 & 15.37 & 0.09 & 0.11 & G & 84.49 & 16.34 & 78.98 & 15.09 \\
5253884788591163648 & 158.53969 & -61.59759 & 4.61631 & 13.91 & 14.75 & 12.99 & 1.01 & 0.11 & O & 84.20 & 16.29 & 78.52 & 15.01 \\
5253661725170126720 & 159.49855 & -62.20590 & 4.63195 & 14.41 & 15.35 & 13.63 & 0.9 & 0.11 & O & 84.00 & 16.25 & 79.82 & 15.25 \\
1981006115714214912 & 327.39800 & 52.39523 & 4.63908 & 11.46 & 12.45 & 10.48 & 0.91 & 0.23 & L & 83.91 & 16.23 & 85.05 & 16.25 \\
5521459979795304320 & 129.42007 & -47.36195 & 4.63985 & 7.71 & 8.26 & 7.05 & 0.38 & 0.04 & L & 83.90 & 16.23 & 80.08 & 15.3 \\
2170880813073764352 & 322.34628 & 49.11002 & 4.64071 & 11.77 & 12.62 & 10.87 & 0.99 & 0.13 & G & 83.89 & 16.23 & 78.47 & 15.0 \\
3044483895581000192 & 107.31421 & -13.78609 & 4.67003 & 10.09 & 10.85 & 9.26 & 0.77 & 0.07 & L & 83.52 & 16.15 & 79.29 & 15.15 \\
5338207327417387520 & 163.13667 & -60.52675 & 4.67416 & 10.94 & 11.55 & 10.19 & 0.54 & 0.08 & L & 83.47 & 16.14 & 79.15 & 15.13 \\
5338438297925480320 & 162.89899 & -59.38499 & 4.67767 & 9.41 & 9.97 & 8.73 & 0.52 & 0.04 & L & 83.43 & 16.14 & 77.28 & 14.77 \\
3046774762417915136 & 109.15680 & -11.48730 & 4.67830 & 7.83 & 8.33 & 7.20 & 0.32 & 0.03 & L & 83.42 & 16.13 & 78.98 & 15.09 \\
6060173364061645696 & 193.59158 & -58.43063 & 4.68971 & 6.36 & 6.80 & 5.79 & 0.23 & 0.03 & L & 83.27 & 16.11 & 78.33 & 14.97 \\
5861196531541297664 & 187.06483 & -65.04976 & 4.72838 & 14.52 & 15.34 & 13.58 & 1.06 & 0.12 & O & 82.79 & 16.01 & 76.02 & 14.53 \\
1998384927774603520 & 359.11116 & 58.02686 & 4.73481 & 11.71 & 12.60 & 10.79 & 1.03 & 0.13 & G & 82.72 & 16.00 & 77.45 & 14.8 \\
5242088403212116864 & 163.61189 & -61.34710 & 4.75984 & 11.54 & 12.32 & 10.69 & 0.85 & 0.13 & G & 82.41 & 15.94 & 77.35 & 14.78 \\
5533407170051636608 & 122.95171 & -42.05164 & 4.76441 & 14.79 & 15.90 & 13.77 & 1.36 & 0.15 & G & 82.35 & 15.93 & 77.05 & 14.72 \\
5541229748611783296 & 123.70107 & -37.65190 & 4.78070 & 13.80 & 14.82 & 12.79 & 1.24 & 0.13 & O & 82.16 & 15.89 & 77.20 & 14.75 \\
3051692843568009600 & 106.78562 & -7.79513 & 4.49659 & 12.54 & 13.27 & 11.70 & 0.87 & 0.11 & L & 85.78 & 16.59 & 79.04 & 15.11 \\
2011303326105008768 & 353.74839 & 59.35815 & 4.78948 & 12.14 & 13.26 & 11.08 & 1.45 & 0.16 & G & 82.05 & 15.87 & 75.96 & 14.52 \\
3099066951319051008 & 102.70284 & -7.98073 & 4.80971 & 12.57 & 13.26 & 11.77 & 0.62 & 0.08 & L & 81.81 & 15.82 & 78.58 & 15.02 \\
5864184488751391744 & 203.61003 & -64.37098 & 4.82483 & 14.71 & 15.56 & 13.75 & 1.31 & 0.13 & O & 81.63 & 15.79 & 70.95 & 13.56 \\
5329338700985814656 & 130.05832 & -47.55156 & 4.82751 & 13.24 & 14.15 & 12.28 & 1.12 & 0.14 & G & 81.59 & 15.78 & 75.92 & 14.51 \\
2928116120387181824 & 108.72647 & -22.23586 & 4.84478 & 12.81 & 13.54 & 11.97 & 0.8 & 0.12 & G & 81.39 & 15.74 & 76.09 & 14.54 \\
5306782361701536128 & 140.15436 & -56.85401 & 4.86219 & 13.91 & 14.60 & 13.11 & 0.72 & 0.12 & G & 81.18 & 15.70 & 75.90 & 14.51 \\
1960750328384177408 & 327.92260 & 43.13402 & 4.86438 & 8.67 & 9.19 & 8.03 & 0.39 & 0.04 & L & 81.16 & 15.70 & 75.77 & 14.48 \\
2011892703004353792 & 359.57487 & 61.22105 & 4.87514 & 10.66 & 11.41 & 9.83 & 0.75 & 0.07 & L & 81.03 & 15.67 & 77.01 & 14.72 \\
3344297935963515008 & 91.43635 & 13.23999 & 4.90958 & 11.89 & 12.64 & 11.03 & 0.71 & 0.06 & L & 80.63 & 15.60 & 78.05 & 14.92 \\
2078709577944648192 & 297.06443 & 43.12692 & 4.92549 & 8.90 & 9.42 & 8.26 & 0.43 & 0.05 & L & 80.45 & 15.56 & 74.51 & 14.24 \\
5258574068220187648 & 153.88689 & -58.17444 & 4.93255 & 10.24 & 10.94 & 9.46 & 0.59 & 0.08 & L & 80.37 & 15.54 & 77.63 & 14.84 \\
2060460704279873536 & 304.19788 & 36.54994 & 4.94524 & 11.57 & 12.65 & 10.54 & 1.45 & 0.19 & L & 80.22 & 15.52 & 72.74 & 13.9 \\
2055122987639665664 & 301.33609 & 32.65909 & 4.95045 & 12.27 & 13.38 & 11.21 & 1.35 & 0.18 & L & 80.16 & 15.50 & 75.78 & 14.48 \\
270272675510149504 & 64.94524 & 48.95326 & 4.97249 & 9.12 & 9.99 & 8.23 & 0.92 & 0.09 & L & 79.91 & 15.46 & 76.03 & 14.53 \\
5333640230992516480 & 173.32410 & -63.24240 & 4.97458 & 11.78 & 12.80 & 10.78 & 1.26 & 0.15 & G & 79.89 & 15.45 & 74.40 & 14.22 \\
3351921532976862336 & 100.15651 & 11.72748 & 4.97853 & 11.77 & 12.69 & 10.82 & 1.1 & 0.14 & G & 79.84 & 15.44 & 74.52 & 14.24 \\
2003938801532007808 & 342.15829 & 56.32153 & 4.98330 & 8.61 & 9.15 & 7.94 & 0.4 & 0.06 & L & 79.79 & 15.43 & 75.42 & 14.41 \\
6057402526059795072 & 181.66763 & -62.59685 & 4.98851 & 12.06 & 13.02 & 11.10 & 1.14 & 0.12 & O & 79.73 & 15.42 & 74.80 & 14.29 \\
2011315528113463808 & 354.70162 & 59.39182 & 4.99754 & 10.50 & 11.42 & 9.58 & 1.09 & 0.1 & L & 79.63 & 15.40 & 73.99 & 14.14 \\
5699042480743325312 & 120.09545 & -23.70317 & 5.02730 & 10.08 & 10.53 & 9.49 & 0.26 & 0.04 & L & 79.30 & 15.34 & 74.28 & 14.2 \\
515599111517099136 & 33.60315 & 65.59945 & 5.02942 & 11.90 & 12.75 & 11.01 & 0.7 & 0.12 & L & 79.27 & 15.33 & 79.92 & 15.27 \\
2164359918864249728 & 316.94415 & 46.73698 & 5.05758 & 11.90 & 12.74 & 11.01 & 0.99 & 0.13 & L & 78.96 & 15.27 & 73.22 & 13.99 \\
3390186156826555136 & 79.69992 & 13.98667 & 5.06607 & 11.52 & 12.19 & 10.67 & 0.78 & 0.12 & G & 78.87 & 15.25 & 73.13 & 13.98 \\
473293889810320128 & 57.10698 & 59.44227 & 5.06643 & 10.00 & 11.16 & 8.95 & 1.01 & 0.1 & L & 78.87 & 15.25 & 82.97 & 15.86 \\
5595650351503904896 & 118.45324 & -30.46031 & 5.07756 & 10.55 & 11.29 & 9.73 & 0.74 & 0.07 & L & 78.74 & 15.23 & 74.52 & 14.24 \\
5871738271033526016 & 207.68449 & -57.58051 & 5.07890 & 7.43 & 7.89 & 6.85 & 0.28 & 0.03 & L & 78.73 & 15.23 & 73.31 & 14.01 \\
2166303099490547072 & 311.55230 & 45.47861 & 5.09955 & 10.53 & 11.69 & 9.46 & 1.45 & 0.19 & L & 78.51 & 15.18 & 73.66 & 14.08 \\
5241157421762533248 & 162.23993 & -64.17420 & 5.10249 & 13.62 & 14.29 & 12.82 & 0.7 & 0.12 & G & 78.47 & 15.18 & 73.31 & 14.01 \\
5307006215391311360 & 142.54990 & -56.80824 & 5.13704 & 14.57 & 15.64 & 13.51 & 1.39 & 0.14 & O & 78.10 & 15.11 & 72.19 & 13.8 \\
2011892325047232256 & 359.53933 & 61.21370 & 5.14077 & 10.49 & 11.07 & 9.62 & 0.75 & 0.1 & L & 78.06 & 15.10 & 71.37 & 13.64 \\
4080122796947250176 & 281.32290 & -20.64739 & 5.15424 & 7.25 & 7.83 & 6.58 & 0.42 & 0.04 & L & 77.92 & 15.07 & 73.83 & 14.11 \\
4085919765884068736 & 282.74947 & -20.29525 & 6.63703 & 6.63 & 7.21 & 5.93 & 0.38 & 0.03 & L & 65.21 & 12.61 & 62.29 & 11.9 \\
1827869808377481216 & 296.64660 & 22.88975 & 5.19725 & 10.03 & 10.96 & 9.09 & 1.23 & 0.12 & L & 77.46 & 14.98 & 69.51 & 13.28 \\
4690377382729299328 & 10.34143 & -70.61853 & 5.20108 & 15.23 & 15.52 & 14.77 & -0.0 & 0.11 & G & 77.42 & 14.97 & 71.93 & 13.75 \\
5254295559276699392 & 159.07421 & -61.01256 & 5.20456 & 9.06 & 9.56 & 8.44 & 0.29 & 0.05 & L & 77.39 & 14.97 & 73.40 & 14.03 \\
5853170268450896768 & 219.37630 & -63.62524 & 5.21445 & 14.44 & 15.27 & 13.50 & 1.08 & 0.12 & O & 77.28 & 14.95 & 70.47 & 13.47 \\
5257939993613539456 & 147.08272 & -57.81045 & 5.21666 & 12.34 & 13.28 & 11.37 & 1.15 & 0.12 & O & 77.26 & 14.94 & 71.94 & 13.75 \\
513830684503187840 & 34.09382 & 62.55776 & 5.23993 & 12.62 & 13.62 & 11.62 & 1.23 & 0.15 & G & 77.02 & 14.90 & 71.77 & 13.72 \\
5698636279917579520 & 119.52141 & -24.04176 & 5.25024 & 10.34 & 10.80 & 9.73 & 0.35 & 0.05 & L & 76.91 & 14.88 & 70.68 & 13.51 \\
1968971582984827136 & 318.66850 & 41.71634 & 5.25760 & 8.88 & 9.91 & 7.90 & 1.22 & 0.11 & L & 76.84 & 14.86 & 71.92 & 13.75 \\
189726984845700480 & 86.05833 & 37.58687 & 5.25943 & 11.56 & 12.33 & 10.81 & 0.74 & 0.1 & L & 76.82 & 14.86 & 71.81 & 13.72 \\
6053622679932061056 & 188.32775 & -63.50637 & 5.26567 & 9.01 & 9.91 & 8.12 & 0.86 & 0.09 & L & 76.75 & 14.85 & 74.66 & 14.27 \\
5594100246268225280 & 119.84298 & -33.35713 & 5.28196 & 13.39 & 14.27 & 12.46 & 1.01 & 0.11 & O & 76.59 & 14.81 & 72.08 & 13.78 \\
4147381366335558784 & 272.50888 & -13.54596 & 5.30141 & 9.96 & 11.03 & 8.94 & 1.31 & 0.11 & L & 76.39 & 14.77 & 71.29 & 13.62 \\
5334506135119058304 & 171.27392 & -60.73461 & 5.30996 & 8.49 & 9.08 & 7.79 & 0.48 & 0.1 & L & 76.30 & 14.76 & 71.74 & 13.71 \\
5307761545524640256 & 147.17283 & -55.51953 & 5.32402 & 9.79 & 10.57 & 8.95 & 0.79 & 0.1 & L & 76.16 & 14.73 & 71.90 & 13.74 \\
1960981328902089088 & 330.10480 & 43.44535 & 5.33166 & 8.57 & 9.13 & 7.90 & 0.45 & 0.05 & L & 76.08 & 14.72 & 71.00 & 13.57 \\
5338215200143652992 & 163.78784 & -60.54772 & 5.33671 & 11.44 & 12.27 & 10.56 & 0.92 & 0.13 & G & 76.03 & 14.71 & 71.19 & 13.61 \\
5255220656517219840 & 156.71194 & -59.66953 & 5.34632 & 9.03 & 9.64 & 8.31 & 0.58 & 0.05 & L & 75.94 & 14.69 & 70.43 & 13.46 \\
458239995077788544 & 38.63042 & 58.83162 & 5.36511 & 10.46 & 11.49 & 9.51 & 1.2 & 0.1 & L & 75.75 & 14.65 & 70.75 & 13.52 \\
4190143160245024256 & 298.08750 & -11.36692 & 5.37668 & 7.54 & 8.03 & 6.92 & 0.25 & 0.03 & L & 75.63 & 14.63 & 72.20 & 13.8 \\
2010285491880986112 & 346.79198 & 58.55419 & 5.44090 & 9.28 & 9.96 & 8.51 & 0.64 & 0.06 & L & 75.00 & 14.51 & 70.57 & 13.49 \\
5547742052903182080 & 122.60782 & -32.52136 & 5.46460 & 10.99 & 11.72 & 10.18 & 0.74 & 0.12 & G & 74.78 & 14.46 & 70.24 & 13.42 \\
5312211543950752128 & 142.56597 & -53.05868 & 5.48394 & 11.19 & 12.09 & 10.25 & 1.06 & 0.14 & G & 74.59 & 14.43 & 69.67 & 13.31 \\
5338131529834231680 & 164.77043 & -60.27884 & 5.49457 & 11.65 & 12.46 & 10.76 & 0.91 & 0.13 & G & 74.49 & 14.41 & 69.62 & 13.31 \\
5891675303053080704 & 218.13779 & -56.88775 & 5.49457 & 6.55 & 7.11 & 5.93 & 0.36 & 0.04 & L & 74.49 & 14.41 & 70.33 & 13.44 \\
523887951723531648 & 11.62454 & 63.54327 & 5.51273 & 11.17 & 12.21 & 10.18 & 1.29 & 0.17 & L & 74.32 & 14.37 & 68.58 & 13.11 \\
5715183929918131968 & 115.47870 & -21.13306 & 5.51615 & 10.27 & 10.82 & 9.61 & 0.45 & 0.04 & L & 74.28 & 14.37 & 69.00 & 13.19 \\
459035766618689280 & 36.89776 & 58.91715 & 5.53070 & 10.37 & 11.47 & 9.37 & 1.28 & 0.11 & L & 74.15 & 14.34 & 69.95 & 13.37 \\
5253795384546671104 & 158.01837 & -61.78262 & 5.54225 & 8.70 & 9.18 & 8.09 & 0.25 & 0.03 & L & 74.04 & 14.32 & 70.07 & 13.39 \\
4103989346187406464 & 276.80604 & -15.11799 & 5.54693 & 10.07 & 10.94 & 9.18 & 0.95 & 0.13 & G & 73.99 & 14.31 & 69.51 & 13.28 \\
5539107450645759232 & 118.43778 & -36.97038 & 5.56408 & 10.59 & 11.47 & 9.75 & 0.88 & 0.13 & G & 73.83 & 14.28 & 70.02 & 13.38 \\
5254512193075687168 & 158.63079 & -59.80854 & 5.57332 & 11.84 & 12.94 & 10.79 & 1.31 & 0.13 & O & 73.75 & 14.26 & 69.99 & 13.38 \\
5525918495131126912 & 126.02410 & -44.85228 & 5.59210 & 13.08 & 14.24 & 12.02 & 1.45 & 0.16 & G & 73.57 & 14.23 & 68.31 & 13.05 \\
506602976101284736 & 26.76131 & 59.60626 & 5.60412 & 13.19 & 13.92 & 12.35 & 0.64 & 0.15 & L & 73.46 & 14.21 & 71.43 & 13.65 \\
5283779135317992448 & 98.37366 & -65.99373 & 5.63702 & 15.67 & 16.06 & 15.11 & 0.16 & 0.11 & G & 73.16 & 14.15 & 68.38 & 13.07 \\
2005753545481718912 & 331.89771 & 55.36274 & 5.65812 & 12.18 & 13.11 & 11.22 & 1.23 & 0.12 & L & 72.97 & 14.11 & 65.86 & 12.59 \\
5242185808733501696 & 162.09637 & -60.65394 & 5.66418 & 12.16 & 12.99 & 11.26 & 0.93 & 0.11 & O & 72.91 & 14.10 & 68.37 & 13.07 \\
2015622212085282048 & 354.86371 & 62.37214 & 5.66617 & 11.06 & 12.01 & 10.12 & 1.03 & 0.09 & L & 72.89 & 14.10 & 69.29 & 13.24 \\
2202863166783787520 & 330.67041 & 59.45248 & 5.68839 & 13.10 & 14.14 & 12.10 & 1.26 & 0.15 & G & 72.69 & 14.06 & 67.76 & 12.95 \\
5261561063335550208 & 95.02971 & -75.36110 & 5.70035 & 15.26 & 15.65 & 14.69 & 0.17 & 0.11 & G & 72.58 & 14.04 & 67.70 & 12.94 \\
2931247014102560000 & 108.29864 & -18.73074 & 5.72861 & 10.60 & 11.39 & 9.75 & 0.62 & 0.12 & L & 72.33 & 13.99 & 71.94 & 13.75 \\
2034428980559814400 & 299.89044 & 33.74604 & 5.78290 & 11.05 & 11.99 & 10.12 & 0.99 & 0.13 & L & 71.85 & 13.90 & 68.67 & 13.12 \\
5600471160241231616 & 118.49014 & -28.36762 & 5.80047 & 12.61 & 13.41 & 11.73 & 0.91 & 0.11 & O & 71.70 & 13.87 & 66.46 & 12.7 \\
422226488141991296 & 3.61766 & 56.25293 & 5.80901 & 8.78 & 9.37 & 8.08 & 0.44 & 0.08 & L & 71.63 & 13.85 & 67.82 & 12.96 \\
5613165915335320192 & 111.16913 & -26.18849 & 5.81585 & 11.45 & 12.33 & 10.54 & 0.94 & 0.12 & L & 71.57 & 13.84 & 67.94 & 12.98 \\
5327836325732931840 & 131.23286 & -50.56002 & 5.85935 & 9.21 & 9.96 & 8.39 & 0.72 & 0.07 & L & 71.19 & 13.77 & 67.59 & 12.92 \\
5595072420703114624 & 116.96477 & -32.17133 & 5.86387 & 13.12 & 14.08 & 12.16 & 1.13 & 0.14 & G & 71.15 & 13.76 & 66.27 & 12.66 \\
5544213926244557184 & 120.20160 & -37.82794 & 5.88476 & 10.63 & 11.53 & 9.71 & 1.02 & 0.13 & G & 70.98 & 13.73 & 66.36 & 12.68 \\
5436296928693979392 & 143.46188 & -36.61574 & 5.89839 & 9.12 & 9.52 & 8.58 & 0.41 & 0.05 & L & 70.86 & 13.71 & 61.54 & 11.76 \\
467560314629168640 & 41.46454 & 63.30457 & 5.90466 & 11.96 & 12.78 & 11.08 & 0.91 & 0.12 & L & 70.81 & 13.70 & 65.96 & 12.61 \\
5308893149150949248 & 145.29272 & -53.81604 & 5.90482 & 11.10 & 11.98 & 10.19 & 0.97 & 0.09 & L & 70.81 & 13.70 & 66.62 & 12.73 \\
2055014277739104896 & 303.09511 & 32.87160 & 5.95590 & 8.91 & 9.76 & 8.02 & 0.88 & 0.09 & L & 70.38 & 13.61 & 66.83 & 12.77 \\
5927687916632523264 & 250.53743 & -57.31247 & 5.95730 & 12.82 & 13.38 & 12.12 & 0.46 & 0.11 & G & 70.37 & 13.61 & 65.85 & 12.58 \\
5544001136384668288 & 121.32198 & -37.58019 & 6.02134 & 13.52 & 14.50 & 12.51 & 1.23 & 0.13 & O & 69.84 & 13.51 & 64.30 & 12.29 \\
4092905375639902464 & 277.97221 & -19.12510 & 6.74522 & 6.35 & 7.01 & 5.62 & 0.55 & 0.05 & L & 64.47 & 12.47 & 60.53 & 11.57 \\
1808020329279916288 & 300.29090 & 15.80350 & 6.10820 & 9.90 & 10.44 & 9.26 & 0.31 & 0.04 & L & 69.14 & 13.37 & 65.87 & 12.59 \\
4312361436842603520 & 287.31663 & 10.55247 & 6.11423 & 7.66 & 8.44 & 6.84 & 0.86 & 0.07 & L & 69.09 & 13.36 & 63.38 & 12.11 \\
6053428684887800320 & 185.88240 & -64.47089 & 6.12121 & 11.32 & 12.29 & 10.35 & 0.96 & 0.09 & L & 69.03 & 13.35 & 67.57 & 12.91 \\
4303770918113986304 & 299.38759 & 11.04366 & 6.17926 & 9.72 & 10.21 & 9.10 & 0.14 & 0.02 & L & 68.58 & 13.26 & 67.01 & 12.81 \\
4093976334264606976 & 273.85944 & -20.62955 & 6.17945 & 10.19 & 11.07 & 9.25 & 1.11 & 0.14 & L & 68.58 & 13.26 & 62.31 & 11.91 \\
5932812431123862016 & 241.29147 & -53.91943 & 6.19933 & 9.48 & 10.30 & 8.64 & 0.78 & 0.08 & L & 68.42 & 13.23 & 65.23 & 12.47 \\
506581226385580288 & 27.77925 & 59.88821 & 6.20627 & 10.30 & 11.02 & 9.50 & 0.66 & 0.06 & L & 68.37 & 13.22 & 64.66 & 12.36 \\
6059764002146656128 & 191.59278 & -59.12473 & 6.22040 & 8.07 & 8.64 & 7.38 & 0.4 & 0.04 & L & 68.26 & 13.20 & 64.79 & 12.38 \\
2059598687167348352 & 299.44206 & 35.63605 & 6.22543 & 12.68 & 13.69 & 11.69 & 1.26 & 0.16 & L & 68.22 & 13.19 & 62.54 & 11.95 \\
2008504454839717120 & 341.60318 & 59.44219 & 6.23397 & 9.00 & 9.92 & 8.08 & 0.95 & 0.08 & L & 68.15 & 13.18 & 65.22 & 12.46 \\
430670222050230912 & 9.18544 & 62.27424 & 6.24022 & 11.73 & 12.72 & 10.75 & 1.16 & 0.15 & L & 68.11 & 13.17 & 63.72 & 12.18 \\
525136962570940160 & 18.75456 & 65.59940 & 6.27279 & 10.23 & 11.24 & 9.28 & 1.17 & 0.1 & L & 67.86 & 13.12 & 63.08 & 12.06 \\
2015820463470505600 & 354.31691 & 62.42899 & 6.29664 & 9.24 & 10.22 & 8.28 & 1.08 & 0.09 & L & 67.67 & 13.09 & 64.22 & 12.27 \\
4512950187838606464 & 286.51934 & 15.74941 & 6.30024 & 14.61 & 15.49 & 13.67 & 1.03 & 0.13 & G & 67.65 & 13.08 & 62.94 & 12.03 \\
5823134325151372032 & 240.29463 & -63.77655 & 6.31663 & 6.22 & 6.59 & 5.63 & 0.12 & 0.02 & L & 67.52 & 13.06 & 63.71 & 12.18 \\
2027263738130844288 & 299.36918 & 26.55645 & 6.32059 & 8.23 & 9.14 & 7.30 & 1.05 & 0.09 & L & 67.49 & 13.05 & 62.86 & 12.01 \\
1994462866719961216 & 354.40810 & 54.84718 & 6.33647 & 9.03 & 9.72 & 8.26 & 0.63 & 0.12 & G & 67.38 & 13.03 & 63.32 & 12.1 \\
5339149677605627264 & 169.58945 & -59.23796 & 6.39427 & 12.57 & 13.31 & 11.72 & 0.77 & 0.1 & O & 66.95 & 12.95 & 62.66 & 11.98 \\
6057514092119497472 & 183.24857 & -62.09682 & 6.39726 & 10.47 & 11.36 & 9.60 & 0.86 & 0.07 & L & 66.92 & 12.94 & 63.99 & 12.23 \\
2006989121667184384 & 340.36050 & 56.43277 & 6.41896 & 8.55 & 9.09 & 7.89 & 0.36 & 0.04 & L & 66.76 & 12.91 & 62.90 & 12.02 \\
4096979650282842112 & 276.18542 & -16.79717 & 6.42429 & 8.41 & 9.08 & 7.59 & 0.67 & 0.06 & L & 66.73 & 12.91 & 62.53 & 11.95 \\
3291491450496573824 & 74.97904 & 10.28845 & 6.44163 & 14.32 & 14.74 & 13.69 & 0.27 & 0.11 & G & 66.60 & 12.88 & 61.69 & 11.79 \\
5254071873026676864 & 160.70349 & -61.12298 & 6.45365 & 11.21 & 11.96 & 10.38 & 0.75 & 0.12 & G & 66.51 & 12.86 & 62.36 & 11.92 \\
5312196047720402048 & 143.34884 & -52.75585 & 6.45380 & 11.06 & 12.07 & 10.08 & 1.14 & 0.1 & L & 66.51 & 12.86 & 62.85 & 12.01 \\
5868480143187802240 & 199.74280 & -62.38235 & 6.45975 & 8.08 & 8.71 & 7.34 & 0.5 & 0.08 & L & 66.47 & 12.86 & 63.00 & 12.04 \\
174489098011145216 & 71.94298 & 36.72278 & 6.46466 & 7.05 & 7.73 & 6.27 & 0.65 & 0.06 & L & 66.43 & 12.85 & 62.04 & 11.86 \\
513282131279401728 & 23.91530 & 65.33050 & 6.55713 & 12.49 & 13.65 & 11.42 & 1.45 & 0.16 & G & 65.77 & 12.72 & 60.90 & 11.64 \\
4096140001386430080 & 275.82979 & -18.57477 & 6.56959 & 9.80 & 10.83 & 8.83 & 1.13 & 0.09 & L & 65.68 & 12.70 & 62.19 & 11.88 \\
272444829450300160 & 67.57792 & 53.94018 & 6.56983 & 11.86 & 12.74 & 10.95 & 0.96 & 0.13 & G & 65.68 & 12.70 & 61.52 & 11.76 \\
5541507237862358912 & 123.09332 & -36.94374 & 6.66423 & 7.71 & 8.14 & 7.16 & 0.22 & 0.02 & L & 65.02 & 12.58 & 59.83 & 11.43 \\
5302258008774271488 & 127.18202 & -60.12256 & 6.69695 & 7.11 & 7.60 & 6.50 & 0.22 & 0.03 & L & 64.80 & 12.53 & 61.49 & 11.75 \\
5338072980840100608 & 165.93830 & -60.64226 & 6.69721 & 9.84 & 10.49 & 9.10 & 0.59 & 0.06 & L & 64.80 & 12.53 & 60.23 & 11.51 \\
4314923363333177984 & 293.01969 & 11.54976 & 6.69729 & 12.54 & 13.22 & 11.75 & 0.65 & 0.12 & G & 64.80 & 12.53 & 60.62 & 11.58 \\
2177714415280658944 & 323.72762 & 55.94226 & 6.71632 & 12.85 & 13.93 & 11.82 & 1.31 & 0.15 & G & 64.67 & 12.51 & 60.06 & 11.48 \\
6054829806275577216 & 185.33793 & -62.28164 & 6.73287 & 6.30 & 6.81 & 5.68 & 0.26 & 0.04 & L & 64.56 & 12.49 & 61.26 & 11.71 \\
429544700100302080 & 4.26041 & 60.80280 & 6.79828 & 13.65 & 14.60 & 12.67 & 1.02 & 0.13 & L & 64.12 & 12.40 & 61.45 & 11.74 \\
4204653587029046400 & 287.08654 & -7.43777 & 6.80601 & 7.34 & 8.02 & 6.57 & 0.58 & 0.05 & L & 64.07 & 12.39 & 60.67 & 11.6 \\
5935042378098601856 & 243.98144 & -51.12073 & 6.81248 & 10.33 & 11.31 & 9.38 & 1.1 & 0.14 & G & 64.03 & 12.38 & 59.99 & 11.47 \\
4505300988492333312 & 281.47541 & 12.33610 & 7.50794 & 9.75 & 10.36 & 9.00 & 0.53 & 0.07 & L & 59.79 & 11.56 & 55.75 & 10.65 \\
430766016998901376 & 8.31747 & 62.90726 & 6.84634 & 10.97 & 11.87 & 10.07 & 1.04 & 0.09 & L & 63.80 & 12.34 & 58.53 & 11.19 \\
5324034867356093056 & 137.06555 & -51.43625 & 6.92436 & 7.22 & 7.93 & 6.44 & 0.59 & 0.05 & L & 63.30 & 12.24 & 60.37 & 11.54 \\
2030848897634605440 & 300.19314 & 30.90759 & 6.96110 & 12.11 & 13.21 & 11.06 & 1.41 & 0.18 & L & 63.06 & 12.20 & 57.36 & 10.96 \\
5352181712213705856 & 159.03578 & -56.04323 & 6.98477 & 10.22 & 10.83 & 9.31 & 0.72 & 0.06 & L & 62.91 & 12.17 & 58.40 & 11.16 \\
3031875585286182144 & 110.50990 & -14.31818 & 6.99483 & 9.24 & 9.82 & 8.54 & 0.5 & 0.06 & L & 62.85 & 12.16 & 57.89 & 11.06 \\
5334563996911649408 & 179.47384 & -62.64613 & 7.00373 & 11.44 & 12.37 & 10.49 & 1.06 & 0.14 & G & 62.79 & 12.14 & 58.58 & 11.2 \\
5903821951590649600 & 228.74274 & -46.87257 & 7.05894 & 13.89 & 14.42 & 13.21 & 0.37 & 0.11 & G & 62.44 & 12.08 & 58.39 & 11.16 \\
5877533315817003648 & 219.29985 & -62.01092 & 7.06626 & 6.42 & 6.96 & 5.77 & 0.31 & 0.04 & L & 62.40 & 12.07 & 59.21 & 11.32 \\
3113441691460573312 & 102.63473 & 0.00700 & 7.09748 & 11.97 & 12.83 & 11.03 & 0.88 & 0.11 & L & 62.20 & 12.03 & 59.52 & 11.38 \\
5240438203718296192 & 165.36850 & -64.29067 & 7.12163 & 13.71 & 14.51 & 12.82 & 0.87 & 0.13 & G & 62.06 & 12.00 & 57.78 & 11.04 \\
5309174967720762496 & 144.21441 & -53.03278 & 7.13431 & 9.69 & 10.51 & 8.83 & 0.93 & 0.11 & L & 61.98 & 11.99 & 56.52 & 10.8 \\
5860785795219397376 & 184.39009 & -65.75399 & 7.13451 & 13.83 & 14.46 & 12.97 & 0.58 & 0.09 & O & 61.98 & 11.99 & 59.27 & 11.33 \\
5257664497238811776 & 148.85895 & -58.42969 & 7.19619 & 8.95 & 9.58 & 8.22 & 0.51 & 0.04 & L & 61.60 & 11.92 & 57.85 & 11.06 \\
5600628115523816320 & 117.51301 & -28.25514 & 7.19862 & 10.32 & 11.10 & 9.50 & 0.78 & 0.1 & L & 61.59 & 11.91 & 57.38 & 10.97 \\
5626365410677889792 & 131.05061 & -35.47371 & 7.21689 & 9.94 & 10.60 & 9.17 & 0.59 & 0.12 & G & 61.48 & 11.89 & 57.65 & 11.02 \\
2174677564161400064 & 326.32669 & 54.49638 & 7.23099 & 11.38 & 12.40 & 10.39 & 1.19 & 0.14 & G & 61.39 & 11.87 & 57.12 & 10.92 \\
2007997408188526336 & 337.20867 & 58.21093 & 7.23213 & 10.62 & 11.46 & 9.74 & 0.86 & 0.07 & L & 61.39 & 11.87 & 57.81 & 11.05 \\
4307944836090489600 & 290.25978 & 8.51633 & 7.23996 & 9.35 & 10.33 & 8.39 & 1.1 & 0.09 & L & 61.34 & 11.86 & 57.39 & 10.97 \\
2165771172070496512 & 317.72654 & 49.14204 & 7.25140 & 9.95 & 10.88 & 9.00 & 1.05 & 0.09 & L & 61.27 & 11.85 & 57.23 & 10.94 \\
5335963189825411072 & 172.84735 & -60.58341 & 7.34403 & 13.08 & 13.96 & 12.13 & 1.04 & 0.12 & O & 60.73 & 11.75 & 56.08 & 10.72 \\
5613564621430610560 & 111.82868 & -25.78535 & 7.41934 & 12.70 & 13.62 & 11.73 & 0.78 & 0.23 & L & 60.29 & 11.66 & 60.57 & 11.58 \\
3112475495616980992 & 104.50389 & -0.37596 & 7.42462 & 10.35 & 11.04 & 9.57 & 0.59 & 0.06 & L & 60.26 & 11.66 & 57.05 & 10.9 \\
5855468247702904704 & 190.52089 & -69.40756 & 7.51028 & 6.10 & 6.55 & 5.55 & 0.2 & 0.04 & L & 59.78 & 11.56 & 55.20 & 10.55 \\
2934712880912798464 & 108.42673 & -17.62026 & 7.51211 & 12.39 & 13.36 & 11.42 & 1.11 & 0.14 & G & 59.77 & 11.56 & 55.63 & 10.63 \\
5337191279923824384 & 168.04213 & -61.75487 & 7.53200 & 7.80 & 8.35 & 7.14 & 0.29 & 0.03 & L & 59.66 & 11.54 & 56.89 & 10.87 \\
3368698813404804352 & 95.55497 & 14.67813 & 7.56688 & 8.12 & 8.76 & 7.42 & 0.45 & 0.04 & L & 59.46 & 11.50 & 56.28 & 10.76 \\
5337958876494096256 & 165.10434 & -60.99319 & 7.63695 & 12.31 & 13.20 & 11.37 & 0.99 & 0.11 & O & 59.08 & 11.43 & 55.10 & 10.53 \\
5339394082770287232 & 167.42135 & -58.83772 & 7.72081 & 6.61 & 7.08 & 6.01 & 0.15 & 0.02 & L & 58.63 & 11.34 & 55.95 & 10.69 \\
5415098722470316544 & 152.59186 & -44.15874 & 7.77785 & 13.69 & 14.15 & 13.08 & 0.23 & 0.11 & G & 58.32 & 11.28 & 54.51 & 10.42 \\
2016028168089215488 & 356.26093 & 63.00385 & 7.80112 & 10.08 & 11.04 & 9.12 & 1.01 & 0.08 & L & 58.20 & 11.26 & 55.38 & 10.58 \\
2030063919381336832 & 299.79498 & 29.45072 & 7.81823 & 9.37 & 10.16 & 8.51 & 0.82 & 0.07 & L & 58.11 & 11.24 & 54.04 & 10.33 \\
1873112207907294848 & 316.06930 & 39.97223 & 7.85582 & 9.05 & 9.82 & 8.20 & 0.8 & 0.07 & L & 57.91 & 11.20 & 53.55 & 10.23 \\
470361114339849472 & 61.24359 & 58.65978 & 7.91561 & 7.16 & 7.92 & 6.32 & 0.74 & 0.06 & L & 57.61 & 11.14 & 54.02 & 10.32 \\
5614916921960857088 & 114.04436 & -25.36403 & 7.96016 & 14.49 & 15.58 & 13.45 & 1.29 & 0.13 & O & 57.38 & 11.10 & 53.35 & 10.2 \\
2170785842762144512 & 322.18718 & 48.97821 & 7.96686 & 10.10 & 10.90 & 9.24 & 0.8 & 0.12 & G & 57.34 & 11.09 & 53.70 & 10.26 \\
1825621002188696448 & 294.15720 & 20.33293 & 7.99014 & 6.58 & 7.41 & 5.72 & 0.81 & 0.07 & L & 57.23 & 11.07 & 53.96 & 10.31 \\
428620663657823232 & 7.49410 & 60.21196 & 8.00066 & 8.51 & 9.23 & 7.71 & 0.66 & 0.05 & L & 57.17 & 11.06 & 53.61 & 10.25 \\
261548119462093568 & 77.66762 & 49.68760 & 8.00263 & 9.06 & 9.69 & 8.32 & 0.53 & 0.06 & L & 57.16 & 11.06 & 53.29 & 10.18 \\
5236551193933797888 & 174.75935 & -65.20662 & 8.00290 & 14.65 & 15.67 & 13.62 & 1.18 & 0.12 & O & 57.16 & 11.06 & 53.56 & 10.24 \\
3050050207554658048 & 105.24924 & -8.70898 & 8.01127 & 9.62 & 10.32 & 8.79 & 0.68 & 0.07 & L & 57.12 & 11.05 & 53.30 & 10.19 \\
5852880955104044800 & 214.51090 & -64.42147 & 8.19958 & 14.15 & 15.00 & 13.17 & 1.04 & 0.12 & O & 56.19 & 10.87 & 51.58 & 9.86 \\
5887482762148283008 & 228.20632 & -54.75528 & 8.22041 & 9.02 & 9.90 & 8.19 & 0.91 & 0.1 & L & 56.09 & 10.85 & 51.56 & 9.85 \\
512524361613040640 & 23.18010 & 63.59380 & 8.37701 & 6.64 & 7.46 & 5.78 & 0.8 & 0.11 & L & 55.35 & 10.71 & 52.09 & 9.96 \\
3329849043206545920 & 92.80659 & 9.61249 & 8.61488 & 8.67 & 9.24 & 7.99 & 0.3 & 0.03 & L & 54.27 & 10.50 & 51.93 & 9.92 \\
202939854734748032 & 70.99117 & 40.83478 & 8.63925 & 11.13 & 11.87 & 10.29 & 0.72 & 0.06 & L & 54.17 & 10.48 & 50.60 & 9.67 \\
5613972681993587200 & 115.49584 & -25.87617 & 8.93422 & 8.74 & 9.31 & 8.04 & 0.41 & 0.04 & L & 52.90 & 10.23 & 49.24 & 9.41 \\
5254097093074642944 & 159.83465 & -61.15243 & 9.19783 & 8.80 & 9.39 & 8.12 & 0.24 & 0.03 & L & 51.83 & 10.02 & 50.58 & 9.67 \\
4056026175045038464 & 267.15626 & -30.47597 & 9.31686 & 8.24 & 9.08 & 7.43 & 0.77 & 0.07 & L & 51.36 & 9.93 & 48.08 & 9.19 \\
5854560115494081024 & 215.45224 & -61.54966 & 9.46519 & 8.26 & 8.97 & 7.47 & 0.58 & 0.05 & L & 50.79 & 9.82 & 48.09 & 9.19 \\
4269036830424588800 & 288.19714 & 3.55740 & 9.48055 & 7.90 & 8.67 & 7.12 & 0.66 & 0.05 & L & 50.74 & 9.81 & 47.54 & 9.09 \\
5329838158460391296 & 131.22276 & -46.34296 & 9.56113 & 7.97 & 8.53 & 7.36 & 0.32 & 0.03 & L & 50.43 & 9.75 & 46.73 & 8.93 \\
5835124087174043136 & 244.71595 & -57.89980 & 9.75376 & 6.15 & 6.70 & 5.52 & 0.25 & 0.02 & L & 49.73 & 9.62 & 47.09 & 9.0 \\
5351423049186195328 & 158.22527 & -58.52100 & 9.75912 & 11.01 & 11.86 & 10.14 & 0.71 & 0.07 & L & 49.71 & 9.62 & 48.18 & 9.21 \\
5993655659352495616 & 243.61906 & -40.79315 & 9.76457 & 12.20 & 12.89 & 11.39 & 0.62 & 0.12 & G & 49.69 & 9.61 & 46.24 & 8.84 \\
5254662177677566464 & 155.34567 & -61.07408 & 9.76811 & 8.59 & 9.09 & 7.96 & 0.23 & 0.03 & L & 49.68 & 9.61 & 46.62 & 8.91 \\
2013029941628292352 & 359.39565 & 62.71824 & 9.80569 & 9.44 & 10.16 & 8.65 & 0.66 & 0.06 & L & 49.54 & 9.58 & 45.95 & 8.78 \\
5241804518715438336 & 165.39269 & -62.21022 & 9.84085 & 12.20 & 13.06 & 11.27 & 0.92 & 0.11 & O & 49.42 & 9.56 & 45.97 & 8.79 \\
5328248672646357120 & 132.04364 & -48.65915 & 9.84168 & 11.91 & 13.00 & 10.91 & 1.19 & 0.11 & L & 49.42 & 9.56 & 46.36 & 8.86 \\
5328949100222702848 & 130.67412 & -48.68614 & 10.02929 & 14.30 & 15.33 & 13.28 & 1.19 & 0.14 & G & 48.76 & 9.43 & 45.15 & 8.63 \\
4685261526923834496 & 2.60032 & -75.17706 & 10.09004 & 14.71 & 15.03 & 14.23 & 0.0 & 0.11 & G & 48.56 & 9.39 & 44.31 & 8.47 \\
2070224337474904064 & 311.49913 & 45.30694 & 10.14797 & 9.42 & 10.48 & 8.42 & 1.12 & 0.09 & L & 48.36 & 9.35 & 45.81 & 8.75 \\
5337257834740652160 & 167.55357 & -60.84747 & 10.27245 & 11.09 & 12.12 & 10.09 & 1.11 & 0.11 & L & 47.95 & 9.27 & 45.07 & 8.61 \\
201574982848108416 & 74.92307 & 40.83603 & 10.30573 & 9.92 & 10.67 & 9.10 & 0.73 & 0.08 & L & 47.84 & 9.25 & 43.93 & 8.4 \\
4156450099578283776 & 279.51377 & -8.36895 & 10.34150 & 8.88 & 9.93 & 7.92 & 1.07 & 0.09 & L & 47.72 & 9.23 & 45.11 & 8.62 \\
5241780677399802624 & 165.37783 & -62.29079 & 10.35488 & 10.31 & 11.08 & 9.47 & 0.63 & 0.06 & L & 47.68 & 9.22 & 45.65 & 8.72 \\
5859119760248045312 & 198.50696 & -64.32488 & 10.35635 & 10.85 & 11.83 & 9.89 & 1.06 & 0.13 & L & 47.68 & 9.22 & 44.47 & 8.5 \\
5538569613358406144 & 117.35518 & -38.23935 & 10.50594 & 12.62 & 13.34 & 11.79 & 0.67 & 0.12 & G & 47.20 & 9.13 & 43.95 & 8.4 \\
4267549637851481344 & 286.16423 & 1.30614 & 17.13794 & 7.88 & 8.66 & 7.00 & 0.75 & 0.07 & L & 33.44 & 6.47 & 30.68 & 5.86 \\
5337764640889249536 & 168.58836 & -60.05292 & 10.70960 & 9.27 & 9.92 & 8.51 & 0.45 & 0.05 & L & 46.56 & 9.01 & 44.25 & 8.46 \\
506779550797525760 & 31.95200 & 58.44353 & 10.87727 & 8.84 & 9.58 & 8.04 & 0.65 & 0.06 & L & 46.06 & 8.91 & 42.87 & 8.19 \\
2007201567928631296 & 340.21724 & 56.82946 & 10.88439 & 8.04 & 8.70 & 7.29 & 0.48 & 0.04 & L & 46.04 & 8.90 & 43.43 & 8.3 \\
5871922507947292032 & 205.07765 & -57.61318 & 10.94947 & 7.47 & 8.03 & 6.79 & 0.33 & 0.03 & L & 45.84 & 8.87 & 42.87 & 8.19 \\
3027495856819349248 & 113.41167 & -16.31710 & 10.98248 & 11.04 & 11.89 & 10.16 & 0.82 & 0.12 & G & 45.75 & 8.85 & 42.75 & 8.17 \\
4256744187345732224 & 280.53297 & -4.29349 & 11.05302 & 9.92 & 11.04 & 8.88 & 1.26 & 0.1 & L & 45.54 & 8.81 & 42.59 & 8.14 \\
203496585576324224 & 72.44976 & 42.28970 & 11.11731 & 8.60 & 9.23 & 7.85 & 0.44 & 0.06 & L & 45.35 & 8.77 & 42.91 & 8.2 \\
5611465073923671424 & 106.94491 & -24.91952 & 11.18235 & 11.25 & 11.81 & 10.56 & 0.35 & 0.11 & G & 45.17 & 8.74 & 42.18 & 8.06 \\
5313887130948758016 & 142.92069 & -49.65499 & 11.20064 & 8.88 & 9.83 & 7.95 & 0.92 & 0.08 & L & 45.12 & 8.73 & 42.85 & 8.19 \\
462407693902385792 & 52.35821 & 60.44647 & 11.27625 & 11.76 & 12.88 & 10.76 & 1.18 & 0.1 & L & 44.90 & 8.69 & 42.43 & 8.11 \\
5932569709575669504 & 243.32248 & -54.23490 & 11.28752 & 7.98 & 8.65 & 7.24 & 0.43 & 0.04 & L & 44.87 & 8.68 & 42.80 & 8.18 \\
3430067092837622272 & 91.64561 & 26.32922 & 11.30513 & 9.34 & 9.97 & 8.64 & 0.47 & 0.06 & L & 44.82 & 8.67 & 41.46 & 7.92 \\
2002637323358768000 & 343.65706 & 54.26545 & 11.31916 & 13.43 & 14.15 & 12.54 & 0.74 & 0.1 & L & 44.78 & 8.66 & 41.37 & 7.91 \\
200708636406382720 & 75.34662 & 39.96038 & 11.62570 & 7.34 & 7.94 & 6.68 & 0.34 & 0.04 & L & 43.95 & 8.50 & 41.10 & 7.85 \\
5332375453374624640 & 178.07378 & -65.40418 & 11.63735 & 9.33 & 10.09 & 8.59 & 0.58 & 0.07 & L & 43.92 & 8.49 & 41.00 & 7.84 \\
2030427789026783488 & 299.45419 & 30.26590 & 11.66304 & 10.42 & 11.28 & 9.52 & 1.05 & 0.13 & L & 43.85 & 8.48 & 38.75 & 7.41 \\
2073922579215436288 & 301.01866 & 39.10421 & 11.92821 & 12.97 & 13.86 & 12.03 & 0.93 & 0.13 & G & 43.16 & 8.35 & 40.05 & 7.65 \\
1999252442448732288 & 358.02928 & 58.74172 & 12.14061 & 9.32 & 10.20 & 8.46 & 0.86 & 0.08 & L & 42.63 & 8.24 & 39.46 & 7.54 \\
5336389564126521728 & 175.70084 & -58.99339 & 12.18311 & 10.90 & 11.71 & 10.02 & 0.75 & 0.08 & L & 42.52 & 8.22 & 39.90 & 7.62 \\
6054992602724692608 & 188.59725 & -61.23762 & 12.21766 & 11.13 & 12.23 & 10.11 & 1.29 & 0.12 & L & 42.44 & 8.21 & 38.68 & 7.39 \\
4066375912402666624 & 274.06943 & -23.30591 & 12.27464 & 15.32 & 16.30 & 14.35 & 1.29 & 0.13 & O & 42.30 & 8.18 & 36.85 & 7.04 \\
5616601820448126336 & 111.52996 & -25.25730 & 12.35350 & 9.39 & 10.15 & 8.59 & 0.74 & 0.06 & L & 42.11 & 8.14 & 38.10 & 7.28 \\
5240441472232302848 & 165.56688 & -64.26289 & 12.43802 & 8.85 & 9.60 & 8.06 & 0.53 & 0.05 & L & 41.91 & 8.11 & 40.02 & 7.65 \\
5884729035255064064 & 238.67837 & -54.56644 & 12.63346 & 8.96 & 9.87 & 8.03 & 0.82 & 0.1 & L & 41.45 & 8.02 & 39.63 & 7.57 \\
470386952863752576 & 61.53736 & 58.80875 & 12.65005 & 10.26 & 11.19 & 9.37 & 0.7 & 0.09 & L & 41.41 & 8.01 & 40.77 & 7.79 \\
5865206961464617088 & 201.62523 & -63.16263 & 12.88787 & 11.05 & 12.22 & 10.01 & 1.34 & 0.21 & L & 40.87 & 7.91 & 37.51 & 7.17 \\
4253435825622331392 & 280.73864 & -5.82091 & 12.91058 & 9.10 & 9.92 & 8.35 & 0.72 & 0.08 & L & 40.82 & 7.90 & 37.22 & 7.11 \\
5310669788148987520 & 139.59222 & -54.41226 & 13.12071 & 13.73 & 14.71 & 12.75 & 1.06 & 0.14 & G & 40.36 & 7.81 & 37.37 & 7.14 \\
5311616398935271168 & 140.00627 & -52.85618 & 13.23958 & 10.85 & 11.86 & 9.89 & 0.98 & 0.11 & L & 40.11 & 7.76 & 37.96 & 7.25 \\
4313179507891570304 & 287.50172 & 12.53654 & 13.43999 & 10.08 & 11.20 & 9.07 & 1.38 & 0.18 & L & 39.68 & 7.68 & 35.09 & 6.71 \\
5350852677538959104 & 162.75755 & -58.59059 & 13.45493 & 10.91 & 11.91 & 9.97 & 0.94 & 0.08 & L & 39.65 & 7.67 & 37.75 & 7.22 \\
5600915775257809152 & 119.42569 & -27.60189 & 13.45979 & 11.49 & 12.36 & 10.66 & 0.84 & 0.1 & L & 39.64 & 7.67 & 36.28 & 6.93 \\
5614312705966204288 & 117.01604 & -25.57777 & 13.59892 & 9.50 & 10.14 & 8.79 & 0.49 & 0.05 & L & 39.36 & 7.61 & 36.03 & 6.89 \\
459263743483634304 & 36.80736 & 59.46060 & 13.63864 & 9.14 & 10.11 & 8.19 & 0.96 & 0.11 & L & 39.28 & 7.60 & 36.90 & 7.05 \\
5596601154188852352 & 121.58947 & -30.09687 & 13.67010 & 9.49 & 10.23 & 8.67 & 0.57 & 0.05 & L & 39.21 & 7.58 & 37.12 & 7.09 \\
6030635804488868480 & 249.53582 & -31.47765 & 13.68681 & 12.78 & 13.33 & 12.09 & 0.32 & 0.11 & G & 39.18 & 7.58 & 36.48 & 6.97 \\
4267397694768545920 & 287.05729 & 1.29863 & 13.75460 & 6.61 & 7.39 & 5.85 & 0.66 & 0.06 & L & 39.04 & 7.55 & 35.95 & 6.87 \\
5586922973654572416 & 116.29911 & -36.97475 & 13.76670 & 12.17 & 12.95 & 11.27 & 0.78 & 0.12 & G & 39.02 & 7.55 & 36.05 & 6.89 \\
4087335043492541696 & 286.51307 & -18.42825 & 13.77231 & 12.49 & 13.06 & 11.81 & 0.31 & 0.11 & G & 39.01 & 7.54 & 36.44 & 6.96 \\
206577210999441536 & 74.41700 & 46.09253 & 13.84765 & 11.03 & 12.01 & 10.07 & 1.06 & 0.09 & L & 38.86 & 7.52 & 35.59 & 6.8 \\
2243309938950947200 & 304.41505 & 62.75205 & 13.98367 & 14.12 & 14.63 & 13.61 & 0.02 & 0.11 & G & 38.59 & 7.46 & 36.68 & 7.01 \\
5351331755370445056 & 161.23472 & -56.28954 & 14.10712 & 8.07 & 8.99 & 7.51 & 0.51 & 0.05 & L & 38.35 & 7.42 & 36.08 & 6.9 \\
5597327141100381568 & 119.74674 & -29.30786 & 14.15735 & 9.98 & 10.74 & 9.17 & 0.61 & 0.05 & L & 38.26 & 7.40 & 35.87 & 6.86 \\
2016626856473497344 & 352.30314 & 63.37430 & 14.37514 & 10.78 & 11.94 & 9.72 & 1.29 & 0.11 & L & 37.85 & 7.32 & 35.28 & 6.74 \\
6026412893938675712 & 254.58229 & -33.60913 & 6.06133 & 6.67 & 7.17 & 5.95 & 0.46 & 0.04 & L & 69.51 & 13.45 & 64.16 & 12.26 \\
2161786374436607616 & 315.02658 & 42.59755 & 14.71797 & 8.39 & 9.71 & 7.28 & 1.52 & 0.12 & L & 37.23 & 7.20 & 34.44 & 6.58 \\
508915489570374272 & 24.30841 & 57.75922 & 14.79237 & 8.81 & 9.08 & 8.01 & 0.59 & 0.06 & L & 37.09 & 7.17 & 30.31 & 5.79 \\
2034684200359279488 & 297.82201 & 32.67553 & 15.00336 & 13.12 & 14.18 & 12.05 & 1.42 & 0.18 & L & 36.73 & 7.10 & 32.06 & 6.13 \\
5864955727424819200 & 203.49590 & -64.05556 & 15.04436 & 9.72 & 10.54 & 8.88 & 0.57 & 0.06 & L & 36.65 & 7.09 & 35.56 & 6.8 \\
2016581673416790656 & 350.61846 & 62.75714 & 15.09343 & 10.12 & 11.35 & 9.12 & 1.27 & 0.11 & L & 36.57 & 7.07 & 34.13 & 6.52 \\
2071433765909167232 & 308.22621 & 46.60125 & 15.11946 & 8.82 & 9.73 & 7.91 & 0.8 & 0.07 & L & 36.53 & 7.06 & 34.69 & 6.63 \\
3324153371114695680 & 95.35961 & 6.47015 & 15.23122 & 8.02 & 8.65 & 7.32 & 0.36 & 0.04 & L & 36.34 & 7.03 & 34.08 & 6.51 \\
5537860123428416640 & 119.69307 & -38.99433 & 15.55821 & 11.46 & 12.34 & 10.55 & 0.9 & 0.12 & L & 35.80 & 6.92 & 32.75 & 6.26 \\
6704330080883057536 & 281.53600 & -48.63307 & 16.09459 & 12.59 & 13.03 & 11.97 & 0.12 & 0.11 & G & 34.95 & 6.76 & 32.33 & 6.18 \\
1870258975238302208 & 310.85080 & 35.58778 & 16.39062 & 6.07 & 6.69 & 5.36 & 0.34 & 0.03 & L & 34.51 & 6.67 & 32.41 & 6.19 \\
6026305309220584576 & 253.41732 & -33.34511 & 16.40369 & 12.99 & 13.59 & 12.25 & 0.39 & 0.11 & G & 34.49 & 6.67 & 32.03 & 6.12 \\
4638315266636230400 & 30.74872 & -74.05691 & 16.48065 & 14.19 & 14.70 & 13.59 & 0.13 & 0.11 & G & 34.38 & 6.65 & 32.24 & 6.16 \\
5338036117182452096 & 166.05607 & -60.97991 & 16.65998 & 8.19 & 8.90 & 7.38 & 0.5 & 0.05 & L & 34.11 & 6.60 & 32.24 & 6.16 \\
2058374144759464064 & 301.11066 & 34.11225 & 17.07369 & 8.46 & 9.24 & 7.61 & 0.69 & 0.06 & L & 33.53 & 6.49 & 31.04 & 5.93 \\
5878388529664102016 & 218.79935 & -60.99798 & 17.11025 & 9.85 & 10.96 & 8.74 & 1.27 & 0.12 & L & 33.48 & 6.48 & 31.01 & 5.93 \\
2198162651491732608 & 329.46952 & 56.16389 & 17.87198 & 9.83 & 10.85 & 8.87 & 0.92 & 0.1 & L & 32.47 & 6.28 & 30.98 & 5.92 \\
5253717937706836480 & 159.23233 & -61.58131 & 18.05246 & 11.66 & 12.47 & 10.73 & 0.76 & 0.1 & O & 32.24 & 6.24 & 30.06 & 5.75 \\
6026596989041710336 & 254.88447 & -32.95258 & 18.13188 & 12.53 & 13.10 & 11.76 & 0.4 & 0.11 & G & 32.14 & 6.22 & 29.64 & 5.66 \\
5255254711361371520 & 157.07013 & -59.35018 & 18.17758 & 8.30 & 8.97 & 7.52 & 0.44 & 0.06 & L & 32.08 & 6.21 & 30.21 & 5.77 \\
188724234539584256 & 78.84160 & 40.07802 & 18.19076 & 9.78 & 10.66 & 8.85 & 0.74 & 0.1 & L & 32.07 & 6.20 & 30.62 & 5.85 \\
5351161399785606016 & 161.13616 & -57.56536 & 18.87302 & 7.15 & 7.82 & 6.43 & 0.36 & 0.04 & L & 31.25 & 6.04 & 29.46 & 5.63 \\
1873250780732545920 & 314.33680 & 40.17749 & 20.14034 & 9.27 & 10.36 & 8.28 & 1.13 & 0.11 & L & 29.85 & 5.77 & 27.46 & 5.25 \\
5523162573544337408 & 129.25540 & -44.11465 & 20.49764 & 6.66 & 7.31 & 5.90 & 0.41 & 0.04 & L & 29.48 & 5.70 & 27.52 & 5.26 \\
5937099633141128448 & 251.32962 & -51.34264 & 20.85306 & 9.60 & 10.51 & 8.67 & 0.74 & 0.06 & L & 29.13 & 5.63 & 27.90 & 5.33 \\
4644478166748030976 & 35.20622 & -73.08565 & 21.36729 & 13.63 & 14.02 & 13.06 & 0.0 & 0.11 & G & 28.63 & 5.54 & 26.33 & 5.03 \\
4094784475310672128 & 274.24882 & -19.07583 & 21.83410 & 7.48 & 8.43 & 6.62 & 0.62 & 0.06 & L & 28.20 & 5.45 & 27.59 & 5.27 \\
4103564728516764032 & 280.45457 & -14.50543 & 11.03608 & 13.65 & 14.58 & 12.94 & 0.58 & 0.12 & G & 45.59 & 8.82 & 44.40 & 8.49 \\
6350220751862829952 & 358.65290 & -83.28872 & 22.44150 & 14.31 & 15.01 & 13.60 & 0.34 & 0.11 & G & 27.66 & 5.35 & 26.14 & 5.0 \\
5600052040150252800 & 114.64682 & -28.49960 & 23.17284 & 9.22 & 9.95 & 8.42 & 0.58 & 0.05 & L & 27.04 & 5.23 & 24.68 & 4.72 \\
5253571526514498176 & 159.11275 & -62.19251 & 24.21976 & 12.41 & 13.32 & 11.49 & 0.76 & 0.1 & O & 26.21 & 5.07 & 24.73 & 4.73 \\
5858474003300201856 & 193.43279 & -65.89971 & 26.46392 & 11.93 & 12.63 & 11.09 & 0.51 & 0.09 & O & 24.63 & 4.76 & 22.91 & 4.38 \\
6096564686351860992 & 213.33208 & -44.89374 & 26.68846 & 12.41 & 13.00 & 11.69 & 0.28 & 0.11 & G & 24.48 & 4.74 & 22.71 & 4.34 \\
5355057622305532928 & 155.17091 & -55.32138 & 28.16616 & 7.82 & 8.68 & 6.96 & 0.73 & 0.06 & L & 23.57 & 4.56 & 21.60 & 4.13 \\
5964193485048327808 & 252.91061 & -45.42671 & 28.86509 & 8.85 & 10.11 & 7.76 & 1.15 & 0.11 & L & 23.17 & 4.48 & 22.46 & 4.29 \\
5597379741549105280 & 119.59202 & -29.13008 & 30.09021 & 8.12 & 9.00 & 7.26 & 0.72 & 0.06 & L & 22.50 & 4.35 & 20.69 & 3.95 \\
5238808628736339584 & 164.28834 & -65.13474 & 15.71624 & 8.66 & 9.31 & 7.85 & 0.47 & 0.04 & L & 35.54 & 6.87 & 33.41 & 6.38 \\
5864135319959353600 & 204.15366 & -64.55832 & 34.05097 & 9.10 & 10.18 & 8.12 & 0.98 & 0.1 & L & 20.62 & 3.99 & 19.18 & 3.67 \\
5546476927338700416 & 123.26755 & -34.57851 & 41.46411 & 6.46 & 7.30 & 5.58 & 0.61 & 0.05 & L & 17.95 & 3.47 & 16.69 & 3.19 \\
2027951173435143680 & 297.87876 & 27.46021 & 44.87621 & 6.66 & 7.50 & 5.78 & 0.64 & 0.06 & L & 16.98 & 3.28 & 15.61 & 2.98 \\
\hline\hline
\end{tabular}
\end{table}

==> tab_age_1.5_B_PA_PAC.tex <==
\begin{table}
\begin{tabular}{cccccccccccccc}
Gaia DR2 source Id & RA[deg] & DEC[deg] & P[d] & G[mag] & G_BP[mag] & G_RP[mag] & E(gbp-grb)[mag] & sigma_E(gbp-grb)[mag] & Note & t_pa[Myr] & sigma(t)_pa[Myr] & t_pac[Myr] & sigma(t)_pac[Myr] \\
3442172745919329664 & 82.35887 & 27.00089 & 3.34920 & 11.57 & 12.21 & 10.78 & 0.72 & 0.12 & G & 141.71 & 26.10 & 122.49 & 21.72 \\
4704080802304630784 & 12.82014 & -68.98430 & 0.99469 & 18.24 & 18.45 & 17.79 & 0.18 & 0.11 & G & 303.00 & 55.82 & 257.01 & 45.57 \\
5521400228203695232 & 123.35129 & -42.27568 & 1.00189 & 16.05 & 16.93 & 15.15 & 1.23 & 0.15 & G & 301.64 & 55.56 & 268.78 & 47.65 \\
6379351625245757568 & 359.99997 & -75.19496 & 1.03777 & 17.68 & 17.98 & 17.36 & 0.02 & 0.11 & G & 295.07 & 54.35 & 269.73 & 47.82 \\
4711142067840447360 & 21.61608 & -64.87535 & 1.06447 & 17.86 & 18.05 & 17.41 & 0.16 & 0.11 & G & 290.41 & 53.50 & 245.31 & 43.49 \\
4639539705975935360 & 50.85364 & -74.96868 & 1.11640 & 17.83 & 18.12 & 17.50 & 0.02 & 0.11 & G & 281.88 & 51.92 & 254.78 & 45.17 \\
4690768156035338624 & 18.95551 & -70.54573 & 1.14292 & 17.53 & 17.82 & 17.09 & 0.18 & 0.11 & G & 277.77 & 51.17 & 243.67 & 43.20 \\
4703965697180635136 & 9.31520 & -67.04117 & 1.15729 & 17.89 & 18.12 & 17.43 & 0.17 & 0.11 & G & 275.60 & 50.77 & 234.88 & 41.64 \\
4666616485480394368 & 60.40851 & -69.47789 & 1.15905 & 16.29 & 16.45 & 15.90 & 0.12 & 0.08 & O & 275.34 & 50.72 & 223.60 & 39.64 \\
4691081375113472256 & 20.83822 & -70.57775 & 1.17564 & 17.33 & 17.45 & 17.02 & 0.0 & 0.11 & G & 272.90 & 50.27 & 220.70 & 39.13 \\
4637614151878607232 & 20.74650 & -76.24745 & 1.20857 & 17.80 & 17.95 & 17.36 & 0.1 & 0.11 & G & 268.22 & 49.41 & 223.07 & 39.55 \\
5834840099568788864 & 241.98124 & -58.78225 & 1.23577 & 13.71 & 14.05 & 13.19 & 0.31 & 0.11 & G & 264.51 & 48.73 & 230.11 & 40.80 \\
4636112425153243904 & 16.19343 & -76.86050 & 1.25457 & 17.34 & 17.55 & 16.84 & 0.21 & 0.11 & G & 262.02 & 48.27 & 218.67 & 38.77 \\
4690721839108141568 & 19.01385 & -70.91305 & 1.30481 & 17.25 & 17.73 & 17.00 & -0.0 & 0.11 & G & 255.66 & 47.09 & 246.30 & 43.67 \\
4698739817197286912 & 23.24870 & -66.49795 & 1.30920 & 17.05 & 17.30 & 16.67 & 0.05 & 0.11 & G & 255.13 & 47.00 & 223.23 & 39.58 \\
5298606801235832064 & 140.10591 & -62.22648 & 1.36601 & 18.36 & 18.60 & 17.89 & 0.18 & 0.11 & G & 248.43 & 45.76 & 211.15 & 37.44 \\
5850083595712857472 & 220.66054 & -64.27433 & 1.37135 & 17.67 & 18.47 & 16.71 & 1.23 & 0.15 & G & 247.83 & 45.65 & 210.17 & 37.26 \\
4690414800484275840 & 12.25946 & -70.13797 & 1.37867 & 17.09 & 17.39 & 16.78 & -0.0 & 0.11 & G & 247.00 & 45.50 & 219.47 & 38.91 \\
5935901715187592704 & 255.13630 & -53.09007 & 1.39879 & 15.45 & 15.92 & 14.78 & 0.58 & 0.12 & G & 244.77 & 45.09 & 212.04 & 37.59 \\
5615958881027868544 & 115.24714 & -22.49207 & 1.39928 & 15.46 & 16.23 & 14.69 & 0.89 & 0.11 & O & 244.72 & 45.08 & 224.10 & 39.73 \\
4627114812265929856 & 55.76893 & -76.93405 & 1.42992 & 17.95 & 18.31 & 17.50 & 0.18 & 0.11 & G & 241.42 & 44.47 & 216.52 & 38.39 \\
4690838421706602624 & 15.93439 & -70.90033 & 1.43044 & 17.33 & 17.58 & 16.94 & 0.06 & 0.11 & G & 241.37 & 44.46 & 210.25 & 37.28 \\
4637822960304562560 & 24.11091 & -75.12545 & 1.43113 & 17.25 & 17.49 & 16.82 & 0.11 & 0.11 & G & 241.29 & 44.45 & 208.02 & 36.88 \\
6027070573648725632 & 251.47116 & -33.16585 & 1.45594 & 13.89 & 14.47 & 13.13 & 0.75 & 0.12 & G & 238.71 & 43.97 & 207.84 & 36.85 \\
5321579073778197888 & 130.00710 & -52.33019 & 1.53045 & 15.25 & 15.90 & 14.48 & 0.81 & 0.12 & G & 231.37 & 42.62 & 203.63 & 36.10 \\
6008381624727734784 & 237.76802 & -39.75981 & 1.57244 & 17.10 & 17.91 & 16.20 & 1.12 & 0.14 & G & 227.48 & 41.90 & 197.69 & 35.05 \\
4649187405119614848 & 75.03872 & -75.15255 & 1.57491 & 16.97 & 17.25 & 16.49 & 0.18 & 0.11 & G & 227.26 & 41.86 & 195.43 & 34.65 \\
4108167833903339520 & 259.75244 & -27.43467 & 1.58118 & 16.78 & 17.65 & 15.71 & 1.45 & 0.16 & G & 226.69 & 41.76 & 184.78 & 32.76 \\
4691023998645738368 & 17.49608 & -69.93794 & 1.60821 & 16.70 & 16.83 & 16.30 & 0.0 & 0.11 & G & 224.30 & 41.32 & 185.40 & 32.87 \\
4650261219962135424 & 85.33831 & -74.16668 & 1.62049 & 16.91 & 17.29 & 16.43 & 0.22 & 0.11 & G & 223.23 & 41.12 & 199.23 & 35.32 \\
426580107514101376 & 15.41660 & 60.59426 & 1.62477 & 14.87 & 15.52 & 14.07 & 0.85 & 0.13 & G & 222.87 & 41.05 & 193.24 & 34.26 \\
4684195339947360512 & 6.98869 & -76.24706 & 1.64272 & 17.58 & 17.86 & 17.10 & 0.17 & 0.11 & G & 221.34 & 40.77 & 190.24 & 33.73 \\
2031982665929461504 & 296.05399 & 29.68730 & 1.64410 & 16.22 & 17.13 & 15.31 & 1.2 & 0.14 & G & 221.22 & 40.75 & 195.53 & 34.67 \\
181620805307496192 & 76.98162 & 33.05659 & 1.66805 & 14.61 & 15.30 & 13.80 & 0.88 & 0.13 & G & 219.23 & 40.38 & 191.76 & 34.00 \\
4702506576531479424 & 12.34403 & -69.50825 & 1.68632 & 17.24 & 17.63 & 16.86 & 0.08 & 0.11 & G & 217.74 & 40.11 & 200.62 & 35.57 \\
2021540814501736320 & 293.71912 & 25.61797 & 1.69319 & 17.40 & 18.66 & 16.25 & 1.87 & 0.19 & G & 217.19 & 40.01 & 181.51 & 32.18 \\
4684369749977673472 & 13.14590 & -75.95877 & 1.75282 & 17.35 & 17.52 & 16.89 & 0.09 & 0.11 & G & 212.53 & 39.15 & 176.02 & 31.21 \\
4392367984521092608 & 254.76077 & 4.79169 & 1.77576 & 14.89 & 15.22 & 14.38 & 0.23 & 0.11 & G & 210.81 & 38.83 & 182.05 & 32.28 \\
4652327614621999872 & 70.43479 & -74.41493 & 1.79655 & 16.84 & 16.86 & 16.26 & 0.21 & 0.11 & G & 209.28 & 38.55 & 157.93 & 28.00 \\
5516409029527928064 & 125.97858 & -47.25490 & 1.83399 & 15.20 & 15.90 & 14.37 & 0.91 & 0.13 & G & 206.59 & 38.06 & 179.11 & 31.76 \\
5814577169727787392 & 254.58683 & -67.66312 & 1.85575 & 13.93 & 14.19 & 13.51 & 0.06 & 0.11 & G & 205.07 & 37.78 & 177.09 & 31.40 \\
4189050211325803008 & 299.56897 & -12.07101 & 1.99398 & 17.75 & 18.07 & 17.21 & 0.24 & 0.11 & G & 196.05 & 36.11 & 168.03 & 29.79 \\
252595410453952384 & 67.62787 & 43.65313 & 1.99947 & 13.06 & 14.01 & 12.09 & 1.29 & 0.15 & G & 195.72 & 36.05 & 169.51 & 30.05 \\
5928285810456681344 & 247.54255 & -57.33140 & 2.00665 & 13.64 & 14.08 & 13.01 & 0.44 & 0.11 & G & 195.28 & 35.97 & 169.56 & 30.06 \\
5851830444814064512 & 206.04645 & -65.60886 & 2.02729 & 15.84 & 16.51 & 14.95 & 0.97 & 0.13 & G & 194.03 & 35.74 & 163.09 & 28.92 \\
2928096226097916160 & 109.16266 & -22.18043 & 2.04402 & 14.73 & 15.46 & 13.87 & 0.96 & 0.13 & G & 193.04 & 35.56 & 167.34 & 29.67 \\
5322875157471168768 & 129.59122 & -49.81203 & 2.04472 & 15.13 & 15.93 & 14.31 & 0.92 & 0.13 & G & 192.99 & 35.55 & 172.95 & 30.66 \\
5859972946880769408 & 189.52856 & -66.38308 & 2.06540 & 15.01 & 15.58 & 14.31 & 0.63 & 0.09 & O & 191.78 & 35.33 & 166.54 & 29.53 \\
4636099402811865344 & 19.45728 & -76.56544 & 2.06770 & 16.80 & 17.11 & 16.32 & 0.16 & 0.11 & G & 191.65 & 35.30 & 165.51 & 29.35 \\
6379917835078618752 & 359.03700 & -73.64989 & 2.08819 & 17.15 & 17.32 & 16.70 & 0.05 & 0.11 & G & 190.47 & 35.09 & 157.75 & 27.97 \\
5211831178906807040 & 93.60903 & -79.18168 & 2.09182 & 16.74 & 16.98 & 16.24 & 0.15 & 0.11 & G & 190.26 & 35.05 & 159.82 & 28.34 \\
2162679246615275264 & 315.66755 & 45.09280 & 2.11305 & 16.28 & 17.23 & 15.27 & 1.34 & 0.15 & G & 189.06 & 34.83 & 160.69 & 28.49 \\
200016111582079744 & 73.82548 & 39.97972 & 2.12061 & 13.35 & 13.95 & 12.58 & 0.73 & 0.08 & L & 188.64 & 34.75 & 162.79 & 28.86 \\
5613411827982576768 & 112.81549 & -25.90739 & 2.14810 & 11.58 & 12.04 & 10.97 & 0.29 & 0.08 & O & 187.13 & 34.47 & 177.10 & 31.40 \\
5256605839340504576 & 149.84616 & -60.33354 & 2.30293 & 14.62 & 15.23 & 13.86 & 0.71 & 0.12 & G & 179.15 & 33.00 & 156.16 & 27.69 \\
228673477705878400 & 63.37936 & 41.31878 & 2.31244 & 14.04 & 14.74 & 13.23 & 0.85 & 0.13 & G & 178.69 & 32.92 & 155.94 & 27.65 \\
6377896696484508544 & 355.61170 & -75.25641 & 2.33045 & 17.06 & 17.34 & 16.70 & -0.0 & 0.11 & G & 177.82 & 32.76 & 152.48 & 27.03 \\
5521137101325930624 & 122.45845 & -43.97272 & 2.34215 & 14.33 & 14.88 & 13.65 & 0.56 & 0.11 & G & 177.26 & 32.65 & 155.50 & 27.57 \\
5521712145909463680 & 128.16223 & -46.79047 & 2.36600 & 15.36 & 16.18 & 14.36 & 1.23 & 0.15 & G & 176.14 & 32.45 & 146.23 & 25.93 \\
5534744416711687424 & 119.86019 & -40.02830 & 2.36819 & 14.81 & 15.55 & 13.92 & 0.99 & 0.13 & G & 176.04 & 32.43 & 150.12 & 26.62 \\
4688062360997085440 & 21.38773 & -70.75956 & 2.37759 & 16.60 & 17.05 & 16.33 & 0.0 & 0.11 & G & 175.61 & 32.35 & 158.35 & 28.08 \\
5310255272261039488 & 138.08441 & -55.23391 & 2.39764 & 14.44 & 15.10 & 13.65 & 0.79 & 0.12 & G & 174.68 & 32.18 & 151.83 & 26.92 \\
3134002107923090944 & 101.39057 & 7.81629 & 2.42684 & 12.82 & 13.74 & 12.10 & 0.88 & 0.11 & O & 173.37 & 31.94 & 159.38 & 28.26 \\
4445130042844217216 & 249.98383 & 7.67920 & 2.44837 & 15.83 & 16.15 & 15.32 & 0.18 & 0.11 & G & 172.41 & 31.76 & 147.84 & 26.21 \\
1865228537734352896 & 317.06710 & 32.74552 & 2.45861 & 14.11 & 14.56 & 13.50 & 0.39 & 0.11 & G & 171.96 & 31.68 & 149.84 & 26.57 \\
4650211741937480192 & 86.25630 & -73.56541 & 2.47100 & 16.37 & 16.64 & 15.80 & 0.23 & 0.11 & G & 171.42 & 31.58 & 142.51 & 25.27 \\
207722317998325632 & 80.88983 & 44.76008 & 2.47685 & 12.75 & 13.46 & 11.93 & 0.85 & 0.13 & G & 171.17 & 31.53 & 148.94 & 26.41 \\
523700107035878272 & 14.38545 & 63.15643 & 2.48837 & 13.96 & 14.89 & 13.01 & 1.22 & 0.14 & G & 170.67 & 31.44 & 147.96 & 26.23 \\
5596920115637629184 & 119.15388 & -30.95279 & 2.49448 & 13.91 & 14.77 & 12.99 & 1.15 & 0.12 & O & 170.41 & 31.39 & 143.42 & 25.43 \\
4757183606166564864 & 83.55789 & -63.16699 & 2.50146 & 16.10 & 16.40 & 15.61 & 0.14 & 0.11 & G & 170.11 & 31.34 & 146.36 & 25.95 \\
5329778887909167232 & 131.65005 & -46.52931 & 2.52412 & 15.66 & 16.74 & 14.60 & 1.51 & 0.16 & G & 169.15 & 31.16 & 143.40 & 25.42 \\
5520935444020919296 & 122.93820 & -44.17210 & 2.54078 & 14.99 & 15.78 & 14.08 & 1.05 & 0.14 & G & 168.46 & 31.03 & 143.50 & 25.44 \\
5613111347760892672 & 110.69908 & -26.71455 & 2.54548 & 12.91 & 13.38 & 12.29 & 0.4 & 0.11 & G & 168.26 & 31.00 & 146.61 & 25.99 \\
2934255449716149760 & 107.39410 & -18.56329 & 2.54653 & 13.25 & 14.02 & 12.37 & 0.99 & 0.13 & G & 168.22 & 30.99 & 144.44 & 25.61 \\
5520440663787736192 & 122.44604 & -45.35460 & 2.55121 & 15.84 & 16.42 & 15.08 & 0.69 & 0.12 & G & 168.03 & 30.95 & 144.42 & 25.61 \\
2932101334643047680 & 105.10347 & -20.43170 & 2.55778 & 12.65 & 13.15 & 11.98 & 0.36 & 0.05 & L & 167.76 & 30.90 & 158.77 & 28.15 \\
470144751068871808 & 61.63394 & 58.11309 & 2.57812 & 16.51 & 16.97 & 15.88 & 0.42 & 0.11 & G & 166.93 & 30.75 & 144.63 & 25.64 \\
5597352047599988352 & 119.45786 & -29.38405 & 2.58612 & 11.59 & 12.21 & 10.84 & 0.73 & 0.1 & O & 166.60 & 30.69 & 141.09 & 25.02 \\
5404862853352596736 & 149.21983 & -51.60892 & 2.60474 & 13.30 & 14.09 & 12.41 & 1.0 & 0.11 & O & 165.86 & 30.55 & 144.14 & 25.56 \\
5599566983722741248 & 114.47706 & -29.43804 & 2.62004 & 14.18 & 14.88 & 13.38 & 0.81 & 0.12 & G & 165.25 & 30.44 & 144.41 & 25.60 \\
5617745003304609536 & 109.88037 & -23.80181 & 2.63003 & 14.53 & 15.53 & 13.52 & 1.35 & 0.15 & G & 164.86 & 30.37 & 141.06 & 25.01 \\
2004103831357741696 & 332.32734 & 51.40539 & 2.63200 & 14.84 & 15.40 & 14.13 & 0.59 & 0.12 & G & 164.78 & 30.35 & 143.15 & 25.38 \\
3425576270732293632 & 93.99953 & 23.74749 & 2.63501 & 11.57 & 12.24 & 10.79 & 0.75 & 0.1 & L & 164.66 & 30.33 & 145.55 & 25.81 \\
4690127037676227840 & 13.29901 & -70.85695 & 2.63769 & 16.20 & 16.67 & 15.89 & 0.0 & 0.11 & G & 164.56 & 30.31 & 152.87 & 27.10 \\
5254994264542210560 & 153.53708 & -59.85044 & 2.64145 & 15.11 & 15.96 & 14.18 & 1.08 & 0.12 & O & 164.41 & 30.29 & 144.29 & 25.58 \\
5932284528150696704 & 245.22589 & -53.55461 & 2.64407 & 11.70 & 11.99 & 11.25 & 0.03 & 0.08 & O & 164.31 & 30.27 & 145.71 & 25.83 \\
5857845872913577856 & 199.32909 & -66.11714 & 2.65755 & 15.60 & 16.34 & 14.72 & 0.96 & 0.13 & G & 163.79 & 30.17 & 140.48 & 24.91 \\
198681686717279616 & 72.85353 & 38.18855 & 2.65963 & 13.15 & 13.88 & 12.23 & 0.78 & 0.07 & L & 163.70 & 30.16 & 160.38 & 28.44 \\
5322962499927658880 & 129.02740 & -49.26527 & 2.66635 & 14.82 & 15.62 & 13.88 & 1.1 & 0.14 & G & 163.45 & 30.11 & 137.93 & 24.46 \\
3330259852538068608 & 91.85611 & 11.15198 & 3.88939 & 11.07 & 11.64 & 10.37 & 0.5 & 0.06 & L & 129.04 & 23.77 & 113.96 & 20.21 \\
5611563995612988928 & 112.16780 & -29.34422 & 2.70160 & 12.72 & 13.13 & 12.17 & 0.27 & 0.11 & G & 162.11 & 29.86 & 141.65 & 25.11 \\
3133819112256378368 & 100.02326 & 7.60583 & 2.70467 & 10.13 & 10.86 & 9.35 & 0.74 & 0.08 & L & 161.99 & 29.84 & 148.35 & 26.30 \\
5515778734493663232 & 127.31510 & -46.74924 & 2.71653 & 14.80 & 15.48 & 13.93 & 0.9 & 0.13 & G & 161.55 & 29.76 & 136.87 & 24.27 \\
4688033735040263168 & 23.36268 & -70.67097 & 2.74408 & 16.45 & 16.67 & 16.04 & -0.0 & 0.11 & G & 160.53 & 29.57 & 134.47 & 23.84 \\
5280590173638560128 & 104.74084 & -68.31085 & 2.75554 & 15.96 & 16.28 & 15.44 & 0.17 & 0.11 & G & 160.11 & 29.49 & 137.01 & 24.29 \\
355488086540394112 & 35.70997 & 50.07193 & 2.75989 & 14.54 & 14.96 & 13.95 & 0.32 & 0.11 & G & 159.96 & 29.47 & 138.60 & 24.57 \\
5520506531407532928 & 121.80022 & -45.06591 & 2.77254 & 14.02 & 14.57 & 13.29 & 0.6 & 0.12 & G & 159.50 & 29.38 & 137.53 & 24.38 \\
5545066700588440832 & 119.73893 & -36.89733 & 2.77514 & 15.07 & 16.06 & 14.05 & 1.35 & 0.15 & G & 159.41 & 29.36 & 135.63 & 24.05 \\
4637956099996538752 & 18.33566 & -75.37716 & 2.77979 & 16.46 & 16.76 & 15.98 & 0.11 & 0.11 & G & 159.24 & 29.33 & 136.37 & 24.18 \\
2948568273607650560 & 105.01213 & -14.16082 & 2.78195 & 13.90 & 14.80 & 13.11 & 0.91 & 0.13 & G & 159.16 & 29.32 & 146.98 & 26.06 \\
4066429066901946368 & 273.26040 & -23.11729 & 5.05787 & 6.82 & 7.37 & 6.23 & 0.25 & 0.03 & L & 109.48 & 20.17 & 101.17 & 17.94 \\
460909093912435072 & 42.02334 & 57.93448 & 2.79873 & 14.03 & 15.07 & 13.01 & 1.39 & 0.15 & G & 158.56 & 29.21 & 135.50 & 24.02 \\
430052537038350976 & 0.60589 & 62.84717 & 2.81345 & 14.41 & 15.25 & 13.49 & 1.08 & 0.14 & G & 158.04 & 29.11 & 136.12 & 24.13 \\
1873298884367855872 & 314.17890 & 40.25849 & 2.82245 & 16.21 & 17.13 & 15.23 & 1.25 & 0.15 & G & 157.73 & 29.05 & 134.27 & 23.81 \\
5616130129962210048 & 110.43814 & -26.53341 & 2.82545 & 12.91 & 13.38 & 12.30 & 0.37 & 0.11 & G & 157.62 & 29.04 & 137.83 & 24.44 \\
3117307814859500416 & 97.77268 & -2.14679 & 3.13523 & 13.29 & 14.09 & 12.47 & 0.9 & 0.12 & L & 147.68 & 27.20 & 128.89 & 22.85 \\
5293246995583678336 & 109.08524 & -60.30341 & 2.84929 & 15.52 & 16.19 & 14.69 & 0.83 & 0.13 & G & 156.80 & 28.88 & 134.04 & 23.76 \\
5544259212380322560 & 120.85675 & -37.19998 & 2.85529 & 14.09 & 14.84 & 13.23 & 0.93 & 0.11 & O & 156.59 & 28.84 & 133.78 & 23.72 \\
2928335747830554240 & 108.43497 & -21.72421 & 2.86166 & 14.22 & 14.98 & 13.36 & 0.94 & 0.13 & G & 156.37 & 28.80 & 135.46 & 24.02 \\
4757607983288353024 & 83.76190 & -62.33990 & 2.86849 & 16.03 & 16.25 & 15.52 & 0.12 & 0.11 & G & 156.14 & 28.76 & 128.93 & 22.86 \\
513074186146353536 & 24.74994 & 64.98924 & 2.87151 & 11.01 & 11.84 & 10.14 & 1.03 & 0.11 & L & 156.04 & 28.74 & 133.53 & 23.67 \\
4688114725237948672 & 24.52435 & -70.61840 & 2.88021 & 16.38 & 16.64 & 15.99 & -0.0 & 0.11 & G & 155.74 & 28.69 & 131.37 & 23.29 \\
261927068718088832 & 81.89283 & 50.86737 & 2.88526 & 13.17 & 13.81 & 12.41 & 0.7 & 0.12 & G & 155.57 & 28.66 & 135.57 & 24.04 \\
4682206533865906944 & 65.11048 & -57.85114 & 2.89258 & 15.71 & 16.00 & 15.30 & -0.0 & 0.11 & G & 155.32 & 28.61 & 135.39 & 24.00 \\
5253289093802878592 & 152.85139 & -61.48616 & 2.91146 & 14.11 & 14.59 & 13.44 & 0.46 & 0.11 & G & 154.69 & 28.50 & 133.37 & 23.65 \\
2947842664653933824 & 104.19146 & -15.63763 & 3.69400 & 13.25 & 13.97 & 12.43 & 0.81 & 0.12 & G & 133.27 & 24.55 & 115.38 & 20.46 \\
5310969267622303872 & 136.56210 & -54.93719 & 2.92762 & 14.52 & 15.11 & 13.78 & 0.63 & 0.12 & G & 154.16 & 28.40 & 133.96 & 23.75 \\
4642866828161408512 & 52.89342 & -70.99389 & 2.92900 & 16.29 & 16.60 & 15.82 & 0.08 & 0.11 & G & 154.11 & 28.39 & 133.66 & 23.70 \\
5533064637824258816 & 119.78798 & -43.17517 & 2.92921 & 13.49 & 13.98 & 12.84 & 0.45 & 0.11 & G & 154.10 & 28.39 & 134.05 & 23.77 \\
5598642947280233984 & 116.71718 & -30.66590 & 2.96840 & 14.15 & 14.95 & 13.28 & 0.97 & 0.11 & O & 152.83 & 28.15 & 132.41 & 23.48 \\
5856662557855409280 & 187.47093 & -68.27871 & 2.98190 & 14.44 & 14.92 & 13.79 & 0.44 & 0.11 & G & 152.39 & 28.07 & 132.05 & 23.41 \\
5318708901756763520 & 131.02834 & -51.91945 & 2.98495 & 15.08 & 15.82 & 14.23 & 0.89 & 0.13 & G & 152.30 & 28.05 & 132.07 & 23.42 \\
4265371574109405824 & 284.35111 & -0.73024 & 2.98806 & 10.56 & 11.32 & 9.69 & 0.99 & 0.14 & L & 152.20 & 28.04 & 127.75 & 22.65 \\
5519861423017907840 & 124.43265 & -45.18550 & 3.00610 & 14.46 & 15.24 & 13.61 & 0.93 & 0.13 & G & 151.62 & 27.93 & 132.55 & 23.50 \\
5241937353463150848 & 162.59092 & -62.19142 & 3.02574 & 15.21 & 16.09 & 14.26 & 1.16 & 0.12 & O & 151.01 & 27.82 & 127.86 & 22.67 \\
466906311366699520 & 48.44587 & 63.34948 & 3.03268 & 13.18 & 14.11 & 12.24 & 1.17 & 0.14 & G & 150.79 & 27.78 & 130.85 & 23.20 \\
5252269709082759936 & 156.40361 & -62.55651 & 3.04556 & 15.10 & 15.67 & 14.35 & 0.64 & 0.12 & G & 150.39 & 27.70 & 128.84 & 22.84 \\
5310863370918375552 & 140.55281 & -53.06412 & 3.05163 & 13.60 & 14.46 & 12.66 & 1.11 & 0.12 & O & 150.20 & 27.67 & 129.35 & 22.93 \\
5863815636949490048 & 202.86552 & -65.32720 & 3.06221 & 15.68 & 16.55 & 14.75 & 1.08 & 0.12 & O & 149.88 & 27.61 & 132.22 & 23.44 \\
2930525287803260288 & 109.84202 & -19.54033 & 3.07149 & 12.79 & 13.35 & 12.07 & 0.57 & 0.09 & O & 149.60 & 27.56 & 130.12 & 23.07 \\
5858259014403682304 & 195.97407 & -66.33292 & 3.08394 & 15.37 & 16.09 & 14.47 & 0.95 & 0.11 & O & 149.22 & 27.49 & 126.48 & 22.43 \\
5235910694044165760 & 176.13694 & -67.30525 & 3.08613 & 8.70 & 9.22 & 8.06 & 0.43 & 0.06 & L & 149.15 & 27.47 & 130.96 & 23.22 \\
5237406545247540608 & 171.64645 & -65.58218 & 3.11677 & 14.99 & 15.84 & 14.04 & 1.12 & 0.14 & G & 148.23 & 27.31 & 125.96 & 22.33 \\
5335753015664095104 & 173.80588 & -60.91465 & 3.12750 & 14.19 & 14.98 & 13.30 & 1.0 & 0.11 & O & 147.91 & 27.25 & 126.73 & 22.47 \\
5594991812757424768 & 115.97856 & -32.50378 & 3.14920 & 14.81 & 15.79 & 13.80 & 1.33 & 0.15 & G & 147.27 & 27.13 & 124.40 & 22.06 \\
2932737092877188352 & 105.22172 & -19.45929 & 3.15504 & 12.36 & 12.85 & 11.73 & 0.4 & 0.11 & G & 147.10 & 27.10 & 128.89 & 22.85 \\
2059517087110475392 & 299.88745 & 36.02152 & 3.16632 & 15.16 & 16.04 & 14.20 & 1.16 & 0.14 & G & 146.78 & 27.04 & 124.65 & 22.10 \\
5329323277776517120 & 130.36480 & -47.64966 & 3.17573 & 14.05 & 14.90 & 13.10 & 1.13 & 0.14 & G & 146.50 & 26.99 & 124.24 & 22.03 \\
5239658688657671680 & 160.70962 & -65.55805 & 3.18304 & 16.74 & 17.37 & 16.02 & 0.6 & 0.12 & G & 146.29 & 26.95 & 129.47 & 22.95 \\
5322878146768508800 & 129.73194 & -49.77016 & 3.18474 & 14.62 & 15.39 & 13.75 & 0.94 & 0.13 & G & 146.24 & 26.94 & 126.17 & 22.37 \\
5612661716228387200 & 111.62263 & -27.92502 & 3.18518 & 12.78 & 13.26 & 12.14 & 0.41 & 0.11 & G & 146.23 & 26.94 & 127.26 & 22.56 \\
377753613615880832 & 14.89365 & 45.40672 & 3.20017 & 11.48 & 11.87 & 10.98 & 0.16 & 0.11 & G & 145.80 & 26.86 & 128.41 & 22.77 \\
5875602191067578752 & 230.82679 & -61.21710 & 3.23038 & 15.66 & 16.48 & 14.71 & 1.1 & 0.14 & G & 144.95 & 26.70 & 122.06 & 21.64 \\
512491028363231616 & 24.35667 & 63.69136 & 3.23980 & 13.13 & 14.16 & 12.13 & 1.33 & 0.15 & G & 144.68 & 26.65 & 124.23 & 22.03 \\
4513100717859042176 & 286.49619 & 16.09800 & 3.26984 & 13.47 & 14.24 & 12.60 & 0.93 & 0.13 & G & 143.85 & 26.50 & 124.57 & 22.09 \\
5617316606087829888 & 109.16777 & -24.50300 & 3.27499 & 12.80 & 13.31 & 12.13 & 0.47 & 0.11 & G & 143.71 & 26.47 & 124.63 & 22.10 \\
5520505328816739584 & 121.80935 & -45.12830 & 3.28292 & 13.45 & 14.07 & 12.67 & 0.69 & 0.12 & G & 143.49 & 26.43 & 123.60 & 21.91 \\
5241803217391469568 & 165.52136 & -62.28989 & 3.28899 & 14.54 & 15.40 & 13.59 & 1.1 & 0.12 & O & 143.32 & 26.40 & 123.77 & 21.94 \\
279382060625871360 & 76.63188 & 55.35352 & 3.29487 & 7.19 & 7.81 & 6.48 & 0.55 & 0.07 & L & 143.16 & 26.37 & 130.06 & 23.06 \\
5405496240766414464 & 148.01595 & -51.99247 & 3.29644 & 13.56 & 14.38 & 12.67 & 1.01 & 0.11 & O & 143.12 & 26.36 & 122.67 & 21.75 \\
505178760644698880 & 31.25913 & 57.14294 & 3.29700 & 12.34 & 12.82 & 11.68 & 0.35 & 0.05 & L & 143.11 & 26.36 & 129.92 & 23.03 \\
5306043592977093504 & 145.89770 & -57.23830 & 3.00860 & 15.29 & 16.16 & 14.31 & 1.23 & 0.13 & O & 151.55 & 27.92 & 124.51 & 22.07 \\
505368121464666112 & 29.62897 & 57.81985 & 3.32910 & 13.78 & 14.44 & 12.98 & 0.74 & 0.12 & G & 142.24 & 26.20 & 123.27 & 21.86 \\
5600862070985787136 & 119.26547 & -28.16158 & 3.33098 & 11.61 & 12.25 & 10.88 & 0.58 & 0.09 & O & 142.19 & 26.19 & 129.95 & 23.04 \\
5605736961940589568 & 110.81312 & -29.72244 & 3.33617 & 12.87 & 13.38 & 12.30 & 0.3 & 0.11 & G & 142.05 & 26.17 & 127.69 & 22.64 \\
5313250548085699712 & 139.88405 & -51.62042 & 3.35503 & 12.70 & 13.62 & 11.69 & 1.34 & 0.13 & O & 141.55 & 26.07 & 113.65 & 20.15 \\
5516452460238707968 & 125.52706 & -47.30395 & 3.36831 & 14.28 & 14.93 & 13.46 & 0.77 & 0.12 & G & 141.20 & 26.01 & 120.90 & 21.44 \\
2073935223599391872 & 300.89457 & 39.15963 & 3.37031 & 13.22 & 13.96 & 12.38 & 1.02 & 0.13 & L & 141.15 & 26.00 & 110.77 & 19.64 \\
5592331544376193792 & 113.82822 & -31.66418 & 3.38307 & 13.77 & 14.53 & 12.93 & 0.87 & 0.13 & G & 140.82 & 25.94 & 123.09 & 21.82 \\
5824464493705913472 & 229.94041 & -66.49608 & 3.38932 & 6.44 & 6.86 & 5.91 & 0.23 & 0.04 & L & 140.65 & 25.91 & 122.58 & 21.73 \\
5598852026287511424 & 116.00045 & -30.14146 & 3.39082 & 13.12 & 13.66 & 12.45 & 0.58 & 0.09 & O & 140.61 & 25.90 & 115.65 & 20.51 \\
2025217890612425344 & 293.14591 & 26.80479 & 3.39154 & 15.51 & 16.38 & 14.54 & 1.15 & 0.14 & G & 140.60 & 25.90 & 118.60 & 21.03 \\
5857294605251013760 & 193.30159 & -67.96426 & 3.40117 & 14.41 & 14.91 & 13.73 & 0.48 & 0.11 & G & 140.35 & 25.85 & 120.94 & 21.44 \\
206211859601169792 & 74.06344 & 44.78185 & 3.40680 & 12.54 & 13.43 & 11.62 & 1.1 & 0.14 & G & 140.20 & 25.83 & 121.28 & 21.50 \\
189739251272296192 & 85.62191 & 37.64633 & 3.41272 & 12.05 & 12.93 & 11.18 & 0.84 & 0.11 & L & 140.05 & 25.80 & 137.19 & 24.32 \\
4690436069162376576 & 10.68389 & -70.27426 & 3.42463 & 16.23 & 16.48 & 15.74 & 0.07 & 0.11 & G & 139.74 & 25.74 & 117.60 & 20.85 \\
5932997939411720960 & 243.72813 & -53.33844 & 3.45291 & 9.79 & 10.63 & 8.92 & 0.92 & 0.08 & L & 139.03 & 25.61 & 125.13 & 22.19 \\
3051144427784813824 & 103.54766 & -7.66438 & 3.45403 & 13.28 & 13.98 & 12.44 & 0.85 & 0.11 & L & 139.00 & 25.60 & 118.21 & 20.96 \\
5547358117187868288 & 122.79503 & -33.51586 & 3.48218 & 10.44 & 11.05 & 9.72 & 0.58 & 0.06 & L & 138.29 & 25.47 & 121.98 & 21.63 \\
5310265099146146816 & 138.32401 & -54.93121 & 3.50424 & 14.23 & 15.01 & 13.34 & 0.96 & 0.13 & G & 137.75 & 25.37 & 118.35 & 20.98 \\
515527570241664512 & 34.14985 & 65.17655 & 3.52190 & 12.69 & 13.52 & 11.78 & 1.02 & 0.13 & G & 137.31 & 25.29 & 118.06 & 20.93 \\
2936165984303583360 & 105.87696 & -15.54334 & 3.52281 & 13.45 & 14.09 & 12.65 & 0.73 & 0.12 & G & 137.29 & 25.29 & 117.81 & 20.89 \\
5268616973048513664 & 107.46385 & -68.48372 & 3.52627 & 15.80 & 16.25 & 15.26 & 0.23 & 0.11 & G & 137.21 & 25.27 & 121.59 & 21.56 \\
5618354751226656640 & 112.51063 & -23.67398 & 3.54416 & 13.26 & 14.12 & 12.36 & 1.08 & 0.14 & L & 136.77 & 25.19 & 115.15 & 20.42 \\
5612495762995320576 & 113.72248 & -26.85579 & 3.55250 & 13.56 & 14.36 & 12.63 & 1.03 & 0.13 & G & 136.57 & 25.16 & 116.02 & 20.57 \\
5547421437881152256 & 122.36346 & -33.26212 & 3.56310 & 11.82 & 12.44 & 11.06 & 0.8 & 0.1 & O & 136.32 & 25.11 & 107.33 & 19.03 \\
2162640763705905920 & 316.08941 & 45.23937 & 3.56914 & 13.70 & 14.61 & 12.76 & 1.13 & 0.14 & G & 136.17 & 25.08 & 117.69 & 20.87 \\
5311139245252191616 & 137.38339 & -53.98770 & 3.59050 & 11.68 & 12.22 & 11.02 & 0.44 & 0.11 & G & 135.67 & 24.99 & 119.08 & 21.11 \\
5599370549100412544 & 114.32029 & -29.60773 & 3.59160 & 14.17 & 15.06 & 13.23 & 1.12 & 0.14 & G & 135.64 & 24.99 & 116.62 & 20.68 \\
2952257272558933248 & 101.92934 & -13.66668 & 4.85729 & 11.71 & 12.23 & 10.93 & 0.57 & 0.12 & G & 112.28 & 20.68 & 93.58 & 16.59 \\
3441484760885586176 & 86.43715 & 27.06790 & 3.62280 & 11.67 & 12.56 & 10.71 & 1.13 & 0.15 & L & 134.91 & 24.85 & 116.22 & 20.61 \\
429562773322439296 & 3.51343 & 60.98626 & 3.63045 & 11.91 & 12.73 & 11.01 & 0.99 & 0.13 & L & 134.73 & 24.82 & 117.57 & 20.85 \\
457807268533229056 & 38.46902 & 57.02750 & 3.64942 & 11.13 & 11.84 & 10.31 & 0.84 & 0.08 & L & 134.29 & 24.74 & 113.64 & 20.15 \\
5329405672431387648 & 130.00864 & -47.19842 & 3.67080 & 13.98 & 14.88 & 13.03 & 1.14 & 0.14 & G & 133.80 & 24.65 & 114.56 & 20.31 \\
5351721738384434048 & 157.29679 & -57.61339 & 3.68221 & 8.08 & 8.45 & 7.59 & 0.14 & 0.03 & L & 133.54 & 24.60 & 114.45 & 20.29 \\
5542528959037609984 & 127.24360 & -36.23207 & 3.70536 & 11.33 & 12.03 & 10.52 & 0.77 & 0.12 & G & 133.02 & 24.50 & 115.26 & 20.44 \\
5539023922122441728 & 118.71081 & -37.62246 & 3.70789 & 12.47 & 13.45 & 11.50 & 1.23 & 0.15 & G & 132.96 & 24.49 & 114.42 & 20.29 \\
4707044742055169152 & 9.21974 & -66.59323 & 3.72828 & 16.74 & 17.10 & 16.23 & 0.14 & 0.11 & G & 132.51 & 24.41 & 115.18 & 20.42 \\
2202500843341252736 & 328.64443 & 59.12168 & 3.75817 & 13.83 & 14.85 & 12.81 & 1.34 & 0.15 & G & 131.85 & 24.29 & 111.95 & 19.85 \\
2200018111723748224 & 335.91092 & 57.68078 & 3.76750 & 11.66 & 12.55 & 10.75 & 1.06 & 0.14 & L & 131.64 & 24.25 & 114.26 & 20.26 \\
3445039825569144192 & 86.71173 & 31.59791 & 3.04664 & 11.88 & 12.55 & 11.09 & 0.76 & 0.1 & L & 150.36 & 27.70 & 130.52 & 23.14 \\
3378049163365268608 & 100.78130 & 20.93911 & 3.78798 & 9.70 & 10.10 & 9.22 & 0.28 & 0.07 & L & 131.19 & 24.17 & 104.58 & 18.54 \\
5856994365517642112 & 194.75148 & -68.57855 & 3.79741 & 13.12 & 13.58 & 12.60 & 0.19 & 0.11 & G & 130.99 & 24.13 & 117.37 & 20.81 \\
5311409896910828800 & 137.14651 & -53.19702 & 3.80582 & 13.72 & 14.48 & 12.86 & 0.89 & 0.13 & G & 130.81 & 24.10 & 113.12 & 20.06 \\
430647231080076416 & 5.01280 & 63.17979 & 3.81071 & 11.68 & 12.53 & 10.74 & 1.01 & 0.13 & L & 130.70 & 24.08 & 116.56 & 20.67 \\
465719182408723072 & 41.18048 & 61.46470 & 3.83288 & 10.43 & 11.14 & 9.64 & 0.76 & 0.09 & L & 130.23 & 23.99 & 112.44 & 19.94 \\
6059635702888301952 & 190.35842 & -59.79419 & 3.83834 & 7.99 & 8.43 & 7.42 & 0.33 & 0.04 & L & 130.11 & 23.97 & 109.04 & 19.33 \\
509629965971797376 & 25.81989 & 59.99762 & 3.84314 & 12.33 & 13.18 & 11.42 & 1.02 & 0.13 & G & 130.01 & 23.95 & 112.09 & 19.87 \\
2031776202613700480 & 296.20306 & 29.26468 & 3.84599 & 6.69 & 7.01 & 6.22 & 0.17 & 0.04 & L & 129.95 & 23.94 & 104.24 & 18.48 \\
2012494342018730496 & 353.33454 & 61.11907 & 3.87118 & 12.21 & 13.18 & 11.23 & 1.22 & 0.14 & G & 129.42 & 23.84 & 110.86 & 19.65 \\
5619369359933924992 & 111.25618 & -23.15791 & 3.89113 & 13.75 & 14.75 & 12.76 & 1.26 & 0.15 & G & 129.01 & 23.76 & 110.43 & 19.58 \\
2072235820984829312 & 299.71473 & 37.64725 & 3.89187 & 14.29 & 14.88 & 13.51 & 0.67 & 0.12 & G & 128.99 & 23.76 & 109.48 & 19.41 \\
2072329902270080128 & 299.38702 & 38.09177 & 3.89671 & 13.59 & 14.22 & 12.81 & 0.68 & 0.12 & G & 128.89 & 23.74 & 110.65 & 19.62 \\
5335934297643679360 & 172.92831 & -60.73455 & 3.89770 & 13.14 & 13.88 & 12.32 & 0.78 & 0.1 & O & 128.87 & 23.74 & 114.23 & 20.25 \\
4253603501158148736 & 280.61175 & -5.34085 & 3.91771 & 10.51 & 11.41 & 9.60 & 1.05 & 0.1 & L & 128.46 & 23.66 & 112.95 & 20.03 \\
5615233993628681216 & 112.66125 & -24.68752 & 3.91882 & 13.09 & 13.87 & 12.21 & 0.91 & 0.11 & O & 128.44 & 23.66 & 112.15 & 19.88 \\
2010134274671099264 & 345.33801 & 57.86702 & 3.91921 & 11.49 & 12.30 & 10.62 & 0.92 & 0.12 & L & 128.43 & 23.66 & 112.91 & 20.02 \\
3052092481686246016 & 107.65830 & -7.12290 & 3.28782 & 12.52 & 13.23 & 11.64 & 0.68 & 0.09 & L & 143.36 & 26.41 & 140.03 & 24.83 \\
5540422122959807232 & 125.36087 & -38.42170 & 3.96098 & 12.55 & 13.54 & 11.57 & 1.22 & 0.13 & O & 127.58 & 23.50 & 110.53 & 19.60 \\
5606739884038472704 & 109.26954 & -28.82351 & 3.96993 & 12.72 & 13.24 & 12.05 & 0.45 & 0.11 & G & 127.40 & 23.47 & 110.42 & 19.58 \\
486834100624652800 & 54.08395 & 62.28723 & 3.99690 & 12.74 & 13.79 & 11.72 & 1.31 & 0.17 & L & 126.86 & 23.37 & 110.88 & 19.66 \\
2015458213056909184 & 351.49362 & 61.26683 & 4.00024 & 12.51 & 13.36 & 11.59 & 0.92 & 0.12 & L & 126.79 & 23.36 & 117.37 & 20.81 \\
506923449381427968 & 32.69322 & 59.25369 & 4.00720 & 12.24 & 13.07 & 11.35 & 0.94 & 0.12 & L & 126.65 & 23.33 & 112.25 & 19.90 \\
5238994102591371776 & 162.35781 & -66.62534 & 4.01417 & 14.04 & 14.61 & 13.31 & 0.56 & 0.11 & G & 126.52 & 23.31 & 109.25 & 19.37 \\
514674933331699584 & 32.62154 & 63.29753 & 4.03790 & 10.27 & 10.96 & 9.49 & 0.76 & 0.1 & L & 126.05 & 23.22 & 106.14 & 18.82 \\
2166861170366710272 & 313.73970 & 47.53379 & 4.04921 & 10.29 & 11.11 & 9.41 & 1.02 & 0.13 & L & 125.83 & 23.18 & 104.29 & 18.49 \\
5242076514741190272 & 162.97536 & -61.46728 & 4.05483 & 12.23 & 12.91 & 11.45 & 0.68 & 0.1 & O & 125.72 & 23.16 & 111.91 & 19.84 \\
5530071831587999232 & 129.78343 & -37.37551 & 4.06392 & 12.24 & 12.87 & 11.48 & 0.66 & 0.09 & O & 125.55 & 23.13 & 107.31 & 19.03 \\
422923956470923008 & 3.79087 & 58.42428 & 4.07117 & 9.54 & 10.14 & 8.83 & 0.61 & 0.06 & L & 125.41 & 23.10 & 105.27 & 18.66 \\
5545837900614099584 & 121.29597 & -34.36027 & 4.08860 & 11.73 & 12.56 & 10.84 & 0.9 & 0.11 & O & 125.07 & 23.04 & 112.92 & 20.02 \\
5254281334339678208 & 160.11285 & -60.07640 & 4.08916 & 13.97 & 14.91 & 12.96 & 1.25 & 0.15 & G & 125.06 & 23.04 & 104.89 & 18.60 \\
5241961409628951296 & 162.73299 & -62.09798 & 4.09530 & 14.32 & 15.12 & 13.43 & 0.99 & 0.11 & O & 124.94 & 23.02 & 105.05 & 18.62 \\
5861648327739540736 & 193.74820 & -65.20062 & 4.10167 & 14.64 & 15.63 & 13.62 & 1.28 & 0.13 & O & 124.82 & 22.99 & 106.69 & 18.92 \\
511706805997227648 & 25.25207 & 63.05553 & 4.13309 & 12.66 & 13.61 & 11.69 & 1.19 & 0.14 & G & 124.23 & 22.88 & 106.37 & 18.86 \\
3127458403130026112 & 101.78917 & 3.96710 & 4.13423 & 10.21 & 10.72 & 9.53 & 0.42 & 0.04 & L & 124.20 & 22.88 & 108.56 & 19.25 \\
462252662762965120 & 50.94951 & 59.35567 & 4.15636 & 11.84 & 12.87 & 10.84 & 1.22 & 0.16 & L & 123.79 & 22.80 & 111.23 & 19.72 \\
5321257604065975040 & 128.76428 & -52.47757 & 4.15812 & 14.51 & 15.28 & 13.68 & 0.83 & 0.13 & G & 123.76 & 22.80 & 108.25 & 19.19 \\
2031590552598614784 & 295.87018 & 29.23810 & 4.15973 & 14.49 & 15.30 & 13.56 & 1.02 & 0.13 & G & 123.73 & 22.79 & 104.88 & 18.60 \\
5852389305960163328 & 208.75541 & -64.03195 & 4.16962 & 11.28 & 12.18 & 10.36 & 1.06 & 0.14 & G & 123.54 & 22.76 & 107.31 & 19.03 \\
5614191175568405376 & 115.20408 & -25.45771 & 4.17117 & 12.42 & 13.36 & 11.45 & 1.15 & 0.12 & O & 123.51 & 22.75 & 107.37 & 19.04 \\
5619786177922254336 & 110.28102 & -21.51060 & 4.17560 & 12.51 & 13.26 & 11.67 & 0.82 & 0.1 & O & 123.43 & 22.74 & 108.01 & 19.15 \\
2934506447605426944 & 105.97944 & -17.87991 & 4.20487 & 11.59 & 12.31 & 10.79 & 0.75 & 0.12 & G & 122.89 & 22.64 & 107.23 & 19.01 \\
4690834328595493760 & 16.04228 & -70.95614 & 4.20529 & 15.60 & 15.92 & 15.22 & 0.0 & 0.11 & G & 122.89 & 22.64 & 103.00 & 18.26 \\
5253875717619475200 & 158.46303 & -61.80622 & 4.23097 & 14.74 & 15.57 & 13.80 & 1.07 & 0.12 & O & 122.42 & 22.55 & 102.30 & 18.14 \\
1981367545804985088 & 329.05685 & 52.98601 & 4.23698 & 11.95 & 12.85 & 11.02 & 1.07 & 0.14 & G & 122.31 & 22.53 & 105.32 & 18.67 \\
515832929535462016 & 41.08082 & 64.76592 & 4.23841 & 10.96 & 11.83 & 10.06 & 1.01 & 0.13 & G & 122.28 & 22.53 & 106.40 & 18.87 \\
5254653759541047424 & 155.20707 & -61.25195 & 4.23925 & 13.98 & 14.57 & 13.25 & 0.57 & 0.12 & G & 122.27 & 22.52 & 105.78 & 18.75 \\
5587972801102905984 & 113.75856 & -35.91299 & 4.24340 & 12.16 & 12.74 & 11.47 & 0.5 & 0.11 & G & 122.19 & 22.51 & 106.66 & 18.91 \\
5521352536886237952 & 123.41069 & -42.69920 & 4.24935 & 13.62 & 14.40 & 12.76 & 0.89 & 0.13 & G & 122.09 & 22.49 & 105.34 & 18.68 \\
3027940437469882880 & 110.38690 & -16.68722 & 4.25689 & 9.32 & 9.95 & 8.59 & 0.64 & 0.06 & L & 121.95 & 22.46 & 102.92 & 18.25 \\
522468168674975616 & 18.17150 & 61.21335 & 4.25925 & 10.96 & 11.64 & 10.19 & 0.63 & 0.07 & L & 121.91 & 22.46 & 109.76 & 19.46 \\
5338024572321721216 & 164.46108 & -60.74208 & 4.26618 & 9.44 & 9.99 & 8.79 & 0.55 & 0.07 & L & 121.79 & 22.43 & 98.39 & 17.44 \\
510584788742165760 & 19.00502 & 61.62071 & 4.27770 & 11.35 & 12.36 & 10.37 & 1.16 & 0.15 & L & 121.58 & 22.40 & 110.40 & 19.57 \\
2014609252631258496 & 342.09618 & 60.40476 & 4.27863 & 11.57 & 12.60 & 10.58 & 1.27 & 0.15 & G & 121.56 & 22.39 & 104.95 & 18.61 \\
5620400182140135168 & 112.95453 & -20.14966 & 4.28543 & 10.96 & 11.65 & 10.18 & 0.67 & 0.06 & L & 121.44 & 22.37 & 107.98 & 19.14 \\
2033008274099620480 & 296.26534 & 31.33077 & 4.28897 & 12.25 & 13.01 & 11.39 & 0.87 & 0.11 & L & 121.38 & 22.36 & 104.31 & 18.49 \\
228741784865956224 & 64.27528 & 41.73183 & 4.29045 & 10.67 & 11.41 & 9.90 & 0.72 & 0.09 & L & 121.35 & 22.35 & 107.04 & 18.98 \\
429890595286480384 & 0.67404 & 61.86107 & 4.30528 & 12.11 & 13.08 & 11.13 & 0.99 & 0.13 & L & 121.09 & 22.31 & 119.51 & 21.19 \\
1977074811892425600 & 332.26210 & 51.04585 & 4.32355 & 8.96 & 9.40 & 8.39 & 0.29 & 0.04 & L & 120.77 & 22.25 & 102.21 & 18.12 \\
2074102933481447808 & 301.83830 & 40.17809 & 4.32699 & 13.77 & 14.52 & 12.91 & 0.82 & 0.08 & L & 120.71 & 22.24 & 106.25 & 18.84 \\
5311298983669288832 & 136.84989 & -54.09276 & 4.35093 & 13.37 & 13.93 & 12.65 & 0.52 & 0.11 & G & 120.30 & 22.16 & 103.83 & 18.41 \\
2060021625508894592 & 302.28232 & 37.15195 & 4.36470 & 9.49 & 10.10 & 8.77 & 0.61 & 0.1 & L & 120.06 & 22.12 & 100.66 & 17.85 \\
429385923752386944 & 0.24680 & 60.95900 & 4.36516 & 10.86 & 11.53 & 9.96 & 0.9 & 0.07 & L & 120.05 & 22.11 & 97.53 & 17.29 \\
2006033847910275584 & 335.02002 & 56.06090 & 4.36625 & 12.13 & 12.97 & 11.21 & 1.01 & 0.13 & G & 120.03 & 22.11 & 102.76 & 18.22 \\
204588190167650048 & 71.39513 & 43.57284 & 4.37214 & 13.22 & 14.18 & 12.25 & 1.19 & 0.14 & G & 119.93 & 22.09 & 102.51 & 18.17 \\
4693901042617667584 & 27.66874 & -70.50366 & 4.37264 & 15.68 & 15.92 & 15.29 & 0.0 & 0.11 & G & 119.92 & 22.09 & 95.77 & 16.98 \\
5594091823824942464 & 119.66611 & -33.50405 & 4.40279 & 11.64 & 12.44 & 10.78 & 0.84 & 0.1 & O & 119.41 & 22.00 & 107.69 & 19.09 \\
197337185858157440 & 84.11148 & 44.59136 & 4.40345 & 11.82 & 12.43 & 11.25 & 0.48 & 0.06 & L & 119.39 & 21.99 & 99.22 & 17.59 \\
6055722403534963840 & 195.79449 & -60.87747 & 4.42452 & 9.46 & 10.21 & 8.65 & 0.78 & 0.08 & L & 119.04 & 21.93 & 104.00 & 18.44 \\
3397212822106196992 & 81.77704 & 16.93643 & 4.43840 & 12.75 & 13.32 & 12.06 & 0.48 & 0.11 & G & 118.81 & 21.88 & 104.10 & 18.46 \\
2936110669428633216 & 106.65835 & -15.80206 & 4.46484 & 12.42 & 13.21 & 11.56 & 0.82 & 0.1 & O & 118.36 & 21.80 & 106.60 & 18.90 \\
5881952871520184960 & 234.52125 & -58.69441 & 4.47575 & 15.24 & 16.25 & 14.22 & 1.32 & 0.13 & O & 118.18 & 21.77 & 99.06 & 17.56 \\
2011892320749270912 & 359.53791 & 61.21363 & 4.47861 & 10.57 & 11.12 & 9.66 & 0.74 & 0.07 & L & 118.14 & 21.76 & 99.57 & 17.65 \\
2005011237689458688 & 335.31995 & 54.53204 & 4.47944 & 11.44 & 12.16 & 10.63 & 0.76 & 0.07 & L & 118.12 & 21.76 & 101.92 & 18.07 \\
5254078504458244352 & 160.72436 & -61.02361 & 4.48366 & 12.84 & 13.68 & 11.94 & 0.97 & 0.11 & O & 118.05 & 21.75 & 102.18 & 18.12 \\
426881614218441600 & 12.47192 & 60.12738 & 4.50162 & 9.55 & 10.21 & 8.79 & 0.7 & 0.08 & L & 117.76 & 21.69 & 99.25 & 17.60 \\
5254000340399606016 & 157.26590 & -60.78069 & 4.50519 & 14.48 & 15.29 & 13.56 & 1.03 & 0.11 & O & 117.70 & 21.68 & 98.04 & 17.38 \\
5594382644652353664 & 119.05201 & -32.60264 & 4.51675 & 11.53 & 12.38 & 10.70 & 0.87 & 0.13 & G & 117.51 & 21.65 & 104.57 & 18.54 \\
5850308411442294400 & 206.85370 & -68.24990 & 4.52474 & 13.65 & 14.14 & 13.00 & 0.37 & 0.11 & G & 117.38 & 21.62 & 101.46 & 17.99 \\
4054440301294394624 & 262.70159 & -33.60992 & 4.52781 & 7.55 & 8.14 & 6.92 & 0.48 & 0.05 & L & 117.33 & 21.61 & 99.80 & 17.69 \\
5534012004528220160 & 119.94883 & -42.02838 & 4.54706 & 13.90 & 14.74 & 12.98 & 1.01 & 0.13 & G & 117.02 & 21.56 & 99.94 & 17.72 \\
506699870563323264 & 33.28119 & 58.07995 & 4.56524 & 11.27 & 11.94 & 10.55 & 0.62 & 0.06 & L & 116.73 & 21.50 & 100.73 & 17.86 \\
2012787293154800896 & 358.60238 & 62.14947 & 4.56615 & 11.45 & 12.28 & 10.57 & 0.96 & 0.12 & L & 116.71 & 21.50 & 99.82 & 17.70 \\
5338148473537341312 & 165.30989 & -60.11656 & 4.58610 & 11.08 & 11.81 & 10.25 & 0.76 & 0.07 & L & 116.40 & 21.44 & 102.76 & 18.22 \\
4690829659971892480 & 16.84515 & -70.88734 & 4.59426 & 15.88 & 16.22 & 15.37 & 0.09 & 0.11 & G & 116.27 & 21.42 & 99.99 & 17.73 \\
5253884788591163648 & 158.53969 & -61.59759 & 4.61631 & 13.91 & 14.75 & 12.99 & 1.01 & 0.11 & O & 115.92 & 21.35 & 99.13 & 17.58 \\
5253661725170126720 & 159.49855 & -62.20590 & 4.63195 & 14.41 & 15.35 & 13.63 & 0.9 & 0.11 & O & 115.67 & 21.31 & 103.28 & 18.31 \\
1981006115714214912 & 327.39800 & 52.39523 & 4.63908 & 11.46 & 12.45 & 10.48 & 0.91 & 0.23 & L & 115.56 & 21.29 & 119.68 & 21.22 \\
5521459979795304320 & 129.42007 & -47.36195 & 4.63985 & 7.71 & 8.26 & 7.05 & 0.38 & 0.04 & L & 115.55 & 21.29 & 104.23 & 18.48 \\
2170880813073764352 & 322.34628 & 49.11002 & 4.64071 & 11.77 & 12.62 & 10.87 & 0.99 & 0.13 & G & 115.54 & 21.28 & 99.48 & 17.64 \\
3044483895581000192 & 107.31421 & -13.78609 & 4.67003 & 10.09 & 10.85 & 9.26 & 0.77 & 0.07 & L & 115.08 & 21.20 & 102.54 & 18.18 \\
5338207327417387520 & 163.13667 & -60.52675 & 4.67416 & 10.94 & 11.55 & 10.19 & 0.54 & 0.08 & L & 115.02 & 21.19 & 102.22 & 18.12 \\
5338438297925480320 & 162.89899 & -59.38499 & 4.67767 & 9.41 & 9.97 & 8.73 & 0.52 & 0.04 & L & 114.96 & 21.18 & 96.83 & 17.17 \\
3046774762417915136 & 109.15680 & -11.48730 & 4.67830 & 7.83 & 8.33 & 7.20 & 0.32 & 0.03 & L & 114.95 & 21.18 & 101.79 & 18.05 \\
6060173364061645696 & 193.59158 & -58.43063 & 4.68971 & 6.36 & 6.80 & 5.79 & 0.23 & 0.03 & L & 114.78 & 21.14 & 100.13 & 17.75 \\
5861196531541297664 & 187.06483 & -65.04976 & 4.72838 & 14.52 & 15.34 & 13.58 & 1.06 & 0.12 & O & 114.19 & 21.03 & 94.22 & 16.71 \\
1998384927774603520 & 359.11116 & 58.02686 & 4.73481 & 11.71 & 12.60 & 10.79 & 1.03 & 0.13 & G & 114.09 & 21.02 & 98.50 & 17.46 \\
5242088403212116864 & 163.61189 & -61.34710 & 4.75984 & 11.54 & 12.32 & 10.69 & 0.85 & 0.13 & G & 113.72 & 20.95 & 98.71 & 17.50 \\
5533407170051636608 & 122.95171 & -42.05164 & 4.76441 & 14.79 & 15.90 & 13.77 & 1.36 & 0.15 & G & 113.65 & 20.93 & 97.92 & 17.36 \\
5541229748611783296 & 123.70107 & -37.65190 & 4.78070 & 13.80 & 14.82 & 12.79 & 1.24 & 0.13 & O & 113.41 & 20.89 & 98.71 & 17.50 \\
3051692843568009600 & 106.78562 & -7.79513 & 4.49659 & 12.54 & 13.27 & 11.70 & 0.87 & 0.11 & L & 117.84 & 21.71 & 98.06 & 17.39 \\
2011303326105008768 & 353.74839 & 59.35815 & 4.78948 & 12.14 & 13.26 & 11.08 & 1.45 & 0.16 & G & 113.28 & 20.87 & 95.28 & 16.89 \\
3099066951319051008 & 102.70284 & -7.98073 & 4.80971 & 12.57 & 13.26 & 11.77 & 0.62 & 0.08 & L & 112.98 & 20.81 & 103.42 & 18.34 \\
5864184488751391744 & 203.61003 & -64.37098 & 4.82483 & 14.71 & 15.56 & 13.75 & 1.31 & 0.13 & O & 112.76 & 20.77 & 82.04 & 14.55 \\
5329338700985814656 & 130.05832 & -47.55156 & 4.82751 & 13.24 & 14.15 & 12.28 & 1.12 & 0.14 & G & 112.72 & 20.76 & 95.89 & 17.00 \\
2928116120387181824 & 108.72647 & -22.23586 & 4.84478 & 12.81 & 13.54 & 11.97 & 0.8 & 0.12 & G & 112.47 & 20.72 & 96.74 & 17.15 \\
5306782361701536128 & 140.15436 & -56.85401 & 4.86219 & 13.91 & 14.60 & 13.11 & 0.72 & 0.12 & G & 112.21 & 20.67 & 96.53 & 17.11 \\
1960750328384177408 & 327.92260 & 43.13402 & 4.86438 & 8.67 & 9.19 & 8.03 & 0.39 & 0.04 & L & 112.18 & 20.66 & 96.20 & 17.06 \\
2011892703004353792 & 359.57487 & 61.22105 & 4.87514 & 10.66 & 11.41 & 9.83 & 0.75 & 0.07 & L & 112.03 & 20.64 & 100.07 & 17.74 \\
3344297935963515008 & 91.43635 & 13.23999 & 4.90958 & 11.89 & 12.64 & 11.03 & 0.71 & 0.06 & L & 111.53 & 20.55 & 103.93 & 18.43 \\
2078709577944648192 & 297.06443 & 43.12692 & 4.92549 & 8.90 & 9.42 & 8.26 & 0.43 & 0.05 & L & 111.31 & 20.50 & 93.72 & 16.62 \\
5258574068220187648 & 153.88689 & -58.17444 & 4.93255 & 10.24 & 10.94 & 9.46 & 0.59 & 0.08 & L & 111.21 & 20.49 & 103.12 & 18.28 \\
2060460704279873536 & 304.19788 & 36.54994 & 4.94524 & 11.57 & 12.65 & 10.54 & 1.45 & 0.19 & L & 111.03 & 20.45 & 89.03 & 15.78 \\
2055122987639665664 & 301.33609 & 32.65909 & 4.95045 & 12.27 & 13.38 & 11.21 & 1.35 & 0.18 & L & 110.96 & 20.44 & 97.92 & 17.36 \\
270272675510149504 & 64.94524 & 48.95326 & 4.97249 & 9.12 & 9.99 & 8.23 & 0.92 & 0.09 & L & 110.65 & 20.38 & 99.09 & 17.57 \\
5333640230992516480 & 173.32410 & -63.24240 & 4.97458 & 11.78 & 12.80 & 10.78 & 1.26 & 0.15 & G & 110.62 & 20.38 & 94.32 & 16.72 \\
3351921532976862336 & 100.15651 & 11.72748 & 4.97853 & 11.77 & 12.69 & 10.82 & 1.1 & 0.14 & G & 110.56 & 20.37 & 94.75 & 16.80 \\
2003938801532007808 & 342.15829 & 56.32153 & 4.98330 & 8.61 & 9.15 & 7.94 & 0.4 & 0.06 & L & 110.50 & 20.35 & 97.47 & 17.28 \\
6057402526059795072 & 181.66763 & -62.59685 & 4.98851 & 12.06 & 13.02 & 11.10 & 1.14 & 0.12 & O & 110.43 & 20.34 & 95.74 & 16.97 \\
2011315528113463808 & 354.70162 & 59.39182 & 4.99754 & 10.50 & 11.42 & 9.58 & 1.09 & 0.1 & L & 110.30 & 20.32 & 93.55 & 16.59 \\
5699042480743325312 & 120.09545 & -23.70317 & 5.02730 & 10.08 & 10.53 & 9.49 & 0.26 & 0.04 & L & 109.89 & 20.24 & 94.94 & 16.83 \\
515599111517099136 & 33.60315 & 65.59945 & 5.02942 & 11.90 & 12.75 & 11.01 & 0.7 & 0.12 & L & 109.86 & 20.24 & 112.38 & 19.93 \\
2164359918864249728 & 316.94415 & 46.73698 & 5.05758 & 11.90 & 12.74 & 11.01 & 0.99 & 0.13 & L & 109.48 & 20.17 & 92.41 & 16.38 \\
3390186156826555136 & 79.69992 & 13.98667 & 5.06607 & 11.52 & 12.19 & 10.67 & 0.78 & 0.12 & G & 109.36 & 20.15 & 92.30 & 16.37 \\
473293889810320128 & 57.10698 & 59.44227 & 5.06643 & 10.00 & 11.16 & 8.95 & 1.01 & 0.1 & L & 109.36 & 20.14 & 123.37 & 21.87 \\
5595650351503904896 & 118.45324 & -30.46031 & 5.07756 & 10.55 & 11.29 & 9.73 & 0.74 & 0.07 & L & 109.21 & 20.12 & 96.62 & 17.13 \\
5871738271033526016 & 207.68449 & -57.58051 & 5.07890 & 7.43 & 7.89 & 6.85 & 0.28 & 0.03 & L & 109.19 & 20.11 & 93.06 & 16.50 \\
2166303099490547072 & 311.55230 & 45.47861 & 5.09955 & 10.53 & 11.69 & 9.46 & 1.45 & 0.19 & L & 108.91 & 20.06 & 94.48 & 16.75 \\
5241157421762533248 & 162.23993 & -64.17420 & 5.10249 & 13.62 & 14.29 & 12.82 & 0.7 & 0.12 & G & 108.88 & 20.06 & 93.48 & 16.57 \\
5307006215391311360 & 142.54990 & -56.80824 & 5.13704 & 14.57 & 15.64 & 13.51 & 1.39 & 0.14 & O & 108.42 & 19.97 & 90.86 & 16.11 \\
2011892325047232256 & 359.53933 & 61.21370 & 5.14077 & 10.49 & 11.07 & 9.62 & 0.75 & 0.1 & L & 108.37 & 19.96 & 88.56 & 15.70 \\
4080122796947250176 & 281.32290 & -20.64739 & 5.15424 & 7.25 & 7.83 & 6.58 & 0.42 & 0.04 & L & 108.19 & 19.93 & 95.99 & 17.02 \\
4085919765884068736 & 282.74947 & -20.29525 & 6.63703 & 6.63 & 7.21 & 5.93 & 0.38 & 0.03 & L & 92.35 & 17.01 & 83.44 & 14.79 \\
1827869808377481216 & 296.64660 & 22.88975 & 5.19725 & 10.03 & 10.96 & 9.09 & 1.23 & 0.12 & L & 107.63 & 19.83 & 84.26 & 14.94 \\
4690377382729299328 & 10.34143 & -70.61853 & 5.20108 & 15.23 & 15.52 & 14.77 & -0.0 & 0.11 & G & 107.58 & 19.82 & 91.22 & 16.17 \\
5254295559276699392 & 159.07421 & -61.01256 & 5.20456 & 9.06 & 9.56 & 8.44 & 0.29 & 0.05 & L & 107.53 & 19.81 & 95.63 & 16.96 \\
5853170268450896768 & 219.37630 & -63.62524 & 5.21445 & 14.44 & 15.27 & 13.50 & 1.08 & 0.12 & O & 107.41 & 19.78 & 87.23 & 15.47 \\
5257939993613539456 & 147.08272 & -57.81045 & 5.21666 & 12.34 & 13.28 & 11.37 & 1.15 & 0.12 & O & 107.38 & 19.78 & 91.51 & 16.22 \\
513830684503187840 & 34.09382 & 62.55776 & 5.23993 & 12.62 & 13.62 & 11.62 & 1.23 & 0.15 & G & 107.08 & 19.72 & 91.42 & 16.21 \\
5698636279917579520 & 119.52141 & -24.04176 & 5.25024 & 10.34 & 10.80 & 9.73 & 0.35 & 0.05 & L & 106.95 & 19.70 & 88.44 & 15.68 \\
1968971582984827136 & 318.66850 & 41.71634 & 5.25760 & 8.88 & 9.91 & 7.90 & 1.22 & 0.11 & L & 106.85 & 19.68 & 92.17 & 16.34 \\
189726984845700480 & 86.05833 & 37.58687 & 5.25943 & 11.56 & 12.33 & 10.81 & 0.74 & 0.1 & L & 106.83 & 19.68 & 91.88 & 16.29 \\
6053622679932061056 & 188.32775 & -63.50637 & 5.26567 & 9.01 & 9.91 & 8.12 & 0.86 & 0.09 & L & 106.75 & 19.66 & 100.60 & 17.84 \\
5594100246268225280 & 119.84298 & -33.35713 & 5.28196 & 13.39 & 14.27 & 12.46 & 1.01 & 0.11 & O & 106.54 & 19.63 & 93.08 & 16.50 \\
4147381366335558784 & 272.50888 & -13.54596 & 5.30141 & 9.96 & 11.03 & 8.94 & 1.31 & 0.11 & L & 106.30 & 19.58 & 91.06 & 16.14 \\
5334506135119058304 & 171.27392 & -60.73461 & 5.30996 & 8.49 & 9.08 & 7.79 & 0.48 & 0.1 & L & 106.19 & 19.56 & 92.54 & 16.41 \\
5307761545524640256 & 147.17283 & -55.51953 & 5.32402 & 9.79 & 10.57 & 8.95 & 0.79 & 0.1 & L & 106.02 & 19.53 & 93.26 & 16.53 \\
1960981328902089088 & 330.10480 & 43.44535 & 5.33166 & 8.57 & 9.13 & 7.90 & 0.45 & 0.05 & L & 105.92 & 19.51 & 90.74 & 16.09 \\
5338215200143652992 & 163.78784 & -60.54772 & 5.33671 & 11.44 & 12.27 & 10.56 & 0.92 & 0.13 & G & 105.86 & 19.50 & 91.37 & 16.20 \\
5255220656517219840 & 156.71194 & -59.66953 & 5.34632 & 9.03 & 9.64 & 8.31 & 0.58 & 0.05 & L & 105.74 & 19.48 & 89.30 & 15.83 \\
458239995077788544 & 38.63042 & 58.83162 & 5.36511 & 10.46 & 11.49 & 9.51 & 1.2 & 0.1 & L & 105.51 & 19.44 & 90.56 & 16.06 \\
4190143160245024256 & 298.08750 & -11.36692 & 5.37668 & 7.54 & 8.03 & 6.92 & 0.25 & 0.03 & L & 105.37 & 19.41 & 95.07 & 16.86 \\
2010285491880986112 & 346.79198 & 58.55419 & 5.44090 & 9.28 & 9.96 & 8.51 & 0.64 & 0.06 & L & 104.59 & 19.27 & 91.29 & 16.18 \\
5547742052903182080 & 122.60782 & -32.52136 & 5.46460 & 10.99 & 11.72 & 10.18 & 0.74 & 0.12 & G & 104.30 & 19.21 & 90.70 & 16.08 \\
5312211543950752128 & 142.56597 & -53.05868 & 5.48394 & 11.19 & 12.09 & 10.25 & 1.06 & 0.14 & G & 104.07 & 19.17 & 89.33 & 15.84 \\
5338131529834231680 & 164.77043 & -60.27884 & 5.49457 & 11.65 & 12.46 & 10.76 & 0.91 & 0.13 & G & 103.94 & 19.15 & 89.36 & 15.84 \\
5891675303053080704 & 218.13779 & -56.88775 & 5.49457 & 6.55 & 7.11 & 5.93 & 0.36 & 0.04 & L & 103.94 & 19.15 & 91.48 & 16.22 \\
523887951723531648 & 11.62454 & 63.54327 & 5.51273 & 11.17 & 12.21 & 10.18 & 1.29 & 0.17 & L & 103.73 & 19.11 & 86.60 & 15.35 \\
5715183929918131968 & 115.47870 & -21.13306 & 5.51615 & 10.27 & 10.82 & 9.61 & 0.45 & 0.04 & L & 103.69 & 19.10 & 87.88 & 15.58 \\
459035766618689280 & 36.89776 & 58.91715 & 5.53070 & 10.37 & 11.47 & 9.37 & 1.28 & 0.11 & L & 103.52 & 19.07 & 90.92 & 16.12 \\
5253795384546671104 & 158.01837 & -61.78262 & 5.54225 & 8.70 & 9.18 & 8.09 & 0.25 & 0.03 & L & 103.38 & 19.04 & 91.48 & 16.22 \\
4103989346187406464 & 276.80604 & -15.11799 & 5.54693 & 10.07 & 10.94 & 9.18 & 0.95 & 0.13 & G & 103.33 & 19.03 & 89.87 & 15.93 \\
5539107450645759232 & 118.43778 & -36.97038 & 5.56408 & 10.59 & 11.47 & 9.75 & 0.88 & 0.13 & G & 103.13 & 19.00 & 91.69 & 16.26 \\
5254512193075687168 & 158.63079 & -59.80854 & 5.57332 & 11.84 & 12.94 & 10.79 & 1.31 & 0.13 & O & 103.02 & 18.98 & 91.75 & 16.27 \\
5525918495131126912 & 126.02410 & -44.85228 & 5.59210 & 13.08 & 14.24 & 12.02 & 1.45 & 0.16 & G & 102.81 & 18.94 & 87.04 & 15.43 \\
506602976101284736 & 26.76131 & 59.60626 & 5.60412 & 13.19 & 13.92 & 12.35 & 0.64 & 0.15 & L & 102.67 & 18.91 & 96.65 & 17.14 \\
5283779135317992448 & 98.37366 & -65.99373 & 5.63702 & 15.67 & 16.06 & 15.11 & 0.16 & 0.11 & G & 102.29 & 18.84 & 87.95 & 15.59 \\
2005753545481718912 & 331.89771 & 55.36274 & 5.65812 & 12.18 & 13.11 & 11.22 & 1.23 & 0.12 & L & 102.05 & 18.80 & 80.97 & 14.36 \\
5242185808733501696 & 162.09637 & -60.65394 & 5.66418 & 12.16 & 12.99 & 11.26 & 0.93 & 0.11 & O & 101.98 & 18.79 & 88.35 & 15.66 \\
2015622212085282048 & 354.86371 & 62.37214 & 5.66617 & 11.06 & 12.01 & 10.12 & 1.03 & 0.09 & L & 101.96 & 18.78 & 91.13 & 16.16 \\
2202863166783787520 & 330.67041 & 59.45248 & 5.68839 & 13.10 & 14.14 & 12.10 & 1.26 & 0.15 & G & 101.71 & 18.74 & 86.89 & 15.41 \\
5261561063335550208 & 95.02971 & -75.36110 & 5.70035 & 15.26 & 15.65 & 14.69 & 0.17 & 0.11 & G & 101.58 & 18.71 & 86.90 & 15.41 \\
2931247014102560000 & 108.29864 & -18.73074 & 5.72861 & 10.60 & 11.39 & 9.75 & 0.62 & 0.12 & L & 101.27 & 18.65 & 100.41 & 17.80 \\
2034428980559814400 & 299.89044 & 33.74604 & 5.78290 & 11.05 & 11.99 & 10.12 & 0.99 & 0.13 & L & 100.67 & 18.54 & 91.08 & 16.15 \\
5600471160241231616 & 118.49014 & -28.36762 & 5.80047 & 12.61 & 13.41 & 11.73 & 0.91 & 0.11 & O & 100.48 & 18.51 & 84.75 & 15.03 \\
422226488141991296 & 3.61766 & 56.25293 & 5.80901 & 8.78 & 9.37 & 8.08 & 0.44 & 0.08 & L & 100.39 & 18.49 & 88.92 & 15.77 \\
5613165915335320192 & 111.16913 & -26.18849 & 5.81585 & 11.45 & 12.33 & 10.54 & 0.94 & 0.12 & L & 100.31 & 18.48 & 89.37 & 15.85 \\
5327836325732931840 & 131.23286 & -50.56002 & 5.85935 & 9.21 & 9.96 & 8.39 & 0.72 & 0.07 & L & 99.84 & 18.39 & 88.97 & 15.77 \\
5595072420703114624 & 116.96477 & -32.17133 & 5.86387 & 13.12 & 14.08 & 12.16 & 1.13 & 0.14 & G & 99.80 & 18.38 & 85.09 & 15.09 \\
5544213926244557184 & 120.20160 & -37.82794 & 5.88476 & 10.63 & 11.53 & 9.71 & 1.02 & 0.13 & G & 99.57 & 18.34 & 85.67 & 15.19 \\
5436296928693979392 & 143.46188 & -36.61574 & 5.89839 & 9.12 & 9.52 & 8.58 & 0.41 & 0.05 & L & 99.43 & 18.32 & 72.21 & 12.80 \\
467560314629168640 & 41.46454 & 63.30457 & 5.90466 & 11.96 & 12.78 & 11.08 & 0.91 & 0.12 & L & 99.36 & 18.30 & 84.78 & 15.03 \\
5308893149150949248 & 145.29272 & -53.81604 & 5.90482 & 11.10 & 11.98 & 10.19 & 0.97 & 0.09 & L & 99.36 & 18.30 & 86.72 & 15.38 \\
2055014277739104896 & 303.09511 & 32.87160 & 5.95590 & 8.91 & 9.76 & 8.02 & 0.88 & 0.09 & L & 98.83 & 18.20 & 88.11 & 15.62 \\
5927687916632523264 & 250.53743 & -57.31247 & 5.95730 & 12.82 & 13.38 & 12.12 & 0.46 & 0.11 & G & 98.81 & 18.20 & 85.19 & 15.10 \\
5544001136384668288 & 121.32198 & -37.58019 & 6.02134 & 13.52 & 14.50 & 12.51 & 1.23 & 0.13 & O & 98.15 & 18.08 & 81.50 & 14.45 \\
4092905375639902464 & 277.97221 & -19.12510 & 6.74522 & 6.35 & 7.01 & 5.62 & 0.55 & 0.05 & L & 91.42 & 16.84 & 79.40 & 14.08 \\
1808020329279916288 & 300.29090 & 15.80350 & 6.10820 & 9.90 & 10.44 & 9.26 & 0.31 & 0.04 & L & 97.28 & 17.92 & 87.39 & 15.49 \\
4312361436842603520 & 287.31663 & 10.55247 & 6.11423 & 7.66 & 8.44 & 6.84 & 0.86 & 0.07 & L & 97.22 & 17.91 & 80.07 & 14.20 \\
6053428684887800320 & 185.88240 & -64.47089 & 6.12121 & 11.32 & 12.29 & 10.35 & 0.96 & 0.09 & L & 97.15 & 17.90 & 92.85 & 16.46 \\
4303770918113986304 & 299.38759 & 11.04366 & 6.17926 & 9.72 & 10.21 & 9.10 & 0.14 & 0.02 & L & 96.58 & 17.79 & 91.95 & 16.30 \\
4093976334264606976 & 273.85944 & -20.62955 & 6.17945 & 10.19 & 11.07 & 9.25 & 1.11 & 0.14 & L & 96.58 & 17.79 & 77.80 & 13.79 \\
5932812431123862016 & 241.29147 & -53.91943 & 6.19933 & 9.48 & 10.30 & 8.64 & 0.78 & 0.08 & L & 96.38 & 17.75 & 86.71 & 15.37 \\
506581226385580288 & 27.77925 & 59.88821 & 6.20627 & 10.30 & 11.02 & 9.50 & 0.66 & 0.06 & L & 96.31 & 17.74 & 85.09 & 15.09 \\
6059764002146656128 & 191.59278 & -59.12473 & 6.22040 & 8.07 & 8.64 & 7.38 & 0.4 & 0.04 & L & 96.18 & 17.72 & 85.67 & 15.19 \\
2059598687167348352 & 299.44206 & 35.63605 & 6.22543 & 12.68 & 13.69 & 11.69 & 1.26 & 0.16 & L & 96.13 & 17.71 & 79.05 & 14.02 \\
2008504454839717120 & 341.60318 & 59.44219 & 6.23397 & 9.00 & 9.92 & 8.08 & 0.95 & 0.08 & L & 96.05 & 17.69 & 87.16 & 15.45 \\
430670222050230912 & 9.18544 & 62.27424 & 6.24022 & 11.73 & 12.72 & 10.75 & 1.16 & 0.15 & L & 95.99 & 17.68 & 82.72 & 14.67 \\
525136962570940160 & 18.75456 & 65.59940 & 6.27279 & 10.23 & 11.24 & 9.28 & 1.17 & 0.1 & L & 95.67 & 17.62 & 81.23 & 14.40 \\
2015820463470505600 & 354.31691 & 62.42899 & 6.29664 & 9.24 & 10.22 & 8.28 & 1.08 & 0.09 & L & 95.45 & 17.58 & 84.96 & 15.06 \\
4512950187838606464 & 286.51934 & 15.74941 & 6.30024 & 14.61 & 15.49 & 13.67 & 1.03 & 0.13 & G & 95.41 & 17.58 & 81.17 & 14.39 \\
5823134325151372032 & 240.29463 & -63.77655 & 6.31663 & 6.22 & 6.59 & 5.63 & 0.12 & 0.02 & L & 95.26 & 17.55 & 83.68 & 14.84 \\
2027263738130844288 & 299.36918 & 26.55645 & 6.32059 & 8.23 & 9.14 & 7.30 & 1.05 & 0.09 & L & 95.22 & 17.54 & 81.20 & 14.40 \\
1994462866719961216 & 354.40810 & 54.84718 & 6.33647 & 9.03 & 9.72 & 8.26 & 0.63 & 0.12 & G & 95.07 & 17.51 & 82.76 & 14.67 \\
5339149677605627264 & 169.58945 & -59.23796 & 6.39427 & 12.57 & 13.31 & 11.72 & 0.77 & 0.1 & O & 94.53 & 17.41 & 81.54 & 14.46 \\
6057514092119497472 & 183.24857 & -62.09682 & 6.39726 & 10.47 & 11.36 & 9.60 & 0.86 & 0.07 & L & 94.50 & 17.41 & 85.60 & 15.18 \\
2006989121667184384 & 340.36050 & 56.43277 & 6.41896 & 8.55 & 9.09 & 7.89 & 0.36 & 0.04 & L & 94.30 & 17.37 & 82.57 & 14.64 \\
4096979650282842112 & 276.18542 & -16.79717 & 6.42429 & 8.41 & 9.08 & 7.59 & 0.67 & 0.06 & L & 94.25 & 17.36 & 81.52 & 14.45 \\
3291491450496573824 & 74.97904 & 10.28845 & 6.44163 & 14.32 & 14.74 & 13.69 & 0.27 & 0.11 & G & 94.10 & 17.33 & 79.23 & 14.05 \\
5254071873026676864 & 160.70349 & -61.12298 & 6.45365 & 11.21 & 11.96 & 10.38 & 0.75 & 0.12 & G & 93.99 & 17.31 & 81.37 & 14.43 \\
5312196047720402048 & 143.34884 & -52.75585 & 6.45380 & 11.06 & 12.07 & 10.08 & 1.14 & 0.1 & L & 93.98 & 17.31 & 82.86 & 14.69 \\
5868480143187802240 & 199.74280 & -62.38235 & 6.45975 & 8.08 & 8.71 & 7.34 & 0.5 & 0.08 & L & 93.93 & 17.30 & 83.38 & 14.78 \\
174489098011145216 & 71.94298 & 36.72278 & 6.46466 & 7.05 & 7.73 & 6.27 & 0.65 & 0.06 & L & 93.89 & 17.29 & 80.57 & 14.28 \\
513282131279401728 & 23.91530 & 65.33050 & 6.55713 & 12.49 & 13.65 & 11.42 & 1.45 & 0.16 & G & 93.05 & 17.14 & 78.29 & 13.88 \\
4096140001386430080 & 275.82979 & -18.57477 & 6.56959 & 9.80 & 10.83 & 8.83 & 1.13 & 0.09 & L & 92.94 & 17.12 & 82.30 & 14.59 \\
272444829450300160 & 67.57792 & 53.94018 & 6.56983 & 11.86 & 12.74 & 10.95 & 0.96 & 0.13 & G & 92.94 & 17.12 & 80.28 & 14.23 \\
5541507237862358912 & 123.09332 & -36.94374 & 6.66423 & 7.71 & 8.14 & 7.16 & 0.22 & 0.02 & L & 92.12 & 16.97 & 76.39 & 13.54 \\
5302258008774271488 & 127.18202 & -60.12256 & 6.69695 & 7.11 & 7.60 & 6.50 & 0.22 & 0.03 & L & 91.83 & 16.92 & 81.75 & 14.49 \\
5338072980840100608 & 165.93830 & -60.64226 & 6.69721 & 9.84 & 10.49 & 9.10 & 0.59 & 0.06 & L & 91.83 & 16.92 & 77.94 & 13.82 \\
4314923363333177984 & 293.01969 & 11.54976 & 6.69729 & 12.54 & 13.22 & 11.75 & 0.65 & 0.12 & G & 91.83 & 16.92 & 79.10 & 14.02 \\
2177714415280658944 & 323.72762 & 55.94226 & 6.71632 & 12.85 & 13.93 & 11.82 & 1.31 & 0.15 & G & 91.67 & 16.89 & 77.65 & 13.77 \\
6054829806275577216 & 185.33793 & -62.28164 & 6.73287 & 6.30 & 6.81 & 5.68 & 0.26 & 0.04 & L & 91.53 & 16.86 & 81.46 & 14.44 \\
429544700100302080 & 4.26041 & 60.80280 & 6.79828 & 13.65 & 14.60 & 12.67 & 1.02 & 0.13 & L & 90.97 & 16.76 & 82.86 & 14.69 \\
4204653587029046400 & 287.08654 & -7.43777 & 6.80601 & 7.34 & 8.02 & 6.57 & 0.58 & 0.05 & L & 90.91 & 16.75 & 80.55 & 14.28 \\
5935042378098601856 & 243.98144 & -51.12073 & 6.81248 & 10.33 & 11.31 & 9.38 & 1.1 & 0.14 & G & 90.86 & 16.74 & 78.57 & 13.93 \\
4505300988492333312 & 281.47541 & 12.33610 & 7.50794 & 9.75 & 10.36 & 9.00 & 0.53 & 0.07 & L & 85.49 & 15.75 & 73.09 & 12.96 \\
430766016998901376 & 8.31747 & 62.90726 & 6.84634 & 10.97 & 11.87 & 10.07 & 1.04 & 0.09 & L & 90.57 & 16.68 & 74.60 & 13.23 \\
5324034867356093056 & 137.06555 & -51.43625 & 6.92436 & 7.22 & 7.93 & 6.44 & 0.59 & 0.05 & L & 89.93 & 16.57 & 80.98 & 14.36 \\
2030848897634605440 & 300.19314 & 30.90759 & 6.96110 & 12.11 & 13.21 & 11.06 & 1.41 & 0.18 & L & 89.64 & 16.51 & 72.40 & 12.84 \\
5352181712213705856 & 159.03578 & -56.04323 & 6.98477 & 10.22 & 10.83 & 9.31 & 0.72 & 0.06 & L & 89.45 & 16.48 & 75.69 & 13.42 \\
3031875585286182144 & 110.50990 & -14.31818 & 6.99483 & 9.24 & 9.82 & 8.54 & 0.5 & 0.06 & L & 89.37 & 16.46 & 74.30 & 13.17 \\
5334563996911649408 & 179.47384 & -62.64613 & 7.00373 & 11.44 & 12.37 & 10.49 & 1.06 & 0.14 & G & 89.29 & 16.45 & 76.45 & 13.56 \\
5903821951590649600 & 228.74274 & -46.87257 & 7.05894 & 13.89 & 14.42 & 13.21 & 0.37 & 0.11 & G & 88.86 & 16.37 & 76.47 & 13.56 \\
5877533315817003648 & 219.29985 & -62.01092 & 7.06626 & 6.42 & 6.96 & 5.77 & 0.31 & 0.04 & L & 88.80 & 16.36 & 79.05 & 14.01 \\
3113441691460573312 & 102.63473 & 0.00700 & 7.09748 & 11.97 & 12.83 & 11.03 & 0.88 & 0.11 & L & 88.55 & 16.31 & 80.35 & 14.25 \\
5240438203718296192 & 165.36850 & -64.29067 & 7.12163 & 13.71 & 14.51 & 12.82 & 0.87 & 0.13 & G & 88.37 & 16.28 & 75.29 & 13.35 \\
5309174967720762496 & 144.21441 & -53.03278 & 7.13431 & 9.69 & 10.51 & 8.83 & 0.93 & 0.11 & L & 88.27 & 16.26 & 71.70 & 12.71 \\
5860785795219397376 & 184.39009 & -65.75399 & 7.13451 & 13.83 & 14.46 & 12.97 & 0.58 & 0.09 & O & 88.27 & 16.26 & 79.97 & 14.18 \\
5257664497238811776 & 148.85895 & -58.42969 & 7.19619 & 8.95 & 9.58 & 8.22 & 0.51 & 0.04 & L & 87.79 & 16.17 & 76.29 & 13.53 \\
5600628115523816320 & 117.51301 & -28.25514 & 7.19862 & 10.32 & 11.10 & 9.50 & 0.78 & 0.1 & L & 87.77 & 16.17 & 74.90 & 13.28 \\
5626365410677889792 & 131.05061 & -35.47371 & 7.21689 & 9.94 & 10.60 & 9.17 & 0.59 & 0.12 & G & 87.63 & 16.14 & 75.89 & 13.46 \\
2174677564161400064 & 326.32669 & 54.49638 & 7.23099 & 11.38 & 12.40 & 10.39 & 1.19 & 0.14 & G & 87.53 & 16.12 & 74.47 & 13.20 \\
2007997408188526336 & 337.20867 & 58.21093 & 7.23213 & 10.62 & 11.46 & 9.74 & 0.86 & 0.07 & L & 87.52 & 16.12 & 76.55 & 13.57 \\
4307944836090489600 & 290.25978 & 8.51633 & 7.23996 & 9.35 & 10.33 & 8.39 & 1.1 & 0.09 & L & 87.46 & 16.11 & 75.36 & 13.36 \\
2165771172070496512 & 317.72654 & 49.14204 & 7.25140 & 9.95 & 10.88 & 9.00 & 1.05 & 0.09 & L & 87.37 & 16.09 & 74.98 & 13.29 \\
5335963189825411072 & 172.84735 & -60.58341 & 7.34403 & 13.08 & 13.96 & 12.13 & 1.04 & 0.12 & O & 86.68 & 15.97 & 72.48 & 12.85 \\
5613564621430610560 & 111.82868 & -25.78535 & 7.41934 & 12.70 & 13.62 & 11.73 & 0.78 & 0.23 & L & 86.13 & 15.87 & 87.41 & 15.50 \\
3112475495616980992 & 104.50389 & -0.37596 & 7.42462 & 10.35 & 11.04 & 9.57 & 0.59 & 0.06 & L & 86.09 & 15.86 & 76.20 & 13.51 \\
5855468247702904704 & 190.52089 & -69.40756 & 7.51028 & 6.10 & 6.55 & 5.55 & 0.2 & 0.04 & L & 85.48 & 15.75 & 71.46 & 12.67 \\
2934712880912798464 & 108.42673 & -17.62026 & 7.51211 & 12.39 & 13.36 & 11.42 & 1.11 & 0.14 & G & 85.46 & 15.74 & 72.77 & 12.90 \\
5337191279923824384 & 168.04213 & -61.75487 & 7.53200 & 7.80 & 8.35 & 7.14 & 0.29 & 0.03 & L & 85.32 & 15.72 & 76.80 & 13.62 \\
3368698813404804352 & 95.55497 & 14.67813 & 7.56688 & 8.12 & 8.76 & 7.42 & 0.45 & 0.04 & L & 85.07 & 15.67 & 75.28 & 13.35 \\
5337958876494096256 & 165.10434 & -60.99319 & 7.63695 & 12.31 & 13.20 & 11.37 & 0.99 & 0.11 & O & 84.58 & 15.58 & 72.35 & 12.83 \\
5339394082770287232 & 167.42135 & -58.83772 & 7.72081 & 6.61 & 7.08 & 6.01 & 0.15 & 0.02 & L & 84.01 & 15.47 & 75.78 & 13.44 \\
5415098722470316544 & 152.59186 & -44.15874 & 7.77785 & 13.69 & 14.15 & 13.08 & 0.23 & 0.11 & G & 83.62 & 15.40 & 71.88 & 12.74 \\
2016028168089215488 & 356.26093 & 63.00385 & 7.80112 & 10.08 & 11.04 & 9.12 & 1.01 & 0.08 & L & 83.47 & 15.38 & 74.78 & 13.26 \\
2030063919381336832 & 299.79498 & 29.45072 & 7.81823 & 9.37 & 10.16 & 8.51 & 0.82 & 0.07 & L & 83.35 & 15.35 & 70.84 & 12.56 \\
1873112207907294848 & 316.06930 & 39.97223 & 7.85582 & 9.05 & 9.82 & 8.20 & 0.8 & 0.07 & L & 83.10 & 15.31 & 69.70 & 12.36 \\
470361114339849472 & 61.24359 & 58.65978 & 7.91561 & 7.16 & 7.92 & 6.32 & 0.74 & 0.06 & L & 82.71 & 15.24 & 71.63 & 12.70 \\
5614916921960857088 & 114.04436 & -25.36403 & 7.96016 & 14.49 & 15.58 & 13.45 & 1.29 & 0.13 & O & 82.42 & 15.18 & 69.99 & 12.41 \\
2170785842762144512 & 322.18718 & 48.97821 & 7.96686 & 10.10 & 10.90 & 9.24 & 0.8 & 0.12 & G & 82.37 & 15.17 & 71.12 & 12.61 \\
1825621002188696448 & 294.15720 & 20.33293 & 7.99014 & 6.58 & 7.41 & 5.72 & 0.81 & 0.07 & L & 82.22 & 15.15 & 72.14 & 12.79 \\
428620663657823232 & 7.49410 & 60.21196 & 8.00066 & 8.51 & 9.23 & 7.71 & 0.66 & 0.05 & L & 82.16 & 15.13 & 71.15 & 12.61 \\
261548119462093568 & 77.66762 & 49.68760 & 8.00263 & 9.06 & 9.69 & 8.32 & 0.53 & 0.06 & L & 82.14 & 15.13 & 70.18 & 12.44 \\
5236551193933797888 & 174.75935 & -65.20662 & 8.00290 & 14.65 & 15.67 & 13.62 & 1.18 & 0.12 & O & 82.14 & 15.13 & 71.02 & 12.59 \\
3050050207554658048 & 105.24924 & -8.70898 & 8.01127 & 9.62 & 10.32 & 8.79 & 0.68 & 0.07 & L & 82.09 & 15.12 & 70.31 & 12.47 \\
5852880955104044800 & 214.51090 & -64.42147 & 8.19958 & 14.15 & 15.00 & 13.17 & 1.04 & 0.12 & O & 80.90 & 14.90 & 66.73 & 11.83 \\
5887482762148283008 & 228.20632 & -54.75528 & 8.22041 & 9.02 & 9.90 & 8.19 & 0.91 & 0.1 & L & 80.77 & 14.88 & 66.81 & 11.85 \\
512524361613040640 & 23.18010 & 63.59380 & 8.37701 & 6.64 & 7.46 & 5.78 & 0.8 & 0.11 & L & 79.83 & 14.70 & 69.72 & 12.36 \\
3329849043206545920 & 92.80659 & 9.61249 & 8.61488 & 8.67 & 9.24 & 7.99 & 0.3 & 0.03 & L & 78.44 & 14.45 & 71.16 & 12.62 \\
202939854734748032 & 70.99117 & 40.83478 & 8.63925 & 11.13 & 11.87 & 10.29 & 0.72 & 0.06 & L & 78.30 & 14.42 & 67.23 & 11.92 \\
5613972681993587200 & 115.49584 & -25.87617 & 8.93422 & 8.74 & 9.31 & 8.04 & 0.41 & 0.04 & L & 76.67 & 14.12 & 65.29 & 11.58 \\
5254097093074642944 & 159.83465 & -61.15243 & 9.19783 & 8.80 & 9.39 & 8.12 & 0.24 & 0.03 & L & 75.29 & 13.87 & 71.48 & 12.67 \\
4056026175045038464 & 267.15626 & -30.47597 & 9.31686 & 8.24 & 9.08 & 7.43 & 0.77 & 0.07 & L & 74.69 & 13.76 & 64.44 & 11.43 \\
5854560115494081024 & 215.45224 & -61.54966 & 9.46519 & 8.26 & 8.97 & 7.47 & 0.58 & 0.05 & L & 73.95 & 13.62 & 65.49 & 11.61 \\
4269036830424588800 & 288.19714 & 3.55740 & 9.48055 & 7.90 & 8.67 & 7.12 & 0.66 & 0.05 & L & 73.88 & 13.61 & 63.88 & 11.33 \\
5329838158460391296 & 131.22276 & -46.34296 & 9.56113 & 7.97 & 8.53 & 7.36 & 0.32 & 0.03 & L & 73.49 & 13.54 & 61.93 & 10.98 \\
5835124087174043136 & 244.71595 & -57.89980 & 9.75376 & 6.15 & 6.70 & 5.52 & 0.25 & 0.02 & L & 72.57 & 13.37 & 64.29 & 11.40 \\
5351423049186195328 & 158.22527 & -58.52100 & 9.75912 & 11.01 & 11.86 & 10.14 & 0.71 & 0.07 & L & 72.55 & 13.36 & 67.79 & 12.02 \\
5993655659352495616 & 243.61906 & -40.79315 & 9.76457 & 12.20 & 12.89 & 11.39 & 0.62 & 0.12 & G & 72.52 & 13.36 & 61.72 & 10.94 \\
5254662177677566464 & 155.34567 & -61.07408 & 9.76811 & 8.59 & 9.09 & 7.96 & 0.23 & 0.03 & L & 72.51 & 13.36 & 62.91 & 11.15 \\
2013029941628292352 & 359.39565 & 62.71824 & 9.80569 & 9.44 & 10.16 & 8.65 & 0.66 & 0.06 & L & 72.33 & 13.32 & 61.10 & 10.83 \\
5241804518715438336 & 165.39269 & -62.21022 & 9.84085 & 12.20 & 13.06 & 11.27 & 0.92 & 0.11 & O & 72.17 & 13.29 & 61.36 & 10.88 \\
5328248672646357120 & 132.04364 & -48.65915 & 9.84168 & 11.91 & 13.00 & 10.91 & 1.19 & 0.11 & L & 72.17 & 13.29 & 62.56 & 11.09 \\
5328949100222702848 & 130.67412 & -48.68614 & 10.02929 & 14.30 & 15.33 & 13.28 & 1.19 & 0.14 & G & 71.32 & 13.14 & 60.00 & 10.64 \\
4685261526923834496 & 2.60032 & -75.17706 & 10.09004 & 14.71 & 15.03 & 14.23 & 0.0 & 0.11 & G & 71.05 & 13.09 & 57.80 & 10.25 \\
2070224337474904064 & 311.49913 & 45.30694 & 10.14797 & 9.42 & 10.48 & 8.42 & 1.12 & 0.09 & L & 70.80 & 13.04 & 62.75 & 11.12 \\
5337257834740652160 & 167.55357 & -60.84747 & 10.27245 & 11.09 & 12.12 & 10.09 & 1.11 & 0.11 & L & 70.26 & 12.94 & 61.18 & 10.85 \\
201574982848108416 & 74.92307 & 40.83603 & 10.30573 & 9.92 & 10.67 & 9.10 & 0.73 & 0.08 & L & 70.12 & 12.92 & 57.88 & 10.26 \\
4156450099578283776 & 279.51377 & -8.36895 & 10.34150 & 8.88 & 9.93 & 7.92 & 1.07 & 0.09 & L & 69.96 & 12.89 & 61.72 & 10.94 \\
5241780677399802624 & 165.37783 & -62.29079 & 10.35488 & 10.31 & 11.08 & 9.47 & 0.63 & 0.06 & L & 69.91 & 12.88 & 63.50 & 11.26 \\
5859119760248045312 & 198.50696 & -64.32488 & 10.35635 & 10.85 & 11.83 & 9.89 & 1.06 & 0.13 & L & 69.90 & 12.88 & 59.81 & 10.60 \\
5538569613358406144 & 117.35518 & -38.23935 & 10.50594 & 12.62 & 13.34 & 11.79 & 0.67 & 0.12 & G & 69.28 & 12.76 & 59.07 & 10.47 \\
4267549637851481344 & 286.16423 & 1.30614 & 17.13794 & 7.88 & 8.66 & 7.00 & 0.75 & 0.07 & L & 51.00 & 9.39 & 42.00 & 7.45 \\
5337764640889249536 & 168.58836 & -60.05292 & 10.70960 & 9.27 & 9.92 & 8.51 & 0.45 & 0.05 & L & 68.45 & 12.61 & 61.13 & 10.84 \\
506779550797525760 & 31.95200 & 58.44353 & 10.87727 & 8.84 & 9.58 & 8.04 & 0.65 & 0.06 & L & 67.79 & 12.49 & 57.71 & 10.23 \\
2007201567928631296 & 340.21724 & 56.82946 & 10.88439 & 8.04 & 8.70 & 7.29 & 0.48 & 0.04 & L & 67.76 & 12.48 & 59.52 & 10.55 \\
5871922507947292032 & 205.07765 & -57.61318 & 10.94947 & 7.47 & 8.03 & 6.79 & 0.33 & 0.03 & L & 67.51 & 12.43 & 58.12 & 10.30 \\
3027495856819349248 & 113.41167 & -16.31710 & 10.98248 & 11.04 & 11.89 & 10.16 & 0.82 & 0.12 & G & 67.38 & 12.41 & 57.92 & 10.27 \\
4256744187345732224 & 280.53297 & -4.29349 & 11.05302 & 9.92 & 11.04 & 8.88 & 1.26 & 0.1 & L & 67.11 & 12.36 & 57.76 & 10.24 \\
203496585576324224 & 72.44976 & 42.28970 & 11.11731 & 8.60 & 9.23 & 7.85 & 0.44 & 0.06 & L & 66.87 & 12.32 & 59.13 & 10.48 \\
5611465073923671424 & 106.94491 & -24.91952 & 11.18235 & 11.25 & 11.81 & 10.56 & 0.35 & 0.11 & G & 66.62 & 12.27 & 57.15 & 10.13 \\
5313887130948758016 & 142.92069 & -49.65499 & 11.20064 & 8.88 & 9.83 & 7.95 & 0.92 & 0.08 & L & 66.55 & 12.26 & 59.37 & 10.53 \\
462407693902385792 & 52.35821 & 60.44647 & 11.27625 & 11.76 & 12.88 & 10.76 & 1.18 & 0.1 & L & 66.27 & 12.21 & 58.43 & 10.36 \\
5932569709575669504 & 243.32248 & -54.23490 & 11.28752 & 7.98 & 8.65 & 7.24 & 0.43 & 0.04 & L & 66.23 & 12.20 & 59.67 & 10.58 \\
3430067092837622272 & 91.64561 & 26.32922 & 11.30513 & 9.34 & 9.97 & 8.64 & 0.47 & 0.06 & L & 66.17 & 12.19 & 55.55 & 9.85 \\
2002637323358768000 & 343.65706 & 54.26545 & 11.31916 & 13.43 & 14.15 & 12.54 & 0.74 & 0.1 & L & 66.12 & 12.18 & 55.33 & 9.81 \\
200708636406382720 & 75.34662 & 39.96038 & 11.62570 & 7.34 & 7.94 & 6.68 & 0.34 & 0.04 & L & 65.02 & 11.98 & 55.97 & 9.92 \\
5332375453374624640 & 178.07378 & -65.40418 & 11.63735 & 9.33 & 10.09 & 8.59 & 0.58 & 0.07 & L & 64.98 & 11.97 & 55.71 & 9.88 \\
2030427789026783488 & 299.45419 & 30.26590 & 11.66304 & 10.42 & 11.28 & 9.52 & 1.05 & 0.13 & L & 64.89 & 11.95 & 49.05 & 8.70 \\
2073922579215436288 & 301.01866 & 39.10421 & 11.92821 & 12.97 & 13.86 & 12.03 & 0.93 & 0.13 & G & 63.98 & 11.79 & 54.10 & 9.59 \\
1999252442448732288 & 358.02928 & 58.74172 & 12.14061 & 9.32 & 10.20 & 8.46 & 0.86 & 0.08 & L & 63.28 & 11.66 & 53.21 & 9.43 \\
5336389564126521728 & 175.70084 & -58.99339 & 12.18311 & 10.90 & 11.71 & 10.02 & 0.75 & 0.08 & L & 63.14 & 11.63 & 54.76 & 9.71 \\
6054992602724692608 & 188.59725 & -61.23762 & 12.21766 & 11.13 & 12.23 & 10.11 & 1.29 & 0.12 & L & 63.03 & 11.61 & 51.14 & 9.07 \\
4066375912402666624 & 274.06943 & -23.30591 & 12.27464 & 15.32 & 16.30 & 14.35 & 1.29 & 0.13 & O & 62.85 & 11.58 & 45.96 & 8.15 \\
5616601820448126336 & 111.52996 & -25.25730 & 12.35350 & 9.39 & 10.15 & 8.59 & 0.74 & 0.06 & L & 62.59 & 11.53 & 49.95 & 8.86 \\
5240441472232302848 & 165.56688 & -64.26289 & 12.43802 & 8.85 & 9.60 & 8.06 & 0.53 & 0.05 & L & 62.33 & 11.48 & 56.30 & 9.98 \\
5884729035255064064 & 238.67837 & -54.56644 & 12.63346 & 8.96 & 9.87 & 8.03 & 0.82 & 0.1 & L & 61.72 & 11.37 & 55.89 & 9.91 \\
470386952863752576 & 61.53736 & 58.80875 & 12.65005 & 10.26 & 11.19 & 9.37 & 0.7 & 0.09 & L & 61.67 & 11.36 & 59.75 & 10.59 \\
5865206961464617088 & 201.62523 & -63.16263 & 12.88787 & 11.05 & 12.22 & 10.01 & 1.34 & 0.21 & L & 60.96 & 11.23 & 50.26 & 8.91 \\
4253435825622331392 & 280.73864 & -5.82091 & 12.91058 & 9.10 & 9.92 & 8.35 & 0.72 & 0.08 & L & 60.89 & 11.22 & 49.45 & 8.77 \\
5310669788148987520 & 139.59222 & -54.41226 & 13.12071 & 13.73 & 14.71 & 12.75 & 1.06 & 0.14 & G & 60.28 & 11.10 & 50.71 & 8.99 \\
5311616398935271168 & 140.00627 & -52.85618 & 13.23958 & 10.85 & 11.86 & 9.89 & 0.98 & 0.11 & L & 59.94 & 11.04 & 53.04 & 9.40 \\
4313179507891570304 & 287.50172 & 12.53654 & 13.43999 & 10.08 & 11.20 & 9.07 & 1.38 & 0.18 & L & 59.38 & 10.94 & 44.94 & 7.97 \\
5350852677538959104 & 162.75755 & -58.59059 & 13.45493 & 10.91 & 11.91 & 9.97 & 0.94 & 0.08 & L & 59.34 & 10.93 & 53.22 & 9.44 \\
5600915775257809152 & 119.42569 & -27.60189 & 13.45979 & 11.49 & 12.36 & 10.66 & 0.84 & 0.1 & L & 59.32 & 10.93 & 48.59 & 8.62 \\
5614312705966204288 & 117.01604 & -25.57777 & 13.59892 & 9.50 & 10.14 & 8.79 & 0.49 & 0.05 & L & 58.94 & 10.86 & 48.31 & 8.56 \\
459263743483634304 & 36.80736 & 59.46060 & 13.63864 & 9.14 & 10.11 & 8.19 & 0.96 & 0.11 & L & 58.83 & 10.84 & 51.18 & 9.07 \\
5596601154188852352 & 121.58947 & -30.09687 & 13.67010 & 9.49 & 10.23 & 8.67 & 0.57 & 0.05 & L & 58.75 & 10.82 & 52.01 & 9.22 \\
6030635804488868480 & 249.53582 & -31.47765 & 13.68681 & 12.78 & 13.33 & 12.09 & 0.32 & 0.11 & G & 58.70 & 10.81 & 50.02 & 8.87 \\
4267397694768545920 & 287.05729 & 1.29863 & 13.75460 & 6.61 & 7.39 & 5.85 & 0.66 & 0.06 & L & 58.52 & 10.78 & 48.60 & 8.62 \\
5586922973654572416 & 116.29911 & -36.97475 & 13.76670 & 12.17 & 12.95 & 11.27 & 0.78 & 0.12 & G & 58.49 & 10.77 & 48.96 & 8.68 \\
4087335043492541696 & 286.51307 & -18.42825 & 13.77231 & 12.49 & 13.06 & 11.81 & 0.31 & 0.11 & G & 58.48 & 10.77 & 50.22 & 8.90 \\
206577210999441536 & 74.41700 & 46.09253 & 13.84765 & 11.03 & 12.01 & 10.07 & 1.06 & 0.09 & L & 58.28 & 10.74 & 47.81 & 8.48 \\
2243309938950947200 & 304.41505 & 62.75205 & 13.98367 & 14.12 & 14.63 & 13.61 & 0.02 & 0.11 & G & 57.92 & 10.67 & 51.76 & 9.18 \\
5351331755370445056 & 161.23472 & -56.28954 & 14.10712 & 8.07 & 8.99 & 7.51 & 0.51 & 0.05 & L & 57.60 & 10.61 & 50.28 & 8.91 \\
5597327141100381568 & 119.74674 & -29.30786 & 14.15735 & 9.98 & 10.74 & 9.17 & 0.61 & 0.05 & L & 57.48 & 10.59 & 49.77 & 8.82 \\
2016626856473497344 & 352.30314 & 63.37430 & 14.37514 & 10.78 & 11.94 & 9.72 & 1.29 & 0.11 & L & 56.93 & 10.49 & 48.62 & 8.62 \\
6026412893938675712 & 254.58229 & -33.60913 & 6.06133 & 6.67 & 7.17 & 5.95 & 0.46 & 0.04 & L & 97.75 & 18.01 & 81.63 & 14.47 \\
2161786374436607616 & 315.02658 & 42.59755 & 14.71797 & 8.39 & 9.71 & 7.28 & 1.52 & 0.12 & L & 56.10 & 10.33 & 47.10 & 8.35 \\
508915489570374272 & 24.30841 & 57.75922 & 14.79237 & 8.81 & 9.08 & 8.01 & 0.59 & 0.06 & L & 55.92 & 10.30 & 35.32 & 6.26 \\
2034684200359279488 & 297.82201 & 32.67553 & 15.00336 & 13.12 & 14.18 & 12.05 & 1.42 & 0.18 & L & 55.43 & 10.21 & 40.72 & 7.22 \\
5864955727424819200 & 203.49590 & -64.05556 & 15.04436 & 9.72 & 10.54 & 8.88 & 0.57 & 0.06 & L & 55.33 & 10.19 & 51.83 & 9.19 \\
2016581673416790656 & 350.61846 & 62.75714 & 15.09343 & 10.12 & 11.35 & 9.12 & 1.27 & 0.11 & L & 55.22 & 10.17 & 47.29 & 8.38 \\
2071433765909167232 & 308.22621 & 46.60125 & 15.11946 & 8.82 & 9.73 & 7.91 & 0.8 & 0.07 & L & 55.16 & 10.16 & 49.20 & 8.72 \\
3324153371114695680 & 95.35961 & 6.47015 & 15.23122 & 8.02 & 8.65 & 7.32 & 0.36 & 0.04 & L & 54.90 & 10.11 & 47.56 & 8.43 \\
5537860123428416640 & 119.69307 & -38.99433 & 15.55821 & 11.46 & 12.34 & 10.55 & 0.9 & 0.12 & L & 54.18 & 9.98 & 44.34 & 7.86 \\
6704330080883057536 & 281.53600 & -48.63307 & 16.09459 & 12.59 & 13.03 & 11.97 & 0.12 & 0.11 & G & 53.04 & 9.77 & 44.53 & 7.89 \\
1870258975238302208 & 310.85080 & 35.58778 & 16.39062 & 6.07 & 6.69 & 5.36 & 0.34 & 0.03 & L & 52.44 & 9.66 & 45.58 & 8.08 \\
6026305309220584576 & 253.41732 & -33.34511 & 16.40369 & 12.99 & 13.59 & 12.25 & 0.39 & 0.11 & G & 52.41 & 9.65 & 44.42 & 7.88 \\
4638315266636230400 & 30.74872 & -74.05691 & 16.48065 & 14.19 & 14.70 & 13.59 & 0.13 & 0.11 & G & 52.26 & 9.63 & 45.30 & 8.03 \\
5338036117182452096 & 166.05607 & -60.97991 & 16.65998 & 8.19 & 8.90 & 7.38 & 0.5 & 0.05 & L & 51.91 & 9.56 & 45.78 & 8.12 \\
2058374144759464064 & 301.11066 & 34.11225 & 17.07369 & 8.46 & 9.24 & 7.61 & 0.69 & 0.06 & L & 51.12 & 9.42 & 42.99 & 7.62 \\
5878388529664102016 & 218.79935 & -60.99798 & 17.11025 & 9.85 & 10.96 & 8.74 & 1.27 & 0.12 & L & 51.05 & 9.40 & 42.98 & 7.62 \\
2198162651491732608 & 329.46952 & 56.16389 & 17.87198 & 9.83 & 10.85 & 8.87 & 0.92 & 0.1 & L & 49.68 & 9.15 & 44.78 & 7.94 \\
5253717937706836480 & 159.23233 & -61.58131 & 18.05246 & 11.66 & 12.47 & 10.73 & 0.76 & 0.1 & O & 49.36 & 9.09 & 42.21 & 7.48 \\
6026596989041710336 & 254.88447 & -32.95258 & 18.13188 & 12.53 & 13.10 & 11.76 & 0.4 & 0.11 & G & 49.23 & 9.07 & 41.02 & 7.27 \\
5255254711361371520 & 157.07013 & -59.35018 & 18.17758 & 8.30 & 8.97 & 7.52 & 0.44 & 0.06 & L & 49.15 & 9.05 & 42.99 & 7.62 \\
188724234539584256 & 78.84160 & 40.07802 & 18.19076 & 9.78 & 10.66 & 8.85 & 0.74 & 0.1 & L & 49.13 & 9.05 & 44.36 & 7.86 \\
5351161399785606016 & 161.13616 & -57.56536 & 18.87302 & 7.15 & 7.82 & 6.43 & 0.36 & 0.04 & L & 48.01 & 8.84 & 42.09 & 7.46 \\
1873250780732545920 & 314.33680 & 40.17749 & 20.14034 & 9.27 & 10.36 & 8.28 & 1.13 & 0.11 & L & 46.10 & 8.49 & 38.20 & 6.77 \\
5523162573544337408 & 129.25540 & -44.11465 & 20.49764 & 6.66 & 7.31 & 5.90 & 0.41 & 0.04 & L & 45.59 & 8.40 & 39.09 & 6.93 \\
5937099633141128448 & 251.32962 & -51.34264 & 20.85306 & 9.60 & 10.51 & 8.67 & 0.74 & 0.06 & L & 45.10 & 8.31 & 41.03 & 7.28 \\
4644478166748030976 & 35.20622 & -73.08565 & 21.36729 & 13.63 & 14.02 & 13.06 & 0.0 & 0.11 & G & 44.42 & 8.18 & 36.80 & 6.52 \\
4094784475310672128 & 274.24882 & -19.07583 & 21.83410 & 7.48 & 8.43 & 6.62 & 0.62 & 0.06 & L & 43.82 & 8.07 & 41.83 & 7.42 \\
4103564728516764032 & 280.45457 & -14.50543 & 11.03608 & 13.65 & 14.58 & 12.94 & 0.58 & 0.12 & G & 67.17 & 12.37 & 63.48 & 11.25 \\
6350220751862829952 & 358.65290 & -83.28872 & 22.44150 & 14.31 & 15.01 & 13.60 & 0.34 & 0.11 & G & 43.08 & 7.94 & 37.97 & 6.73 \\
5600052040150252800 & 114.64682 & -28.49960 & 23.17284 & 9.22 & 9.95 & 8.42 & 0.58 & 0.05 & L & 42.22 & 7.78 & 34.35 & 6.09 \\
5253571526514498176 & 159.11275 & -62.19251 & 24.21976 & 12.41 & 13.32 & 11.49 & 0.76 & 0.1 & O & 41.07 & 7.57 & 36.05 & 6.39 \\
5858474003300201856 & 193.43279 & -65.89971 & 26.46392 & 11.93 & 12.63 & 11.09 & 0.51 & 0.09 & O & 38.85 & 7.16 & 33.03 & 5.86 \\
6096564686351860992 & 213.33208 & -44.89374 & 26.68846 & 12.41 & 13.00 & 11.69 & 0.28 & 0.11 & G & 38.65 & 7.12 & 32.65 & 5.79 \\
5355057622305532928 & 155.17091 & -55.32138 & 28.16616 & 7.82 & 8.68 & 6.96 & 0.73 & 0.06 & L & 37.37 & 6.88 & 30.69 & 5.44 \\
5964193485048327808 & 252.91061 & -45.42671 & 28.86509 & 8.85 & 10.11 & 7.76 & 1.15 & 0.11 & L & 36.80 & 6.78 & 34.38 & 6.10 \\
5597379741549105280 & 119.59202 & -29.13008 & 30.09021 & 8.12 & 9.00 & 7.26 & 0.72 & 0.06 & L & 35.85 & 6.60 & 29.69 & 5.26 \\
5238808628736339584 & 164.28834 & -65.13474 & 15.71624 & 8.66 & 9.31 & 7.85 & 0.47 & 0.04 & L & 53.84 & 9.92 & 46.88 & 8.31 \\
5864135319959353600 & 204.15366 & -64.55832 & 34.05097 & 9.10 & 10.18 & 8.12 & 0.98 & 0.1 & L & 33.18 & 6.11 & 28.19 & 5.00 \\
5546476927338700416 & 123.26755 & -34.57851 & 41.46411 & 6.46 & 7.30 & 5.58 & 0.61 & 0.05 & L & 29.33 & 5.40 & 24.90 & 4.42 \\
2027951173435143680 & 297.87876 & 27.46021 & 44.87621 & 6.66 & 7.50 & 5.78 & 0.64 & 0.06 & L & 27.92 & 5.14 & 23.10 & 4.09 \\
\end{tabular}
\end{table}

